Towards Natural Language-Based Visualization Authoring

A key challenge to visualization authoring is the process of getting familiar with the complex user interfaces of authoring tools. Natural Language Interface (NLI) presents promising benefits due to its learnability and usability. However, supporting NLIs for authoring tools requires expertise in natural language processing, while existing NLIs are mostly designed for visual analytic workflow. In this paper, we propose an authoring-oriented NLI pipeline by introducing a structured representation of users' visualization editing intents, called editing actions, based on a formative study and an extensive survey on visualization construction tools. The editing actions are executable, and thus decouple natural language interpretation and visualization applications as an intermediate layer. We implement a deep learning-based NL interpreter to translate NL utterances into editing actions. The interpreter is reusable and extensible across authoring tools. The authoring tools only need to map the editing actions into tool-specific operations. To illustrate the usages of the NL interpreter, we implement an Excel chart editor and a proof-of-concept authoring tool, VisTalk. We conduct a user study with VisTalk to understand the usage patterns of NL-based authoring systems. Finally, we discuss observations on how users author charts with natural language, as well as implications for future research.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/CHI_appen-interpreter.tex <==
\section{NL-based Visualization Framework}
We consider the design of our natural language framework against the following requirements: (1)  The framework should be reusable for common visualization construction and configuration intents and support different visualization applications. (2) The framework should be easy to extend to cover more visualization commands and the capability can be improved over time. (3) The framework should support flexible natural language input with vague descriptions.

Based on these considerations, we introduce our natural language-based visualization editing framework (Figure \ref{fig:pipeline}). 
The framework consists of two parts, a \textbf{natural language interpreter} and an \textbf{visualization application}. 
When a user inputs a natural language sentence, the interpreter parses it into \textbf{editing actions} and sends the actions to the application. 
The editing actions are a list of structured descriptions of users' intents and can be executed by the application. \wy{Then, we provide a design guidelines of visualization applications based on the NL interpreter.}

%We design a natural language interpreter that parses human utterances to visualization authoring actions and can be applied across different authoring tools. %\sherry{First sentence is a bit duplicated with the last paragraph; And I think this paragraph needs a rewrite.}
% We model users' visualization editing intents as \textit{editing actions} and formulate an editing action as the combination of \textit{operation}, \textit{objects}, and \textit{parameters}. We summarize and categorize common editing actions into six categories that cover visualization authoring functions in authoring tools. 
%Users' natural utterances can be parsed into authoring actions and passed to applications to execute. 
%First, we define a domain-specific language (DSL) of visualization authoring, covering common operations for visualization authoring from 6 aspects. 
%The natural language processing module takes users' utterances as input, and outputs the program in the form of our DSL. The code can be further parsed and implemented by specific applications or code libraries to complete the specific tasks under different design environments.


\subsection{Editing Actions}\label{sec:model}
A wide variety of visualization creation systems \cite{Wongsuphasawat2016VoyagerEA, 6876042, Liu:2018:DIA:3173574.3173697}, code libraries \cite{bostock2011d3}, and declarative languages \cite{satyanarayan2016vega} have been developed to support visualization creation. Existing tools usually consider marks, data bindings, scales, axes, legends, and layout when specifying charts.
%Further, the visualization authoring systems are implemented with different models. Satyanarayan \etal \cite{satyanarayan2019critical} categorize them into three different types, namely, template editors, shelf construction, and visual builders. Common visualization authoring tools like Microsoft Excel, adopt template editors way. Shelf construction methods support more flexible mapping between encoding channels and data fields, and are adopted by Tableau, Polestar \cite{Pioch2006POLESTARCK}, and Voyager \cite{Wongsuphasawat2016VoyagerEA}. Visual builders like Charticulator \cite{Ren_2019_8440827} and iVisDesigner \cite{6876042} are more complicated and support fine control in specifying marks, glyphs, layouts, etc.
These tools have covered a wide range of functions to enable the composition of both standard charts and highly customized interactive visualizations. However, there was no common design model that can let us consistently describe visualization editing intents \cite{satyanarayan2019critical}.
We survey the functions of modern interactive authoring systems including Microsoft Excel, Tableau, Polestar and Voyager\cite{Wongsuphasawat2017Voyager2A}, Lyra \cite{satyanarayan2014lyra}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and declarative model Vega-lite \cite{satyanarayan2016vega} to recognize common authoring operations and functions. %We identified a set of common functions and categorize them into six categories. 


\wy{These visualization construction tools can be divided into three category \cite{satyanarayan2019critical}. Tools like Microsoft Excel supports \textit{template editor} style, where users may start with a chart type and further make extensive customization. Users may say ``Give me a bar chart for \textit{Sales} by \textit{Country}'' for a bar chart with y-axis encoded with Sales and x-axis encoded with different countries.  Tools like Tableau, Voyager \cite{Wongsuphasawat2017Voyager2A} constructs visualizations by mapping data fields to encoding channels (e.g., x, y, color, shape). An example utterance can be ``Bind \textit{Sales} to y-axis'' and ``Bind \textit{Country} to x-axis''. The tools might further automatically recommend rectangles as marks.  Tools like Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909}, construct visualizations from the fine control of marks, glyphs, coordinate systems, and layouts. Users might start with ``draw a rectangle'', and then, ``repeat it horizontally on \textit{Country}'', and finally ``bind height to \textit{Sales}'' to construct a similar bar chart. Therefore, to fit into these  different styles of visualization tools flexibly, we propose the notion of editing action as the combination of operation, object, and parameters, where users' authoring intents can be simplified as \textit{editing operation} and its \textit{target objects}, and the corresponding \textit{parameters}. }


We define \textit{editing actions} as the combination of authoring \textit{operations}, \textit{objects}, and \textit{parameters}. User utterances can be mapped to one or multiple editing actions. The authoring process of visualization is the execution of a sequence of editing actions. Formally, an authoring intention can be defined as a triple:
\begin{equation}\nonumber
    \texttt{editing~action := \{operation, objects, parameters\}}
\end{equation}

The definition of the editing action describes the actions the authors want to take to the visualizations.  The \textit{operation} identifies the type of the author's intent (e.g., ``change color'', ``add annotation''). The \textit{objects} are the targets that the operation applies to, such as the canvas area, the bars in a bar chart, the title text,etc. Finally, the \textit{parameters} indicate the degree or configurations of the operations.


\begin{table*}[!t]
    \centering
    \includegraphics[width=1\linewidth]{pictures/new-taxonomy-cropped.pdf}
    \vspace{0px}
    \caption{An editing action consists of three parts, operation, object, and parameter.  Operation are categorized into six major groups. Objects are categorized into chart components (e.g., axes, legends, title), mark channels (e.g., shape, color, size, position), and annotations (e.g., reference lines, reference bands, trend lines). \todo{remove this table and replace with a simpler image}}
    \label{fig:taxonomy}
    \vspace{-1px}
\end{table*}

\subsubsection{Operations}
%Our framework models the action of users' authoring requests as a sequence of operations %. %The basic operations are primitive operations (e.g., data binding, change color, change font, etc.). More complex operations can be combined with multiple primitive operations and are used to complete typical design tasks. For example, ``turn the bar chart to a pictograph.'' \todo{how to} %All the operations require target objects (e.g., axes, marks) and parameters. 
%Based on existing visualization authoring systems and taxonomies \cite{satyanarayan2016vega, Ren_2019_8440827, Liu:2018:DIA:3173574.3173697, Wang:2018:IEC:3173574.3173909, ren2017chartaccent}, 
%The most primitive operations that appear in visualization authoring tools 
%and 
%We categorize authoring operation into six major groups.
%, namely, data operations, visual encoding operations, layout operations, styling operations, view manipulations, and annotate operations.\todo{no need to list the names of the categories since they will be listed below...} 
%Different o
Operations may apply to different objects, depending on the properties of the objects. 
Table 1 lists the operations and the corresponding target objects and possible parameters. 
As discussed previously, operations are not exclusive because different tools support different design paradigm and human languages also express same meanings with different patterns. For example, binding a data field to x axis, has the same effect as encode the horizontal position of mark to the field.   
%We list common editing actions that are used in visualization authoring.
% \begin{compactitem}
%     \item \textbf{General operations}, like \textit{add}, \textit{remove}, \textit{copy}, are the operations that can be acted upon any object, including graphical elements (e.g., add an annotation) or data encoding (e.g., remove a filter).
%     \item \textbf{Data encoding} is the mapping between data and visual channels.
%     \item \textbf{Data transform} are the operations that are related to data query and calculation, such as \textit{select}, \textit{filter}, \textit{pivot}, and \textit{join}.
%     \item \textbf{Selectors} are the operations that are applied to the objects with visual properties, such as \textit{change color}, \textit{modify shape}. For example, users can change the color of the title; or change the color scheme for the marks in a chart. Users may even replace the marks with icons for expressive visualization design.
%     \item \textbf{Numerical operators} are the operations that are related to the numerical properties of objects. Change range, of something. For example, change the height and width.
%     \item \textbf{layout operators} are a special type of numerical operators that can be widely used for expressive visualization designs. Users may add labels, annotations, and configure the positions of them. They may \textit{move} up or left, \textit{change position} to a specific point, or even \textit{adjust z-order} for the graphical elements.
%     \item \textbf{Text operators} include the operations that are specifically related to text. For example, users may \textit{modify content} of titles, or \textit{change font} for the annotations.
% \end{compactitem}
% \begin{compactitem}
%     \item \textbf{Bind} is the mapping between data and visual channels; data transformation and data fields; data transformation and visual channels 
%     \item \textbf{Add/Remove/Modify} can be applied to graphical element on a visualization design. For example, ``add the legend'', ``modify the title''. They can also be applied to data encoding, such as ``add a filter''.
%     \item \textbf{Set value} is applicable to any object with numerical properties, such as size, height, opacity, etc. 
%     \item \textbf{Change category} is used for the visualization objects with only discrete value properties.
%     \item \textbf{Color} is a special, color related, color scheme 
%     \item \textbf{Font} font style
%     \item \textbf{Style}
%     \item \textbf{Place} (move, position)
% \end{compactitem}
%The operations are categorized by visual features of the target objects. 
%In a visualization design, different visual components may have different properties. These properties further specify the variables that characterize the target components. For example, encoding supports different encoding channels such as position(x, y), size, and color. Marks have properties including shape, color, etc. The shapes for marks are rectangles for bar charts, circles for bubble charts, symbols for scatter plots, etc. The properties for marks also depend on the implementation of the charts. For example, a more flexible authoring tool may support users to replace the basic geometric shapes with icons, or even images. Following the implementation of existing authoring systems, 
\wy{We summarize the authoring operations by going through the category of Vega-Lite grammar \cite{satyanarayan2016vega}, from which we collect a large number of visualization operations related to \textit{data, encoding, and mark}.
To support the construction of more expressive visualizations, we further include common styling operations, and collect operations from ChartAccent \cite{ren2017chartaccent}, Charticulator \cite{Ren_2019_8440827}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909} to develop three more categories related to \textit{layout, styling, and annotation}. } We summarize six main categories of operations:
\begin{compactitem}
    \item \textbf{Data operations} are the operations that retrieve and calculate data from datasets. Typical operations include filter, aggregate, bin, set time unit, and sort.  
    \item \textbf{Encoding operations} are the operations that bind data fields to different encoding channels. Users may also take operations to the axes or directly assign chart types to specify encoding.%, while the effects might be the same. %For example, ``bind Country to x axis'' and ``bind Country to the horizontal position of marks'' have different objects (i.e., x axis and position), while they have the same effects. 
    \item \textbf{Mark operations} include the configurations related to the configuration of marks. Users may change the shape, color, style of marks. The types of mark can be vector shapes, text, images, icons, etc. 
    \item \textbf{Layout operations} include the configurations related to position and offsets of chart elements, such as title, annotation, legend. Users can place an object at a designated position, or move it along a direction.
    \item \textbf{Styling operations} includes graphical operations and textual operations. Graphical operations are performed to color, size, shape, icon, and stroke of graphical elements, such ass axis lines, marks, reference line, etc. Textual operations are acted to text-related properties such as font (size, color, style, weight), content. They can be applied to title, labels, annotations, etc.
    %\item \textbf{View manipulation} refers to operations that create one visualization with multiple views. Chart views can be created into multiple or layered displays. %Multiple views can also be created by ``faceting'' the current view by one data column (e.g., facet the sales by country) or ``repeating'' one chart view to other data values (e.g., repeat the sales chart for US and Japan). 
    \item \textbf{Annotate operations} manipulate annotations (e.g., text, labels, embellishments) that enhance the charts. Annotations can be bound with data. For example, trend lines can show the trend between two time points. Common types of annotations include labels, annotation text, reference line/band, trend line, average line, etc.
    %can show aggregated values by the marks\todo{do we have the corresponding operation for adding labels?} . 
\end{compactitem}



%Based on these operations, more complex high-level operations can be combined. For example, "change the style" usually means the combination of graphic properties and textual properties. This may even apply to the color coding of the marks, further impacting data encoding properties. ``Sales by year'' usually means create a chart, bind x axis with Sales, and bind y axis with Year.

% \begin{compactitem}
%     \item \textbf{Change Chart} removes the current chart encoding and applys new encoding to change the chart into a new one.
%     %ll\item \textbf{Repeat and partition}  
%     \item \textbf{View composition} (facets) applies all the settings and further modifys the data encoding properties.
%     \item \textbf{Fill percentage} adds a background icon with the same foreground icon but different colors.
%     \item \textbf{Interaction} specifies different sets of properties based on users' interaction conditions. Users need to specify the condition and the effects of the interactions.
% \end{compactitem}




\subsubsection{Objects}
Objects are the components that the operations target. 
%For an authoring operation, users usually need to specify the targeting object they want to create, modify, or remove. 
In \wy{WIMP (Window, Icon, Menu, Pointing)} interfaces, users usually click on the menus or select the targeting objects on canvas. For a natural language environment, users need to specify the objects through NL utterances.
For a basic visual chart, the objects include marks, axes, title, legend, gridlines, etc. More advanced objects include annotations such as trend line, reference line, reference band, text annotations, and embellishments.  

\wy{The objects are corresponding to different operations. For example, the objects of \textit{data operations} include data fields, data points, data type, data range etc. The objects of \textit{encoding operations} include the data fields, chart components such as axes, legends, title, and mark channels such as mark size, mark shape, mark position. The objects of \textit{styling operations} include visual properties such as opacity, stroke, text font, text color, and so on.}
% \wy{\begin{compactitem}
%     \item \textbf{Data/Datasets} include data fields, data points, data type, data range etc. When users conduct data operations, they need to assign parameters to these objects.
%     \item \textbf{Chart Components} are the basic parts of charts. This category includes plot area, axes, legends, title, etc.
%     \item \textbf{Mark channels} are targeted by encoding operations. Users need to encode data fields with different channels of marks, such as mark shape, mark color, and mark size.  
%     \item \textbf{Annotations} are additional graphical or textual elements to the charts. Annotations can be bound with data value or data points. For example, reference lines, reference bands are directed related to data; text annotations, image annotations can be placed near one certain data point; data labels can be shown at near each data point to show the values.
%     \item \textbf{Configs} are the properties of visual elements that styling operations take effects, including text font, stoke, opacity, width, and so on.
%     \item \textbf{Layout} are position-related visual properties. Users may need to change position, alignment, offset, z-index of the elements when position is not encoded with data.
% \end{compactitem}
% }

The objects in an editing action can be under specified. For example, a user may say ``give me a chart'' after uploading a dataset. An intelligent system can recommend a best encoding to users, or ask users to clarify the command.
We directly models users intention and use a special notation ``*'' to represent  the under specified objects. The implementation of visualization systems cam further decide definite reference strategies.

%Clearly, a target component may support more than one target operations\todo{???}. %A mark may simultaneously support encoding operations and styling operations. 

% To describe an authoring operation, users usually need to specify the targeting object they want to create, modify, or remove. 
% In graphical user interface systems, users usually click on the menus, or select the targeting objects on visualization canvas. For natural language environment, users need to specify the objects through their utterances.

% \textbf{Objects} are the components that the operations targeted to. For example, for a basic visual chart, the components include marks, axes, title, legend, encoding, etc. Authoring tools for standard charts usually only support limited number of target properties. Supported components can further include annotations such as trend line, reference line, text annotations, etc., depending on the implementation of different authoring tools.  
% Clearly, a target component may support more than one target properties. An implementation of visualization mark may simultaneously support general properties, graphic properties, and data encoding properties. 
% For example, the rectangles in a bar chart can be configured to different color and widths. The rectangle mark can also be replaced with other shapes to reach expressive visualization designs. While different target properties are handled by corresponding operations. The parameters further configure how to change these objects. 

%Once users obtain a chart, they may further say ``turn it to red''. The systems may infer the intention of the users is ``turn the marks to red''. We 

\textbf{Object Selectors.}
As discussed in Section 3, users show special patterns when referring to objects with natural language. 
They may refer to objects through \textit{object properties}. 
%For example, users may ask the system to ``turn the red line blue'', which means ``turn the line in red color to blue color''. Therefore, w
We support an object selector for users to filter the objects. For example, the intention ``turn the red line blue''  does not directly specify the object because there is no component named ``red line''. %The ``red line'' can be selected as \texttt{[shape=line,~ color=red]}, 
The statement can be presented as \sact{SetColor}{[shape=line,color=red]}{color=blue}, meaning to select objects the properties, ``line'' and ``red''. 
%The similar pattern can also be applied if visualization components are clearly referred to, but users would like to select parts of them. For example, ``add black stroke to the blue bar'' for a colored bar chart can be translated to \texttt{setStroke, [shape=bar, color=blue], color=black])\}}, meaning users wants to change the style of the mark with blue color and the operation is \texttt{setStroke}. 
The properties that users describe should exist in the predefined library of property and parameters. Otherwise, the natural language interpreter may not be able to match them and leave quotation marks to the text phrases. %Further, the natural language interpreter may not be able to understand the attribute type and leave a star mark as placeholder. Applications may further parse the attributes based on the context of authoring.
For example, ``add black stroke to the abc bar'' can be translated to 
\sact{setStroke}{[shape=bar,*=`abc']}{stroke=black}.

\textbf{Object Naming.}
We support object naming to enable easy reference. For example, after applying a filter ``US'' and ``2020'' to the chart, users can simply name the chart as ``US2020''. This helps them easily refer to this chart. Object naming further enables nested design of visualizations. For example, users may put two visualizations together by opening up a new canvas and saying ``put US2019 and US2020 side by side.'' This also helps enable creative visualization design. Figure \ref{fig:examples}c shows an example where the user  use two icons to create a pictograph and reuse it in another chart to create novel visualization design.



\subsubsection{Parameters}
Parameters are specific configurations of the operations. The parameters correspond to the operations and objects. It describes what extents the operations are performed, or how the operations are applied to the objects. Based on the object properties, we need to further define a library of parameters. By defining the forms of these parameters,  users' free-form natural language can be translated into machine-understandable commands. Table 1 shows example parameters corresponding to different chart objects. 
When users specify their requirements in natural language, the parameters can be clear and definite. For example, ``please set the chart 10px wide and 13px height.''
The parameters can be implemented as numerical values for chart width and height, enumerations for font style and encoding channels, boolean values for adding or removing components.



\textbf{Vague Parameters}
Natural languages might be rough and vague. We define a set of vague parameters for different operation types. For example, for color values, we support e a list of color names (e.g., \texttt{color=red}, \texttt{color=navy~blue}). We also define a number of extent keywords, ranging from ``extremely'', ``very'', ``moderate'', ``a little'', to ``very little''. Users can therefore describe the adjustments of size as ``make it really large'', which will be mapped to ``very large'' and can be parsed as \texttt{\{setSize, *, size=very.large\}}.
Authoring tools can further interpret them into machine-understandable values based on design environments.



\textbf{Relational Parameters}
With a well-defined parameter set, we can further turn the vague description of the intention to concrete parameters. We support two types of relational parameter that can converse users utterances such as ``make it larger'', or ``set the color of the title darker than the bars''. For each relational parameter, users need to specify the objects it compared to, and the direction of change. For example, ``make the title darker'' is explained as make ``itself'' darker, where the object is the title; ``place the legend on the right of the plot area'' is explained as ``right'' to the ``plot''. Formally, the utterances are interpreted to \texttt{\{setColor, title, color=self[+]\}} and 
\texttt{\{place, legend, position=plot[right]\}}. \texttt{self[+]} means the value larger than it self while \texttt{plot[right]} means on the right of the plot. Applications should further determine the exact values of these parameters after receiving these vague parameters.






\subsubsection{Example Utterances}
Combining operations, objects, and parameters, authoring actions can represent various authoring utterances. An utterance may corresponds to multiple authoring actions. 
Here we show example utterances and the corresponding authoring actions to further illustrate the use of authoring actions. In Table \ref{tab:examples}, the utterances are represent with one to four authoring actions. These examples include object selectors (d, e),  vague parameters (b, c, d, e, f), and relational parameters (b, d).

\begin{table}[ht]
\centering
\includegraphics[width=0.5\columnwidth]{pictures/example-utterances-1-cropped.pdf}
\caption{Example utterances (left) and corresponding authoring actions (right). One utterance may correspond to multiple authoring actions.}
\label{tab:examples}
\end{table}


\textbf{Editing Action Coverage}
\wy{To verify our taxonomy, we go through natural language-based visualization systems and multimodal visualization tools which include speech or text as input, including DataTone \cite{gao2015datatone}, FlowSense \cite{yu2019flowsense}, Analyza \cite{dhamdhere2017analyza}, Orko \cite{srinivasan2017orko}, DataBreeze \cite{srinivasan2020interweaving}, InChorus \cite{srinivasan2020inchorus}, and Valletto \cite{kassel2018valletto}. We collect 58 example utterances from the examples of these papers to examine the coverage of the framework. In total, 47 utterances can be covered. \todo{how we are more than them: how ambiguity operators are exist in the examples? how are these papers cover the taxonomy? further data analysis} The remaining examples that are not covered falls into the two categories: (1) The utterance expresses an intent of data analysis, instead of visualization construction. For example, while ``What is the relationship between unemployment and family income for those families earning more than 20000 and less than 150000 between 2007 and 2010 for California and Michigan?'' \cite{gao2015datatone} can be visualized with a scatter plot to show the correlations, it does not directly describe the editing operation. 
(2) The utterance describe the operations conducted directly to the graphical user interface. For example, the utterance ``Highlight the selected cars in a parallel coordinates plot'' \cite{yu2019flowsense} is aimed to highlight the cars selected from one chart on another chart. This helps users conduct analysis through multiple linked views. This category of operations is not covered by our framework.
}




\subsection{Implementation Guideline for the Framework}\label{sec:guideline}
\textbf{NL Interpreter}

Pros and cons**
**

\todo{what are the guidelines}

\textbf{Visualization Applications}
Visualization applications should implement an execution engine that processes the interpreted editing actions and executes the operations. If the operations are clearly specified, the execution engine blends the objects and calls the related functions. If the operation is not supported, the execution engine can return error messages to notice the users. If the operation is not supported but related operations are supported, the application can  further show simple examples to help users understand the functions of the system. When the actions are not fully specified, the application could predefine a set of rules to recommend proper actions for under specified utterances. 

The visualization applications should manage users' session and maintains a list of objects on canvas with corresponding attributes. If the objects are clearly referred, the application can simply looks for the objects and applies the operations to the target objects.
For objects with selectors, applications can traverse through the object list and finds out all the objects with specific parameters. If the objects cannot be resolved, the application could return error messages to notify users.

%\textbf{Resolving Vague Parameters}
% three types of vague parameters: 
% VisTalk implement a wide range of dynamic widgets to deal with 
% Dynamic Widgets 
% change value (text box, +/- buttons)
% change category (select box)
% change color (color panel)
% choose color theme (select box)
% position (select box; +/- buttons)
% modify content
%Next, we identify the parameters from the output. The intents produced by the NL interpreter contain four types of paramters, namely, exact parameters, under specified parameters, vague parameters, and relational parameters. 
There are three types of parameters, exact parameters, vague parameters, and relational parameters.
For exact parameters, we directly map the extracted parameters to the data value. We just check whether the value can be legally assigned. For example, `10px' for height can be simply assigned to the objects. 
%For under specified parameters, VisTalk implements a wide range of dynamic widgets. For example, if a user inputs a statement, ``change the bar color'', the system highlights the keyword ``color'' and popups a color selector. 
For vague parameters, VisTalk maintains a list of explanations to the vague parameters supported by the NL interpreter. Whenever users input a vague parameter, VisTalk lookups the descriptive parameters and finds the corresponding accurate value. For example, the parameter ``red'' yields the color code RGB(255, 0, 0). For ``high'' values, VisTalk infers it to the range (average, max).
For relational parameters, VisTalk also empirically maintains a set of predefined rules to adjust the value. For examples, ``on the top'' for ``put it on the top of the china bar'', means putting the item 10px away from the rectangle; ``make it bigger'', means increasing the size by 20\%. For relational parameters, VisTalk also highlights the parameters in the original utterances to enable users to do modifications through interactive widgets.



% \subsection{Reusable Chart Templates}
% export the charts as templates.
% Power BI





\section{Example Implementation}
To assess the design of our natural language framework, we build an a deep learning-based natural language interpreter that extracts operations, objects, and parameters and organized into a sequence of editing actions. Building upon this natural language interpreter, we build a proof-of-concept NL-based visualization authoring system in the form of VisTalk. 



\subsection{Natural Language Interpreter}
%We model the natural language processing module as the conversion from natural language to our predefined domain-specific language. To do this, we model conversion problem as a natural language understanding problem in natural language processing.
%We formulate this problem as a semantic parsing problem \todo{?} that takes human utterances as input, and outputs executable authoring actions. 
%As modeled in Section \ref{sec:model}, an input utterance may include multiple authoring action intents. 
%In the visual human-computer interaction, understanding human queries is really important. 
Natural language understanding is the core component of a natural language-based system. 
Usually, the understanding of natural language inputs takes two steps: first identifying users' intents in the utterances as functions; then extracting useful parts as parameters for the targeting functions. We design a multi-stage  natural language interpreter from natural language utterances to editing actions. First, we recognize data entities and outputs representations of utterance with data entities replaced with abstract arguments. After that, we design a deep learning-based natural language processing module that extracts intents and entities from the utterances \cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}.  Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy. We only need to add more sentences the training dataset to extend the capability of the NL interpreter.  Finally, the intents and entities are mapped to operations, objects, and parameters and organized into a sequence of editing actions. 

% The natural language interpreter bridges human utterances and authoring applications in a general way. For an input utterance, NL interpreter aims to translate it to  a sequence of editing actions that can be executed by visualization authoring applications. 


%To automatically understanding the input sentence and taking operations in the application accordingly, we need to firstly recognize the user’s entire intent. With obtained intent, we should further extract the useful parts in the sentence as references and parameters of the operation functions. 

%Therefore, to establish rules and analyze the syntax structure of the sentence is either complicated or low scalable. 
%Because the accuracy of these systems largely depends on the formulation of rules, the difficulty of maintaining a set of NL patterns and rules also substantially increased.
%If the input sentence is in a different form, we may have to add new rules to explain it. In addition, when the input is incomplete and ambiguous, it becomes harder to identify a set of NL patterns cover the input by rules. 
% Therefore, our example implementation of the natural language interpreter takes a deep learning-based method \cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}. Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy.
% We only need to add more sentences the training dataset to extend the capability of the NL interpreter. 
% This implementation of NL interpreter consists of three steps, namely, token recognition, authoring intent and entity extraction, and editing action synthesis. Rule-based methods can also be adopted for NL interpreter.  




\textbf{Token Recognition} Before the interpretation of user utterances, we recognize dataset-related entities in the utterance as the first step. These entities are table names, column names, and cell values in a table. The natural language interpreter is therefore aware of the data context. %For example, for a dataset ``CarSales.csv'', we identify data column names like ``Sales'' and ``Brand'', and data values like ``Ford'' and ``Honda'' in users' natural language utterances. To do this, we enumerate all the n-grams and check against the table entities in the input query in descending order of length. Once a k-gram is recognized (k may be different from n), we remove all the remaining n-grams that has overlapping parts with it. %We assign these entities as \textit{exact match} or \textit{partial match} of dataset entities for typo tolerance. 
After that, we replace these recognized tokens with abstract arguments like $<column>$, $<value>$ as input for the next stage. 
Further, we also link entities like number and date as special entities through similar ways. We assign numbers and dates into four categories: $<integer>$, $<float>$, $<date>$, and $<year>$.
This way, the difficulties and uncertainties of understanding the authoring intents can be reduced \cite{yu2018typesql, guo2019towards, dong2019data}. 
The token recognition phase outputs representations of user utterance with data entities replaced with abstract arguments.

\textbf{\wy{Intent and Entity Extraction}}
The purpose of this stage is to identify  \wy{objects and parameters} corresponding to the operations. They can be further organized into editing actions through a synthesis stage. An NL utterance for visualization authoring may involve multiple intents.
For instance, the sentence in Figure \ref{model_example} expresses four visualization authoring intents. Similar to NLP tasks such as semantic role labeling, sequence labeling, and named entity recognition, extracting objects and parameters in an utterance is actually a BIO tagging problem~\cite{ramshaw1999text}. In our task, we define the entities as the utterance parts which act as objects and parameters in editing actions. We create a series of labels following the BIO format to indicate the role of each utterance parts (Figure \ref{model_example}). We train a neural network-based model to recognize intents and entities from input utterances.  Rule-based methods can also be applied. Specifically, on the basis of the work of Liu \etal \cite{liu2016attention}, we design a joint model for intent detection and entity recognition based on encoder-decoder framework, attention mechanism \cite{vaswani2017attention}, and CRF algorithm\cite{lafferty2001conditional}. Through our neural model, the predicted intent tags and entity labels of each words can be obtained.

\begin{figure}[t]
\vspace{0px}
\centering
\includegraphics[width=0.5\linewidth]{pictures/labels.pdf}

\vspace{-1px}\caption{Intent tags and word labels of an example NL utterance. We regard color, chart type, y field (the data field bind to y axis), and x field (the data field bind to x axis) as entities in our model. Following the BIO (beginning, inside, outside) format\cite{ramshaw1999text}, we can map the words in the sentence into a sequence of labels, where B-, I-, and O represent begin, inside, and outside, respectively.}
\label{model_example}
\end{figure}


%The model takes user utterance as the input and recognizes its intent and entities. For example, in Figure \ref{model_example}, after passing through the token recognition module, the given sentence is fed into the neural model. We can obtain the predicted intent tag, \textit{SetChartType}, \textit{SetColor}, \textit{BindX}, \textit{BindY}, and entity labels of each words, O, O, B-Color, B-ChartType, I-ChartType , O, B-YField, O, B-XField.
%We implement a neural network-based model to recognize the intent and entities of the sentence. Compared with traditional rule-based models with syntax analysis and semantic analysis, neural network-based model is simpler to maintain \cite{chen-etal-2016-sentence, pasupat2015compositional}. It is also more scalable to new data because there is no requirement to make changes to existing rules or set more extra rules.
%Based on the modeling of authoring actions, we treat all the parameters and objects as entities in a NL utterance. Together with intents (operations), we organize entities (objects and parameters) into authoring actions.
% \begin{figure}[!t]
% \centering
% \includegraphics[width=\columnwidth]{pictures/model_arch2.pdf}
% \caption{The architecture of our model for intent and entity extraction.}
% \label{model_arch}
% \end{figure}
% As shown in Figure \ref{model_arch}, o

%Our deep learning model is based on encoder-decoder framework. Specifically, we employ Bi-LSTM\cite{hochreiter1997long} as the encoder and LSTM cell as the decoder\cite{liu2016attention}. \todo{remove this part but add the model figure?: In the encoder part, the input words are mapped into an embedding space and represented as vectors, which are used in decoder to generate the target output. At a time step $t$, we use the hidden state $H_t$ to represent the input word $x_t$. $H_t$ is obtained by concatenating $h_t$ and $h_t’$, the hidden states of forward and backward LSTM networks. The last state of the forward and backward LSTM network carries information of the entire sentence, so we concatenate $h_n$ and $h_n’$ as the intent vector of the whole sequence. The intent vector and word representations will then be sent into the decoder. } For intent recognition, due to the fact that a sentence may contain multiple intents, we predict the probability of all intents. If the probability of an intent is greater than 0.5, we consider it as one intent of the given utterance. For entity extraction, the attention mechanism is incorporated for better representation of each input word before determining the entity labels\cite{liu2016attention,vaswani2017attention}. To address the problem of inaccurate entity sequence prediction, we further apply Conditional Random Field (CRF) algorithm in the prediction process\cite{xu2013convolutional,zhang2016joint,huang2015bidirectional}, so that during tagging a word, we can adopt the previously labeled information and Viterbi algorithm to get the optimal entity sequence prediction. Finally, we extract the intention category and labels for all segments $Y = (y_1, ..., y_n)$. The parameters of the LSTM and CRF are jointly trained.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{pictures/interface.PNG}
    \caption{VisTalk interface (a). Users can type in their natural language utterances in the text box (b) to customize their visualization design (c). Users can author different charts at the same time (d). The table view shows the underlying dataset. The underlying dataset (e). 
    Users can click the words as interactive widgets to resolve ambiguities (f). The auto-completion panel pops out during the input process (g).
    }
    \label{fig:interface}
    \vspace{-5px}
\end{figure*}

\sherry{I feel the description of the dataset is still useful; The acc table, and some sample utterances?} \todo{discuss how to clarify the }
We collect a VisAuthoring dataset to train our model. It contains about 78K visualization authoring utterances, covering data operations, encoding operations, annotate operations, styling operations and view manipulations. As a first step, this dataset is composed of two main sources. First, we obtain the dataset by collecting more than 13K human-labeled natural language utterances \cite{zhong2017seq2sql, locascio2016neural}. Second, we manually induce a synchronous context-free grammar (SCFG) based on the human-labeled utterances and use the SCFG to synthesize the rest data \cite{jia2016data}. The dataset consists of natural language sentences and their corresponding intent tag, entity labels of each word in the sentences. %In total, there are \todo{31} kinds of intents, covering all the operation types. Additionally, there are \todo{32} kinds of entity tags, such as {B-mark.Mark, I-sort.Sort, B-unit.NumberUnit, B-text.String} and so on.
We evaluate our model performance on the VisAuthoring dataset. %Furthermore, to verify the generality of our model, we also conduct experiments on the ATIS dataset\cite{hemphill1990atis}. ATIS is the public benchmark dataset in natural language understanding, which has many characteristics of spoken language and is completely collected in the actual office environment. The results are shown in Table \ref{model_result}. 
\todo{term-based prediction accuracy. we have ~20 intents}
We assess from three aspects: intent accuracy, slot accuracy, and slot F1 score. The accuracy is 99.94\%, 99.74\%, and 99.74\%, respectively, showing that our model works quite well. %The performance results on ATIS are very close to the state-of-the-art results. Moreover, our model is more adaptive to visualization authoring tasks.


% \begin{table}[ht]
% \centering
% \begin{tabular}{p{2.5cm}<{\centering}|p{1.7cm}<{\centering}|p{1.7cm}<{\centering}}

% \toprule  %添加表格头部粗线
% Datasets & VisAuthoring & ATIS   \\
% \hline
% Intent Accuracy & 99.94 & 97.08  \\
% Slot Accuracy  & 99.74 & 97.59 \\
% Slot F1 Score & 99.74 & 97.60  \\

% \bottomrule %添加表格底部粗线
% \end{tabular}
% \vspace{2px}
% \caption{The performance of our model on VisAuthoring dataset and ATIS dataset. Intent accuracy represents the model performance in intent recognition, while slot accuracy and slot F1 score denote model performance in word role label detection.}
% \label{model_result}
% \end{table} 


\textbf{Editing Action Synthesis}
Given intents and entities, we then perform program synthesis to organize them into a sequence of editing actions. Editing actions consist of three parts, operation, objects, and parameters. For extracted intents and entities, the intents are mapped to operations, while the entities are mapped to objects and parameters. 

We synthesize editing actions by traversing the intent list. The intent obtained can be directly mapped to the operation types. Based on operation types, we can determine the corresponding objects and parameters. 
%The matching process works as follows: For each intent of an utterance, we traverse the extracted entity list one by one. We map the intent to an operation. If the entity belongs to the operation, it can be matched to the operation and directly filled into the object or parameter. Once an entity is successfully matched to an operation, we delete it from the entity list, which means each entity in the list can only belong to one operation. 
If there is no parameter or object for an operation, we fill it with a ``*'' mark, meaning the default state. After this process, we will obtain a list of editing actions.
%From remaining entities, there are two possible situations. One is that an intent is reused in the utterance. For example, in the case “change color of china and US bar to green and blue”, the entities “china” and “green” are left and haven’t been matched to any intent because the intent “change color” is reused. In this circumstance, we assume users specify the objects and parameters in order, so we fill the residual entities into the closest intent based on entity name and type. The other situation is that the residual entity exists as the selector of the object. For these cases, we check the list of objects and their supported properties, and fill the entity type and entity value into the selector of the object with proximity principle. If such matching object cannot be found, for example, users may only say ``red'' or ``bar'' as an utterance, then these entities are packaged one by one as editing actions without operations.
After getting a list of editing actions, we further rank them based on the category they belong to. Considering the operation types in the editing actions, we sort the editing actions from global operations, such as data operation, data encoding, view manipulation to local operations, such as changing the color, changing the title content.



==> sections/CHI_discussion-new.tex <==
\section{Discussion}
Below, we discuss implications from our user study observations, and potential directions to improve our work. By taking an one-interpreter-for-all schema, we alleviate the needs for users to get familiar with specific visualization concept models, and therefore lower the learning curve for users of different background. That said, instead of following specific visualization design paradigms~\cite{satyanarayan2019critical},  we avoid shaping users' mental model towards a specific editing process. However, unified interface with NL comes with challenges.

First, \textbf{it is challenging for the interpreter to account for users' different expressions with the same aims.}
Users that have different backgrounds, or are familiar with different visualization tools, can submit utterances that are too flexible to disambiguate.
Section~\ref{sec:model} enumerates the different visualization creation types: to create the chart from scratch, the utterances can be as high level as just mentioning the data columns (and the system is expected to automatically infer the chart type); 
It can also go as low-level as binding each specific mark channel (\eg rectangles) individually.
To achieve the seamless switch between these types, we need to build \emph{interpreters} that understand different commands.
Assuming we follow the deep learning approach as in our sample implementation, a crucial step would be to collect a diverse set of training utterances that express the same intent in various level of details.
This can be achieved by feeding crowd labelers with different \emph{visualization objectives}.
For example, users are more likely to say \sutt{sales by country} if we ask them to create a chart that inspect the correlation between ``sale'' and ``country'';
However, they may be intrigued to say \sutt{bind country to x-axis}, if we ask them to treat ``country'' as an independent factor in a series of analyses.
Alternative, we can diversify utterances by constraining them on \emph{construction workflows.}
In this case, we will ask expert users to write utterances, \emph{as if their utterances can only be parsed into a serial of actions of one specific construction workflows} (e.g., template editor, shelf-construction, or visual builders).
We can then further augment the dataset by paraphrasing these commands. 


Second, \textbf{users' more flexible NL inputs pose challenges for NL-based applications.} While the capability of parsing natural language utterances increases, our applications might be \emph{designed} to only focus on a subset of visualization creation and a editing actions. For example, how should a system react to \sutt{change the rectangle to circle}, if it only wants to support analytical interactions, and therefore does not allow mark customization? Would it disappoint people, if by design an application ignore more utterances than another tool, even when the interpreter parses it correctly? User studies on how users react to the boundary of applications is interesting. Alternatively, we can improve command recommendation, make suggestions to users when their utterance does not belong to the supported function type, and let people understand the scope of application functions.

Obviously, natural language is not always the best choice of input when conducting visualization editing. Other forms of input, such as speech, mouse, touch, pen, etc., could also be combined together to support more multimodal interactions, leveraging the strengths of one modality to complement the weaknesses of others. When the natural language interpreter takes the burdens of parsing utterances, it eases the difficulties of implementing and studying applications with natural language interactions. It can help visualization researchers better focus on the design and research on more natural interaction experience.

==> sections/CHI_discussion.tex <==
\section{Discussion}
\sherry{
This current discussion reads more like re-iterating many things we've already said before, e.g., editing actions as a bridge should be something section 3 already talked about extensively.
Some points I can think of:

\begin{compactenum}
\item Address the recommendation point in user study. Collect real world utterances to understand how people (with different backgrounds) give command in different tasks, different datasets, how to incorporate them into the framework.
\item Define finer-grained operation, so higher level operations can be a chain of lower-leveled ones, so we have a definitive set of operations (setChartType can be interpreted as xaxis, yaxis, etc.)
\item To help viz researchers better focus on the application part, release NL interpreters
\item Extension - more intents - can be more difficult to correctly parse the intents. Make use context to better understand users' intents 
\end{compactenum}
}
% \textbf{Editing Actions as a Bridge.}
% Due to the implementation challenges, prior natural language-based systems have to compromise the diversity and complexity of users' utterances.
% The design of natural language interpreter decouples the parsing tasks from the application that implements the commands. This method eases the difficulties of implementing natural language-based applications. NL-based authoring systems no longer need to implement a semantic parser themselves. Moreover, this also simplifies the maintenance of the natural language interpreter and improves the parsing performance. 
% %Our study of natural language-based authoring tools have demonstrated the effectiveness of using natural language to improve authoring experience. 

\wy{
\textbf{Understanding Utterances from People with Different Background}
From our user study, we find users may describe visualization design intents based on their own mental model of the design process. As mentioned in Section \ref{sec:model}, to create a chart from scratch, users can bind data columns to axes, so the chart type can be automatically inferred; users can start from a chart type and then modify the data fields, so the data binding and corresponding mark channels are obviously reflects; users can even start from a specification of mark (e.g., rectangle) and bind the data columns to different mark channels. To support better visualization creation experience, it might be interesting to understand different users' chart editing behaviors and the corresponding utterances. Editing actions can be further inferred more accurately. Moreover, the editing actions can be analyzed as sequences, so that users' follow-up editing actions can be predicted by the previous actions. 

\textbf{Visualization Design Paradigm.}
Visualization creating and authoring systems are usually designed based on different visualization conceptual models and design paradigms \cite{satyanarayan2019critical}. Users need to understand different design paradigms and get familiar with the user interfaces before making good use of authoring tools. 
However, different from WIMP systems, natural language authoring systems can provide a unified interface for different users. 
This makes the visualization creation experience more flexible and scalable. Expert users may easily switch between different mental models to optimize the process of creating typical chart, or more expressive visualizations. 
It also lowers the learning curve for users of different background. Novice users can start with basic chart and further modify and  customize the charts based on their needs.
However, this has poses new challenges for the implementation of such visualization creation tools to support seamless switch between different chart models. 
As future research, we consider to incorporate NL interpreter to multiple more advanced authoring systems to understand how the interpreters performs across different visualization systems.
}

% \textbf{Visualization Literacy}
% Users' behaviors towards natural language-based authoring systems may vary a lot based on their visualization literacy. Similar to the results of our formative study, the user study further confirms the differences among users with different background. Users with or without visualization expertise may have totally different mental models of creating charts \cite{}. However, natural language interfaces support unified interface for different users, which provides a better learnability. Users can simply switch among different creation process of visualizations.  



\wy{
\textbf{Designing Novel Visualization Tools to Support Multimodal Experiences.} 
The design of natural language interpreter decouples the parsing tasks from the application that implements the commands. This method eases the difficulties of implementing natural language-based applications. It may help visualization researchers better focus on the design of more natural interaction experience. 
In the future, we plan to collect more data on visualization editing and release the NL interpreters. This could lower the barriers of designing and developing novel natural language-based visualization construction techniques and tools.
For example, the authoring systems could design better experience for users to understand the vagueness and under-specification in their natural language input. It can also be challenging for users to understand system functions and how to describe their intents, a better natural language interaction experience should help users  enhance the recommendation of possible future actions to take.
Obviously, natural language is not always the best choice of input when conducting visualization editing. Other forms of input, such as speech, mouse, touch, pen, etc., could also be combined together to support more multimodal interactions, leveraging the strengths of one modality to complement the weaknesses of others. 
}
%One user (P9) learned to take advantage of the vagueness of natural language and said, ``When I am not sure what I want, I can try some vague descriptions and see what the system can give me. '' However, users also felt VisTalk interface gave them less sense of control. As P11 said, ``After getting used to the GUI interfaces, I am quite sure what will happen after I click one button. However, sometimes I am not sure what it turns out when I say a long sentences'' 

%\todo{for example, selector, fine-tuning can be conducted by mouse ... while users can use voice to state their requests}
%\cp{Users also mentioned that they wanted to have control of the precision of selections. In addition, we observed that users utilized the sliders to tweak effects. The sliders also served as a feedback mechanism for exploring the capabilities of the system (e.g., moving the slider swiftly back-and-forth between extremes)..}
%GUI - everything's in control. who's fault? judgement (fault notice/error message/let me know how to improve, or change)/Precision control




\textbf{Limitations.}
%- chart type-based (template based)
\sherry{This part is really implementation limitations, but as demonstrations they don't matter. I think we will want to discuss the potential limitations of frameworks, and how we want to address them in future work.}
\wy{More fine-grained taxonomy?}
As a first step, our current implementation of the natural language interpreter supports a set of common visualization operations. More operations can be included to support different visualization applications. Based on the deep learning model, the supporting operations can be expanded by extending the corpora with more users' utterances and the structured expressions corresponding to the functions of diverse visualization systems. Further enhancements are possible to cover more operations supported by popular authoring tools.
Similarly, the VisTalk prototype has a limited number of functions. VisTalk does make mistakes when encountering unfamiliar natural language patterns that are not covered in the training data. In the future, we plan to explore a method to automatically optimize the natural language model in the process of using the system. The system may learn from user inputs to improve its performance and the coverage of language patterns.

\todo{The current implementation binds table-related information before the intent and entity extraction. However, it may happen that data binding mistakenly bind tokens that are not related to tables. This method trades off the size of training dataset and improves the accuracy of the model for intent and entity extraction. In the future, we plan to collect a larger dataset and train a more robust end-to-end model. }

\wy{However, the capability of natural language understanding is still limited. %For example, the participants still hope to input more complex sentences that can help them process multiple table, or nested visualizations. This poses more challenges to understanding natural language. 
Our future research direction would involve more robust natural language interpreter that facilitate understanding of more complex utterances.}


==> sections/CHI_evaluation.tex <==

\textbf{Example Gallery}
To demonstrate the usability of VisTalk, we produce a variety of charts with example natural language utterances that specify the visualizations as shown in Figure \ref{fig:examples}. %Figure \ref{fig:examples} shows five examples from our gallery. 
These visualizations cover a wide range of operations that users may take in real world visualization authoring scenarios. 
The VisTalk system can enable the creation of basic charts with simple operations such as data operations, encoding operations, and annotate operations with natural language utterances.




% To demonstrate the usability of our VisTalk system, we produced a variety of charts, with example natural language utterances that specify the visualizations. Different natural language descriptions are also supported. 










\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{pictures/examples.pdf}
    \caption{Example visualizations authored in VisTalk with natural language utterances. (a) is based on a stock datatset, (b) and (e) are based on a car sales dataset, (c) is based on a shark attacks dataset, and (d) is based on a product sales data. The terms displayed in bold are column names in data, and the terms displayed in italic are values in data.%\todo{move this one to the supp?}
    }
    \label{fig:examples}
    \vspace{-2px}
\end{figure*}


















\subsection{Exploratory Study: How do Users Construct Visualizations with NLIs?}
With VisTalk at hand, we further conduct a user study to understand how users interact with visualization systems to construct visualizations through natural language.
%To understand how users can construct visualizations through natural language, we take advantage of VisTalk to conduct a user study. 
% To understand how users can produce expressive visualizations through VisTalk, we conduct a qualitative user study. Through the study we validate whether users are able to smoothly use natural language to create charts. Further, we aim to understand the advantages and disadvantages of natural language-based visualization authoring systems.
 We recruited 12 participants (3 female and 9 male, age ranging from 22 to 45) who had normal or corrected-to-normal vision. The participants include undergraduate and graduate students, data analysts, researchers, and software engineers. 
 %\sherry{do we need count per category?}
 They are general users who need to create visualizations to present data in daily work. All of the participants had used Excel to create charts before, while five of them had used Tableau or Power BI to create charts. %Two had experience in using design tools like Adobe Illustrator. 
% Two of them had experience employing natural language functions to do data exploration with general data visualization tools like Tableau and Power BI. 
% None of them had used advanced expressive visualization building tools like Charticulator \cite{Ren_2019_8440827}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, etc. All of them had used natural language agents like Siri, Alexa to complete simple tasks. 

\textbf{Study Procedure}
Our user study lasted for about one hour.
We first surveyed participants' background information with a questionnaire.
Next, we provided a tutorial outlining the features of VisTalk with two examples.
As a warm-up exercise, we encouraged them to freely explore the tool with one sample dataset.
Then, we provided the participants with \textbf{five visualization reproduction tasks}, ordered by complexity. 
These tasks included one basic bar chart, two charts with annotations, one pictograph, and one chart with multiple views. The most difficult tasks are similar to Figures \ref{fig:examples}d and \ref{fig:examples}e.
For each task, we displayed the target chart, described the underlying datasets, and asked participants to reproduce the chart in VisTalk using natural language utterances.
%When the participants are ready, they pressed a ``start button'' to load the dataset and begin the creation of the visualizations. When they finish each task, they pressed an ``end'' button. 
We observed the participants' interaction process and recorded the log of participants operation process.
Afterwards, participants rated their experience with VisTalk in the form of a five-point Likert
scale~\cite{likert1932technique}.
We further collected their free-form feedback through a semi-structured interview.


\begin{comment}
Afterwards, we confirmed the recorded observations with the participants, and they rated each observation by
the ease of discovery, relative to their prior experience working
with queries in the wild. Participants further self-assessed how
much more they learned about the dataset and the model, and
rated the usefulness of different components in Tempura (Q3).
All the ratings were collected in the form of five-point Likert
scale [24]. 

 First, we asked participants to fill out a pre-experiment questionnaire to collect their background information. Then, the participants received a 10-minute tutorial. In the tutorial, every participant watched a video that walks through two examples of using natural language to design a visualization. Then each of them is encouraged to have a quick try using the tools with one sample dataset to understand the features of the system.
 After that, we showed the five target charts and described the underlying datasets. When the participants are ready, they pressed a ``start button'' to load the dataset and begin the creation of the visualizations. When they finish each task, they pressed an ``end'' button. 
 Participants can ask the experimenter for help and clarification during the experiment. %\todo{We prepare a ``guide sheet'' to show them in case users cannot remember the operations and ask for help. To understand users' natural behavior of learning and using natural language systems, we do not provide the guidance by default.}
 We observed the participants' interaction process and recorded the log of participants operation process. After finishing the tasks, participants filled out a questionnaire about the experience. We conducted a semi-structured interview to further understand their overall impressions, difficulties they encountered, and other feedback and thoughts. 
% The study is carried out through web conferencing systems with participants sharing their screens with the experimenter.
% The participants join the study using a web browser on their own machines. Each session lasted for about one hour.   

% %\cp{To normalize expertise effects, we gave users one minute to do whatever they wished to accomplish for each task. After one minute, everyone received a “guide sheet” that showed them the operations for completing the task. For example, the guide sheet for a task could include the operations “brightness”, “sharpen”, and “vibrance.” Debrief. We debriefed the participants after they completed their tasks. We asked them for their overall impressions, the differences they encountered between the two types of interactions, and their overall feedback. In addition, we also asked the participants to complete a short questionnaire.}


% \subsection{Results}

% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=1\linewidth,height=130px]{pictures/sample.pdf}
% %     \caption{completion time}
% %     \label{fig:time}
% %     %\vspace{-10px}
% % \end{figure}
\end{comment}


\textbf{Results} 
All participants were able to use short and concise utterances to complete the tasks.
On average, they completed each task with $\mu=2.4$ utterances ($\sigma=1.26$) in around 139 seconds. 

Overall, participants rated the experience of using natural language to create visualizations highly ($\mu = 4.36, \sigma = 0.69$).
Compared with WIMP interfaces for chart creations, they preferred the natural language-based one because it is easy to learn.
%, and said they would recommend VisTalk to potential users.
Participants said that it is more straightforward to accomplish complex tasks with natural language, because it allows them to combine multiple chart manipulation intents within a simple sentence in the way that meets their needs. 
For example, users can simply say ``show Sales by Brand'' to complete the data retrieval and data encoding. One user (P3) commented, ``In the past I needed to search the menus and click the right buttons to perform the tasks. Sometimes it tales a long time to find the right menu item. Now I don't need to think about where they are.''






People tend to use short utterances for simple tasks, while longer utterances appear for more complex tasks.
For simple tasks, some users even tried to type keywords to see whether the systems can parse their intentions. 
For example, multiple users tried to use ``trendline'' or ``trend line'' to add a trend line to the line chart. In this example, the participant simply omitted the operations and parameters. This requires the system to automatically recognize the operations that can occur with the object ``trendline.''
When system attached a default trend line and the chart was updated, the participant said, ``It worked well. Natural language makes the thing easy.''


We also observed that some users failed to describe intents accurately. For example, when a user (P11) wanted to change the color of the charts, he typed ``highlight in blue'' and the system did not correctly execute the command because no object to highlight is provided. 
Some other participants also felt they could not express their requirements especially at the beginning of the tasks, P7 mentioned, ``Sometimes I forgot the exact words (e.g., trend line) to precisely describe my requirements.'' One participant (P4) opened search engine to look for a correct word. This indicates the importance of the design of the user interface to help users clarify their intents. The interface should also provide recommendations to give hints about potential choices that they can give commands.





%, from the perspectives of learnability (M = 4.5), ease of use (M = 4.25), effectiveness (M = 4.42), powerfulness (M = 3.83), productivity (M = 4.42), enjoyment (M = 4.67), and satisfaction (M=4.42). Figure \ref{fig:rating} lists the feedback of VisTalk. %Twelve and eleven users agree VisTalk is easy to learn and easy to use. Eleven users think VisTalk has improved their productivity. Twelve users felt satisfied. The feedback also reveals space of improvement. Our participants rated it relatively low in terms of the powerfulness of the system and the effectiveness of completing their jobs. It maybe helpful to design more functions and interactions for VisTalk for future work.



% %Number and complexity of utterances varied a lot from user to user. Some participants tend to use single intent statements. (this may caused by their experience of using other natural language tools), some other participants tend to use long and complex statements. (Average word count, max and min) (number of intents each sentence) We observed that all our participants successfully completed tasks purely with text input box alone, whether or not the examples are available to them. 
% %Some other participants rely more on the dynamic widgets to achieve their goals.


% \begin{figure}[!tbp]
%     %\vspace{px}
%     \centering
%     \includegraphics[width=0.8\linewidth]{pictures/ratings.pdf}
%     \caption{User ratings of VisTalk system with a 5-point Likert scale.\todo{delete this chart?}}
%     \label{fig:rating}
%     \vspace{-5px}
% \end{figure}


% \textbf{Qualitative Results}
%Our participants were overall have a very positive experience editing visualization with natural language. 


% %high efficiency
% The majority of participants (10/12) mentioned that the natural language interface saves their time and efforts. The majority of participants (8/12) said they will use natural language as their first choice if their familiar systems support similar functions. P9 said, ``To design a simple chart, using one simple sentence is enough. It is completely different from using mouse to select menus, select the data field from the dataset, specify chart types, and do further adjustments.'' Impressed by the parsing capability of VisTalk, P1 mentioned ``It is surprising that the system could perform correctly even when the sentence was very short and I misspelled some words and had grammatical errors.''

% %easy to learn 
% The participants (12/12) find the system interactions easy to learn even for those without much experience in visualization. One participants stated, ``I can quickly understand the effects of the commands.'' One of the participants who was not familiar with visualization creation tools said, ``Now I don't have motivations to learn to use traditional visualization tools. I will come to VisTalk if I need to create charts. It seems much easier to learn.'' P3 also mentioned, ``It is friendly to non-expert like me. I don't find difficulties of learning to use this tool. It gives me prompt feedback while I am typing and I feel I can complete the tasks easily. The overall experience is quite smooth.'' 

% %default recommendations can help 
% Although the chart recommendation functions are took simple strategies, many of our participants (7/12) mentioned the system recommendation is helpful. One participant said, ``The default charts were well-designed and I don't think I need to do further modifications.'' Three  participants mentioned they enjoyed using short phrases to interact with systems' default recommendations. P9 said, ``I am using these keywords to explore this system, similar to the experience of using search engines. I enjoy the way this system gives me surprises.''
% %discovery - cold start
% Although all of them got used to the natural language experience after a while. We find that cold start can be a problem for users that are not familiar with the system. This might because users are dim about how much the system could tolerate their vague or inaccurate expressions. To solve this problem, we believe more sufficient guidance and feedback can address this issue.

==> sections/CHI_introduction.tex <==

%NL interfaces are widely used
%however, different systems support different visaulization edit and authoring operations
%we propose a framework to decouple the nl understanding and application execution
% advantage: nl interpreter can be reused and easily extended
% we build example nl interpreter and application
% in the future, we will collect more data and release nl interpreter.



\section{Introduction}

Natural language (NL) interfaces are becoming mainstream for modern applications thanks to their usability and learnability.
%seek better usability and learnability by supporting natural language 
%and have attracted visualization researchers' attention. 
Compared with traditional interfaces with complex menu items and mouse interactions, natural language-based systems require less prior knowledge on user interfaces, and users are not restricted to the locations of menus and buttons~\cite{hoque2017applying, setlur2016eviza}. %Therefore, fewer efforts are taken for users to interpret their intentions into the system's allowed functions. 
%\sherry{Is ``visualization editing operations'' a well-defined term across the viz community? If not, we might need to add a one sentence description for it? Also, this phrase is making both sentences exceptionally long.}
\srevise{
Despite the benefit, the use of natural language interface has yet to be ubiquitous in visualization tools due to two challenges.

First, \emph{there has yet to be a comprehensive guidance on what interactions an NL interface should supply.}
Existing visualization tools that support natural language interfaces \cite{dhamdhere2017analyza, gao2015datatone, setlur2016eviza, yu2019flowsense, srinivasan2017natural} 
only cover subsets of visualization editing operations (mostly for visual analytics purposes).
As a result, a richer set of flexible data binding and visual configurations in modern visualization creating toolkits~\cite{bostock2011d3, satyanarayan2016vega} and authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} are largely ignored.
Conversely, to enable the use of natural languages in more scenarios, we need to first build a well-scoped set of ``operations-to-support.''
Second, with each tool following different design paradigms~\cite{satyanarayan2019critical}, \emph{it is challenging to consider the space of acceptable utterance per application.}
In other words, customizing NL interfaces for each visualization application can  take a significant amount of work.
That said, we note that the one-on-one mapping between the NL interface and the visualization tools may not be necessary.
While the low-level implementations are diverse, users' high-level intents of creating, editing, and authoring visualizations are largely shared across applications.
For example, users typically need to change the underlying dataset, specify visual encodings, and adjust visual presentations (e.g., axes, legends, marks, layouts).
As a result, if we can model such intents as an intermediate layer between the raw natural language and the visualization tool, we can easily supply multiple tools with one universal NL interface.
}



\begin{comment}
%%% new commented
Usually existing visualization tools that support natural language interfaces \cite{dhamdhere2017analyza, gao2015datatone, setlur2016eviza, yu2019flowsense, srinivasan2017natural} only cover subsets of visualization editing operations for visual analytics purposes, largely ignoring a richer set of flexible data binding and visual configurations in modern visualization creating toolkits~\cite{bostock2011d3, satyanarayan2016vega} and authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827}. Supporting this broader set of edit operations and enabling users to construct their visualizations with natural language may take a significant amount of work for each individual visualization tool.
\end{comment}
%Extending the existing NL-based systems to understand more operations through natural language, or enabling existing visualization tools to understand natural language, both requires great amount of efforts to design natural language understanding modules according the requirement of these tools.
%than traditional visualization tools. 
%Nevertheless, they involve complicated GUIs and incur a steep learning curve, especially for novice users. While natural language interfaces are promising in lowering the barrier of using advanced visualization authoring tools, unfortunately none of these systems currently support natural language interfaces.

%more flexible data binding and configurations for marks, layouts, annotations, and so on. Users can manipulate visualizations and graphical elements by pointing to the objects, finding configuration menus, and applying predefined functions.

%Contrary to the visualization analytics systems for data analysis, recent authoring systems \cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support more flexible data binding and configurations for marks, layouts, annotations, and so on. Users can manipulate visualizations and graphical elements by pointing to the objects, finding configuration menus, and applying predefined functions. %Theses systems support flexible and advanced authoring requests by direct manipulation of graphical elements and user menus. Users can point to the objects, find the configuration menus, and apply predefined functions carefully.  However,
%learning such complicated functions and adapt-ing to new user interfaces is often time-consuming and cumbersome,especially for novices.
%However, learning such complicated functions and adapting to new user interfaces is often time-consuming and cumbersome, especially for novices. Unfortunately, none of these systems support the usages of natural language.

% One major challenge of applying natural language interfaces for visualization authoring systems is the complexity of authoring operations. Various authoring systems may employ different visualization models and take notably different approaches to optimizing authoring interactions. A same authoring intent is defined as different internal functions across applications~\cite{satyanarayan2019critical}. \todo{very different cannot lead to the huge gap?}With a lack of a unified representation or grammar of visualization authoring intents, there is a huge gap to convert high-level natural language inputs from users to low-level authoring operations implemented by applications.


%One major challenge of applying natural language interfaces for visualization authoring systems is the huge gap between high-level natural language inputs from users and low-level authoring operations implemented by applications. Advanced authoring systems may employ notably different visualization models to optimize authoring interactions. A same authoring intent may be defined as different internal functions across applications~\cite{satyanarayan2019critical}. Without a widely-adopted representation or grammar of visualization authoring intents, it is difficult to model users' natural language authoring utterances.

\begin{comment}
%%% new commented
In fact, the one-on-one mapping between the NL interface and the visualization tools may not be necessary.
While the low-level implementations are diverse, users' high-level intents of creating, editing, and authoring visualizations are largely shared across applications.
For example, users typically need to change the underlying dataset, specify visual encodings, and adjust visual presentations (e.g., axes, legends, marks, layouts).
As a result, if we can model such intents as an intermediate layer between the raw natural language and the visualization tool, we can easily supply multiple tools with one universal NL interface.
\end{comment}

%While the low-level implementation of visualization tools and systems are diverse, users' intents of creating, editing, and authoring visualizations share a large set of overlaps across applications. 
%For example, users typically needs to change the underlying dataset, adjust visual encodings, and conduct changes on visualization styles of axes, legends, marks, layouts, and annotations.

\srevise{
Based on these observations, we propose a framework for building natural language-based visualization systems (Figure~\ref{fig:pipeline}). 
Our framework has two main goals:
First, to alleviate the burden of re-designing NL-interfaces per application, we \textbf{decouples the natural language understanding (with \emph{a natural language interpreter}) and visualization editing command execution (by a \emph{visualization application}).}
At the core of the framework is a set of \emph{editing actions}. 
These actions are machine-executable commands for modeling the aforementioned visualization editing intents.
They bridge users and visualization applications:
%These editing actions are pivotal and bridges users' NL utterances and applications' functions: \sherry{change authoring function to something else?}
the natural language interpreter parses users' utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.

Second, to provide a checklist on what user intents to support, we \textbf{explicitly categorize common \emph{editing operations} abased on extensive surveys on visualization construction tools.}
By doing so, we can map each authoring action maps users' editing intent can into well-defined \textit{editing operation} and its \textit{target objects}, and the corresponding \textit{parameters}.
\srevise{We validated our design by ensuring it is compatible with the utterances in existing NL-based visualization tools.}
}

\begin{comment}
%%% new comment
Based on these observations, we propose a framework for building natural language-based visualization systems (Figure~\ref{fig:pipeline}). 
It decouples the natural language understanding (with \emph{a natural language interpreter}) and visualization editing command execution (by a \emph{visualization application}). 
At the core of the framework is a set of \emph{editing actions}. 
%\wy{After surveying a number of visualization construction tools, we define editing actions as the combination of operations, objects, and parameters. }
These actions are machine-executable commands for modeling the aforementioned visualization editing intents.
They bridge users and visualization applications:
%These editing actions are pivotal and bridges users' NL utterances and applications' functions: \sherry{change authoring function to something else?}
the natural language interpreter parses users' utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.
%explore the usage of natural language interfaces for visualization authoring systems. 
%We design a natural language-based authoring framework with a natural language interpreter that can parse users' utterances into a sequence of authoring actions. 
%, which are used as an abstract layer to bridge users' utterances and different authoring applications. 
\end{comment}


%\sherry{I moved/rephrased the first half of this paragraph above, but dont know what to do with the second part. I think we can just cut it? I assume because you cut some additional model stuff, ``first step'' doesn't make sense anymore; Plus for short paper we don't need to go into such detail?}
%We summarize common editing interactions and formulate them into \textit{editing actions} in the forms of operation, objects, and parameters to model natural language intents into machine-executable commands. As a first step, we summarize the most common authoring operations and categorize them into six major groups, namely data operations, encoding operations, annotate operations, styling operations, layout operations, and view manipulations. 

%On the top of the model, we design a deep learning-based natural language interpreter that parses users' utterances into a list of authoring actions, which can be further adapted and executed by authoring applications. 
%Authoring actions can be further adapted and executed by authoring applications' internal functions.
%This could result in different experiences of using natural language to describe authoring requirements, which may confuse users and decrease the learnability of natural language-based authoring systems.
As a proof-of-concept, we implement a sample interpreter and a prototype application:
The interpreter takes the form of a deep sequence labeling model, trained on a dataset that contains internally collected user intents, as well as synthetic augmentations.
The prototype, VisTalk, supports natural language-based visualization authoring by integrating the interpreter.
%To assess our framework, we implement a deep-learning based natural language interpreter. The NL interpreter takes an NL utterance as input and ouputs a sequence of authoring actions.
%The interpreter can be integrated by different authoring tools to bring in natural language capabilities. 
%Further, we build a prototype application, VisTalk, which integrates the NL interpreter to support natural language-based visualization authoring. 
\srevise{
With VisTalk, we highlighted key factors to consider when implementing interpreters and applications, and demonstrated possible solutions of executing authoring actions and resolving the ambiguities in NL inputs. 
We further used VisTalk in an exploratory user study, where participants completed visualization reconstruction tasks with natural utterances.
Our observations shed light on future work:
We should consider how the interpreters can cope with users with different backgrounds, and how the applications can make recommendations when users' initial command is not supported.
}
The contributions of this work are summarized as follows:





\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\columnwidth]{pictures/workflow-new.pdf}
    \vspace{-10px}
    \caption{NL-based visualization construction framework. }
    \label{fig:pipeline}
    \vspace{-10px}
\end{figure}




%We leverage VisTalk to conduct a user study to understand the effectiveness of natural language-based authoring systems. Our results confirm the effectiveness of natural language-based authoring for novice users. The study also reveals space of improvement for future research on natural language-based visualization authoring systems.

\begin{compactitem}
    \item We summarize and formulate users' intents as \textit{editing actions}, which are atomic units executable by applications. The introduction of such pivotal editing actions helps bridge the gap between natural languages and visualization applications.
    \item We propose an NL-based visualization editing framework that is equipped with a natural language interpreter to parse NL utterances into editing actions, and an authoring application to execute the editing actions.
    \item To illustrate the usage of the framework, we implement an example natural language interpreter that consists of three stages: data entry abstraction, information extraction, and editing action synthesis. We further build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. 
\end{compactitem} 






















% %with rule-based methods, which can be hard to generalize. 
% %Modern authoring tools however require the support of much more abundant and complex functions. The intents from human users can thus be more complex and diverse. This poses new challenges for the design of natural language tools. 



% % {\fontfamily{helveticaneue}\selectfont \{place, legend, position=[plot]right\}}\\
% % {\fontfamily{helvet}\selectfont \{place, legend, position=[plot]right\}}\\
% % {\fontfamily{lmss}\selectfont \{place, legend, position=[plot]right\}}

% %Visualization becomes increasingly popular for storytelling. There are growing interests of create visualization for communication and presentation. 
% A number of visualization authoring systems have emerged to enable the authoring of expressive visualizations. Contrary to the traditional visualization systems for data analysis, recent visualization authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support more flexible data binding and configurations for marks, layouts, annotations, and so on. 
% %\todo{how complex are the authoring operation?}
% %For example, data-driven guides \cite{Kim_2017_7536218}, DataInk \cite{xia2018dataink}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909} support data binding with hand-drawn or vector shapes; %InfoNice \cite{Wang:2018:IEC:3173574.3173909} enables the creation of expressive visualizations through mark customization; 
% %Data illustrator \cite{Liu:2018:DIA:3173574.3173697} proposes repeat and partition features for creative design of visualizations.
% These systems support flexible and advanced authoring requests by direct manipulation of graphical elements and user menus. Users can point to the objects, find the configuration menus, and apply predefined functions carefully. However, learning such complicated functions and adapting to new user interfaces is often time-consuming and cumbersome, especially for novices. 
% %Mouse and touch interaction can also be inefficient for complex visualization design%, especially when the interfaces themselves are also complex
% %\cite{hoque2017applying}. 
% %There are many barriers to learning and adapting to new user interfaces especially for novices.
% %However, they have restricted the target users to "graphic designers". General users without visualization design knowledge are hard to understand visual encoding. InfoNice adopts a "mark customization" approach. However, ...Users still need to learn and get familiar with the interface to implement their design. 

% %As a promising interaction paradigm, natural language has the potential to offer advantages to address these issues. 
% In contrast, natural language interfaces have attracted researchers' attention thanks to its learnability and usability. Compared with traditional interfaces with complex --- but sometimes still insufficient --- menu and mouse interactions~\cite{hoque2017applying}, natural language-based systems require less prior knowledge \cite{setlur2016eviza}. Users are not restricted to the functions and locations of the buttons. Therefore, fewer efforts are taken for users to interpret their intentions into the system's allowed functions. Researchers have conducted research on natural language interfaces for visual analytics \cite{dhamdhere2017analyza, gao2015datatone, yu2019flowsense}. 
% However, most of them focus on visual data exploration and support basic natural language data query with rule-based methods, which can be hard to generalize. 
% Modern authoring tools however require the support of much more abundant and complex functions. The intents from human users can thus be more complex and diverse. This poses new challenges for the design of natural language tools. 
% %support the natural language module by NL-based data query. 

% To fill this gap, we explore the usage of natural language interfaces for visualization authoring systems. 
% Prior work of authoring tools have emerged to provide powerful authoring interactions for users. However, 
% these systems take notably different approaches to optimizing authoring interactions and ease the creation of expressive visualizations \cite{satyanarayan2019critical}. With different menus and interactions, authoring operations are defined as different internal functions across applications. This could result in different experiences of using natural language to describe authoring requirements, which may confuse users and decrease the learnability of natural language-based authoring systems.
% %difficulties of natural language interactions. For instance, the same keyword ``highlight'' may result in different interpretation for different platforms, 


% In response, we explore a natural language-based authoring framework
% with a unified authoring action grammar. To achieve this, we conduct a formative study to understand how users might express their authoring intents. %There are three main findings from the study. First, users might use different workflows for different types of authoring scenarios. Second, natural language utterances may contain fuzzy reference and vague modifiers for parameters. Third, users tend to mix multiple intents in one sentence. 
% Based on the study, we formulate common authoring features into authoring actions in the form of operation, object, and parameter to model natural language intents into machine-executable commands. As a first step, we list most common authoring operations and categorize them into six major groups.  
% %On the top of the model, we design a deep learning-based natural language interpreter that parses users' utterances into a list of authoring actions, which can be further adapted and executed by authoring applications. 
% Authoring actions can be further adapted and executed by authoring applications. 
% The authoring actions are used as an abstract layer to bridge users' utterances and different authoring applications.

% We implement an natural language interpreter with a deep learning-based model, that takes human utterances as input and ouputs a sequence of authoring actions. The interpreter can be integrated by different authoring systems to bring in natural language interfaces. Authoring systems can adapt and execute authoring actions with local authoring functions.  This
% helps enhance the capability of natural language understanding for authoring tools. For users especially novices, this approach reduces the barriers of learning and using visualization authoring systems for different users across applications. %The framework takes natural language as input and parses users' utterances through the natural language interpreter and outputs a list of \textit{authoring actions}. The output can be further executed by visualization authoring systems to respond to users' input and make changes to the visualizations.



% % To evaluate our framework, 
% % We then conducted user study to understand how users interact with the NL-based visualization authoring system.
% % Through our study, we show the benefits and pitfalls of using NL-based method for visualization authoring.

% To assess this framework, we build an example web authoring system, VisTalk, based on the natural language interpreter. We demonstrate the possible ways of executing authoring actions and resolve ambiguities in users' natural language inputs.
% Further, we leverage VisTalk to conduct a user study to understand the effectiveness of natural language-based authoring systems. Results reveal the benefits and weaknesses of VisTalk \todo{expand a bit}, inspiring future research directions for natural language-based authoring systems.
% %Users need to practice using the GUIs to accelerate their design process.
% %Drawbacks for the GUI for visualization authoring systems:
% %Users need to learn the different design process/logic behind the system one by one The GUI changes significantly across systems to support different user groups/needs. As a result, users need to switch between tools, learn different interface when they have different needs
% %In this paper, we explore a natural language framework for Visualization authoring. 
% The contributions of this work are summarized as follows:
% \begin{compactitem}
%     \item We conduct a formative study on how users express their visualization authoring intents with natural language. We summarize and formulate authoring intents as \textit{authoring actions}, which are atomic units executable by applications, to bridge the gap between natural languages and authoring applications.
%     \item We build a deep learning-based natural language interpreter to parse from their input utterances into authoring actions. The natural language interpreter consists of three stage, token recognition, intent and entity extraction, authoring action synthesis.
%     \item To illustrate the usage of the framework, we build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. With this system, we conducted a user study to understand the effectiveness of NL-based authoring experience. 
% \end{compactitem} 




==> sections/CHI_nl-interpreter.tex <==
\section{NL-based Visualization Framework}
We consider the design of our natural language framework against the following requirements: 
(1) Reusability: the framework should be reusable for common visualization construction and configuration intents, and support different visualization applications; 
(2) Extensibility: it should be easy to extend to cover more visualization commands and the capability can be improved over time; and
(3) Flexibility: it should support flexible natural language input with vague descriptions.

Based on these considerations, we introduce our natural language-based visualization editing framework (Figure \ref{fig:pipeline}). 
The framework consists of two parts, a \textbf{natural language interpreter} and a \textbf{visualization application}. 
When a user inputs a natural language sentence, the interpreter parses it into \textbf{editing actions} and sends the actions to the application. 
The editing actions are a list of structured descriptions of users' intents and can be executed by the application. We also provide design guidelines of visualization applications based on the NL interpreter.

%We design a natural language interpreter that parses human utterances to visualization editing actions and can be applied across different editing tools. %\sherry{First sentence is a bit duplicated with the last paragraph; And I think this paragraph needs a rewrite.}
% We model users' visualization editing intents as \textit{editing actions} and formulate an editing action as the combination of \textit{operation}, \textit{objects}, and \textit{parameters}. We summarize and categorize common editing actions into six categories that cover visualization editing functions in editing tools. 
%Users' natural utterances can be parsed into editing actions and passed to applications to execute. 
%First, we define a domain-specific language (DSL) of visualization editing, covering common operations for visualization editing from 6 aspects. 
%The natural language processing module takes users' utterances as input, and outputs the program in the form of our DSL. The code can be further parsed and implemented by specific applications or code libraries to complete the specific tasks under different design environments.


\subsection{Editing Actions}\label{sec:model}
% These visualization construction tools can be divided into three categories~\cite{satyanarayan2019critical}. 
% Tools like Microsoft Excel supports \textit{template editor} style, where users may start with a chart type and further make extensive customization. 
% Users may say \sutt{Give me a bar chart for \textit{Sales} by \textit{Country}} for a bar chart with y-axis encoded with Sales and x-axis encoded with different countries.  
% Tools like Tableau, Voyager \cite{Wongsuphasawat2017Voyager2A} constructs visualizations by mapping data fields to encoding channels (e.g., x, y, color, shape). 
% An example utterance can be \sutt{Bind \textit{Sales} to y-axis} and \sutt{Bind \textit{Country} to x-axis}. 
% The tools might further automatically recommend rectangles as marks. 
% Tools like Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909}, construct visualizations from the fine control of marks, glyphs, coordinate systems, and layouts. 
% Users might start with \sutt{draw a rectangle}, and then, \sutt{repeat it horizontally on \textit{Country}}, and finally \sutt{bind height to \textit{Sales}} to construct a similar bar chart. 
% Therefore, to fit into these  different styles of visualization tools flexibly, we propose the notion of editing action as the combination of operation, object, and parameters, where users' editing intents can be simplified as \textit{editing operation} and its \textit{target objects}, and the corresponding \textit{parameters}. 

%We define \textit{editing actions} as the combination of editing \textit{\color{cop}operations}, \textit{\color{cobj}objects}, and \textit{\color{cpar}parameters}. User utterances can be mapped to one or multiple editing actions. The editing process of visualization is the execution of a sequence of editing actions. Formally, an editing intention can be defined as a triple:


Various systems have covered a wide range of functions to enable the composition of both standard charts and highly customized interactive visualizations. 
However, there was no common design model that can let us consistently describe visualization editing intents~\cite{satyanarayan2019critical}.
In response, we survey the functions of modern interactive visualization systems to unify the intent description.

Visualization construction tools can be divided into three categories~\cite{satyanarayan2019critical}, namely, template editor, shelf-construction, and visual builders. Following this taxonomy, we examine the functions support by these three types of systems that are accessible as commercial products or online demos, including Microsoft Excel, Tableau, Voyager \cite{Wongsuphasawat2017Voyager2A}, Data Illustrator~\cite{Liu:2018:DIA:3173574.3173697}, ChartAccent~\cite{ren2017chartaccent}, Charticulator~\cite{Ren_2019_8440827}, and InfoNice~\cite{Wang:2018:IEC:3173574.3173909}. We document the editing actions involved in creating and editing visualization designs with these systems. The editing actions are collected from the tools' official introduction websites and third-party online tutorials.
Each of the categories prioritizes different construction workflows: 
(1) In \textit{template editor} tools like Microsoft Excel, users frequently start with high level command query on template charts before making further extensive customization.
These commands omit details on visualization channels, and instead stress chart types and targeted data entries.
For example, to query a bar chart with y-axis encoded with Sales and x-axis encoded with different countries from these tools, the most natural driving utterance might be \sutt{Give me a bar chart for \textit{Sales} by \textit{Country}} for a bar chart.
(2) Tools supporting \emph{shelf-construction} (e.g., Tableau\footnote{\url{https://www.tableau.com/}}, Voyager~\cite{Wongsuphasawat2017Voyager2A}) constructs visualizations by mapping data fields to encoding channels (e.g., x, y, color, shape). 
To construct the same example above, the utterance that best aligns with these tools would be \sutt{Bind \textit{Sales} to y-axis} and \sutt{Bind \textit{Country} to x-axis}. 
%The tools might further automatically recommend rectangles as marks. 
(3) \emph{Visual builders} tools like Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909}
 construct visualizations from the fine control of marks, glyphs, coordinate systems, and layouts. 
Users might start with \sutt{draw a rectangle}, and then, \sutt{repeat it horizontally on \textit{Country}}, and finally \sutt{bind height to \textit{Sales}} to construct a similar bar chart. 

Comparing across the aforementioned visualization editing actions, 
we make two observations:
(1) The level of editing intent vary greatly, from single element editing to integrated construction; and (2) despite the varying intents, the core data entries remain present in all utterances.
To fit into these different styles of visualization tools flexibly, we propose the notion of an editing action as the combination of \textit{\color{cop}operations}, \textit{\color{cobj}objects}, and \textit{\color{cpar}parameters}:
\begin{equation*}
    \texttt{editing~action := \sact{operation}{objects}{parameters}}
\end{equation*}

%The definition of the editing action describes the actions the editings want to take to the visualizations.  
The \textit{\color{cop}operation} identifies the type of editing intent (e.g., \sutt{change color}, \sutt{add annotation}). The \textit{\color{cobj}objects} are the targets that the operation applies to, such as the canvas area, the bars in a bar chart, the title text,etc. Finally, the \textit{\color{cpar}parameters} indicate the degree or configurations of the operations.
Figure \ref{fig:taxonomy} lists the operations and the corresponding target objects and possible parameters, and we describe them in detail below.



\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{pictures/exampleActions.pdf}
    \vspace{0px}
    \caption{An utterance can be mapped into a series of editing actions.  An editing action consists of three parts, operation, object, and parameter.The examples show the usages of object selector, vague parameters, and relational parameters.}
    \label{fig:taxonomy}
    \vspace{-1px}
\end{figure*}


% \begin{table*}[!t]
%     \centering
%     \includegraphics[width=1\linewidth]{pictures/new-taxonomy-cropped.pdf}
%     \vspace{0px}
%     \caption{An editing action consists of three parts, operation, object, and parameter.  Operation are categorized into six major groups. Objects are categorized into chart components (e.g., axes, legends, title), mark channels (e.g., shape, color, size, position), and annotations (e.g., reference lines, reference bands, trend lines). \todo{remove this table and replace with a simpler image}}
%     \label{fig:taxonomy}
%     \vspace{-1px}
% \end{table*}

\subsubsection{Operations}
%Our framework models the action of users' editing requests as a sequence of operations %. %The basic operations are primitive operations (e.g., data binding, change color, change font, etc.). More complex operations can be combined with multiple primitive operations and are used to complete typical design tasks. For example, ``turn the bar chart to a pictograph.'' \todo{how to} %All the operations require target objects (e.g., axes, marks) and parameters. 
%Based on existing visualization editing systems and taxonomies \cite{satyanarayan2016vega, Ren_2019_8440827, Liu:2018:DIA:3173574.3173697, Wang:2018:IEC:3173574.3173909, ren2017chartaccent}, 
%The most primitive operations that appear in visualization editing tools 
%and 
%We categorize editing operation into six major groups.
%, namely, data operations, visual encoding operations, layout operations, styling operations, view manipulations, and annotate operations.\todo{no need to list the names of the categories since they will be listed below...} 
%Different o

%We list common editing actions that are used in visualization editing.
% \begin{compactitem}
%     \item \textbf{General operations}, like \textit{add}, \textit{remove}, \textit{copy}, are the operations that can be acted upon any object, including graphical elements (e.g., add an annotation) or data encoding (e.g., remove a filter).
%     \item \textbf{Data encoding} is the mapping between data and visual channels.
%     \item \textbf{Data transform} are the operations that are related to data query and calculation, such as \textit{select}, \textit{filter}, \textit{pivot}, and \textit{join}.
%     \item \textbf{Selectors} are the operations that are applied to the objects with visual properties, such as \textit{change color}, \textit{modify shape}. For example, users can change the color of the title; or change the color scheme for the marks in a chart. Users may even replace the marks with icons for expressive visualization design.
%     \item \textbf{Numerical operators} are the operations that are related to the numerical properties of objects. Change range, of something. For example, change the height and width.
%     \item \textbf{layout operators} are a special type of numerical operators that can be widely used for expressive visualization designs. Users may add labels, annotations, and configure the positions of them. They may \textit{move} up or left, \textit{change position} to a specific point, or even \textit{adjust z-order} for the graphical elements.
%     \item \textbf{Text operators} include the operations that are specifically related to text. For example, users may \textit{modify content} of titles, or \textit{change font} for the annotations.
% \end{compactitem}
% \begin{compactitem}
%     \item \textbf{Bind} is the mapping between data and visual channels; data transformation and data fields; data transformation and visual channels 
%     \item \textbf{Add/Remove/Modify} can be applied to graphical element on a visualization design. For example, ``add the legend'', ``modify the title''. They can also be applied to data encoding, such as ``add a filter''.
%     \item \textbf{Set value} is applicable to any object with numerical properties, such as size, height, opacity, etc. 
%     \item \textbf{Change category} is used for the visualization objects with only discrete value properties.
%     \item \textbf{Color} is a special, color related, color scheme 
%     \item \textbf{Font} font style
%     \item \textbf{Style}
%     \item \textbf{Place} (move, position)
% \end{compactitem}
%The operations are categorized by visual features of the target objects. 
%In a visualization design, different visual components may have different properties. These properties further specify the variables that characterize the target components. For example, encoding supports different encoding channels such as position(x, y), size, and color. Marks have properties including shape, color, etc. The shapes for marks are rectangles for bar charts, circles for bubble charts, symbols for scatter plots, etc. The properties for marks also depend on the implementation of the charts. For example, a more flexible editing tool may support users to replace the basic geometric shapes with icons, or even images. Following the implementation of existing editing systems, 

%Operations may apply to different objects, depending on the properties of the objects. 
%As discussed previously, operations are not exclusive because different tools support different design paradigm and human languages also express same meanings with different patterns. 
%For example, \sutt{bind a data field to x axis}, has the same effect as \sutt{encode the horizontal position of mark to the field.}

We summarize the editing operations by going through the category of Vega-Lite grammar~\cite{satyanarayan2016vega}, from which we collect a large number of visualization operations related to \textit{data, encoding, and mark}.
To support the construction of more expressive visualizations, we further include common styling operations, and collect operations from ChartAccent \cite{ren2017chartaccent}, Charticulator \cite{Ren_2019_8440827}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909} to develop three more categories related to \textit{layout, styling, and annotation}. We summarize six main categories of operations:
\begin{compactitem}
    \item \textbf{Data operations} are the operations that retrieve and calculate data from datasets. Typical operations include filter, aggregate, bin, set time unit, and sort.  
    \item \textbf{Encoding operations} are the operations that bind data fields to different encoding channels. Users may also take operations to the axes or directly assign chart types to specify encoding.%, while the effects might be the same. %For example, ``bind Country to x axis'' and ``bind Country to the horizontal position of marks'' have different objects (i.e., x axis and position), while they have the same effects. 
    \item \textbf{Mark operations} include the configurations related to the configuration of marks. Users may change the shape, color, style of marks. The types of mark can be vector shapes, text, images, icons, etc. 
    \item \textbf{Layout operations} include the configurations related to position and offsets of chart elements, such as title, annotation, legend. Users can place an object at a designated position, or move it along a direction.
    \item \textbf{Styling operations} includes graphical operations and textual operations. Graphical operations are performed to color, size, shape, icon, and stroke of graphical elements, such ass axis lines, marks, reference line, etc. Textual operations are acted to text-related properties such as font (size, color, style, weight), content. They can be applied to title, labels, annotations, etc.
    %\item \textbf{View manipulation} refers to operations that create one visualization with multiple views. Chart views can be created into multiple or layered displays. %Multiple views can also be created by ``faceting'' the current view by one data column (e.g., facet the sales by country) or ``repeating'' one chart view to other data values (e.g., repeat the sales chart for US and Japan). 
    \item \textbf{Annotate operations} manipulate annotations (e.g., text, labels, embellishments) that enhance the charts. Annotations can be bound with data. For example, trend lines can show the trend between two time points. Common types of annotations include labels, annotation text, reference line/band, trend line, average line, etc.
    %can show aggregated values by the marks\todo{do we have the corresponding operation for adding labels?} . 
\end{compactitem}



%Based on these operations, more complex high-level operations can be combined. For example, "change the style" usually means the combination of graphic properties and textual properties. This may even apply to the color coding of the marks, further impacting data encoding properties. ``Sales by year'' usually means create a chart, bind x axis with Sales, and bind y axis with Year.

% \begin{compactitem}
%     \item \textbf{Change Chart} removes the current chart encoding and applys new encoding to change the chart into a new one.
%     %ll\item \textbf{Repeat and partition}  
%     \item \textbf{View composition} (facets) applies all the settings and further modifys the data encoding properties.
%     \item \textbf{Fill percentage} adds a background icon with the same foreground icon but different colors.
%     \item \textbf{Interaction} specifies different sets of properties based on users' interaction conditions. Users need to specify the condition and the effects of the interactions.
% \end{compactitem}




\subsubsection{Objects}
Objects are the components that operations target. 
%For an editing operation, users usually need to specify the targeting object they want to create, modify, or remove. 
In WIMP (Window, Icon, Menu, Pointing) interfaces, users usually click on the menus or select the targeting objects on canvas. For a natural language environment, users need to specify objects through NL utterances.
For basic visual charts, the objects include the marks, axes, titles, legends, gridlines, etc. More advanced objects include annotations such as trend lines, reference lines, reference bands, text annotations, and embellishments.  

The objects correspond to different operations. For example, the objects of \textit{data operations} include data fields, data points, data type, data range etc. The objects of \textit{encoding operations} include the data fields, chart components such as axes, legends, title, and mark channels such as mark size, mark shape, mark position. The objects of \textit{styling operations} include visual properties such as opacity, stroke, text font, text color, and so on.
% \wy{\begin{compactitem}
%     \item \textbf{Data/Datasets} include data fields, data points, data type, data range etc. When users conduct data operations, they need to assign parameters to these objects.
%     \item \textbf{Chart Components} are the basic parts of charts. This category includes plot area, axes, legends, title, etc.
%     \item \textbf{Mark channels} are targeted by encoding operations. Users need to encode data fields with different channels of marks, such as mark shape, mark color, and mark size.  
%     \item \textbf{Annotations} are additional graphical or textual elements to the charts. Annotations can be bound with data value or data points. For example, reference lines, reference bands are directed related to data; text annotations, image annotations can be placed near one certain data point; data labels can be shown at near each data point to show the values.
%     \item \textbf{Configs} are the properties of visual elements that styling operations take effects, including text font, stoke, opacity, width, and so on.
%     \item \textbf{Layout} are position-related visual properties. Users may need to change position, alignment, offset, z-index of the elements when position is not encoded with data.
% \end{compactitem}
% }

The objects in an editing action can be under-specified. For example, a user may say \sutt{give me a chart} after uploading a dataset. An intelligent system can recommend a best encoding to users, or ask users to clarify the command.
We directly model users' intent and use a special notation \texttt{``*''} to represent  the under specified objects. The implementation of visualization systems can further decide definite reference strategies.

%Clearly, a target component may support more than one target operations\todo{???}. %A mark may simultaneously support encoding operations and styling operations. 

% To describe an editing operation, users usually need to specify the targeting object they want to create, modify, or remove. 
% In graphical user interface systems, users usually click on the menus, or select the targeting objects on visualization canvas. For natural language environment, users need to specify the objects through their utterances.

% \textbf{Objects} are the components that the operations targeted to. For example, for a basic visual chart, the components include marks, axes, title, legend, encoding, etc. editing tools for standard charts usually only support limited number of target properties. Supported components can further include annotations such as trend line, reference line, text annotations, etc., depending on the implementation of different editing tools.  
% Clearly, a target component may support more than one target properties. An implementation of visualization mark may simultaneously support general properties, graphic properties, and data encoding properties. 
% For example, the rectangles in a bar chart can be configured to different color and widths. The rectangle mark can also be replaced with other shapes to reach expressive visualization designs. While different target properties are handled by corresponding operations. The parameters further configure how to change these objects. 

%Once users obtain a chart, they may further say ``turn it to red''. The systems may infer the intention of the users is ``turn the marks to red''. We 

\textbf{Object Selectors.}
Users show special patterns when referring to objects with natural language. 
They may refer to objects through \textit{object properties} \cite{hoque2017applying}. 
%For example, users may ask the system to ``turn the red line blue'', which means ``turn the line in red color to blue color''. Therefore, w
We support an object selector for users to filter the objects. For example, the intention \sutt{turn the red line blue}  does not directly specify the object because there is no component named ``red line''. %The ``red line'' can be selected as \texttt{[shape=line,~ color=red]}, 
It can be presented as \sobj{[shape=line,color=red]}, meaning to select objects with the properties ``line'' and ``red''. 
%The similar pattern can also be applied if visualization components are clearly referred to, but users would like to select parts of them. For example, ``add black stroke to the blue bar'' for a colored bar chart can be translated to \texttt{setStroke, [shape=bar, color=blue], color=black])\}}, meaning users wants to change the style of the mark with blue color and the operation is \texttt{setStroke}. 
The properties that users describe should exist in the predefined library of property and parameters. Otherwise, the natural language interpreter may not be able to match them. If the properties do not exist, we refer to the unknown properties with``*'' and leave quotation marks to the text phrases. %Further, the natural language interpreter may not be able to understand the attribute type and leave a star mark as placeholder. Applications may further parse the attributes based on the context of editing.
For example, ``add black stroke to the abc bar'' can be translated to 
\sact{setStroke}{[shape=bar,*=``abc'']}{stroke=black}. The ``abc'' refers to an unknown property *.

\textbf{Object Naming.}
We support object naming to enable easy reference. For example, after applying a filter ``US'' and ``2020'' to the chart, users can simply name the chart as ``US2020''. This helps them easily refer to this chart. Object naming further enables nested design of visualizations. For example, users may put two visualizations together by opening up a new canvas and saying \sutt{put \textit{US2019} and \textit{US2020} side by side.} This also helps enable creative visualization design. Figure \ref{fig:examples}c shows an example where the user uses two icons to create a pictograph and reuses it in another chart to create novel visualization design.



\subsubsection{Parameters}
Parameters are specific configurations of the operations. 
They correspond to the operations and objects, describing to what extent the operations are performed, or how operations are applied to objects. 
%Based on the object properties, we need to further define a library of parameters. 
%By defining the forms of these parameters,  users' free-form natural language can be translated into machine-understandable commands. 
As a result, the types of parameters vary with object properties. 
They can be numerical values for chart width and height, enumerations for font style and encoding channels, and boolean values for adding or removing components.
Figure~\ref{fig:taxonomy} shows example parameters corresponding to different chart objects. 
While parameters can be clear and definite in some cases (\eg the \emph{absolute} pixel \emph{quantity} in \sutt{set the chart 10px wide and 13px height.}), they sometimes take more \emph{qualitative} or \emph{relative} forms:


\textbf{Vague Parameters}
%Natural languages might be rough and vague. 
Utterances usually contain free-form parameters that sound natural to humans, yet are hard-to-decode for the machines \cite{hearst2019toward}. 
We collect these keywords as part of the parameter library, and expect the application tool to further interpret and map them into machine-understandable values based on design environments.
%\emph{We collect a list of keywords that represent}
For example, for color values, we support a list of color names (e.g., \spar{color=red}, \spar{color=navy~blue}). We also define a number of extent keywords, ranging from ``extremely'', ``very'', ``moderate'', ``little'', to ``very little''. Users can therefore describe the adjustments of size as ``make it really large'', which will be mapped to ``very large'' and can be parsed as \sact{setSize}{*}{ size=very.large}.
%Editing tools can further interpret them into machine-understandable values based on design environments.

\textbf{Relational Parameters}
Users also tend to make relative statements anchoring on some exisitng visual elements, \eg \sutt{make it larger}, or \sutt{set the color of the title darker than the bars}.
For these relational parameters, we expect users to specify the objects it compared to, and the direction of change. For example, \sutt{make the title darker} is explained as make \emph{itself} darker, where the object is the title; \sutt{place the legend on the right of the plot area} is explained as \emph{right} to the \emph{plot}. 
Formally, the utterances are interpreted to \sact{setColor}{title}{color=self[darker]} and 
\sact{place}{legend}{position=plot[right]}. 
\spar{self[darker]} means the color darker than it self while \spar{plot[right]} means on the right of the plot. Applications should further determine the exact values of these parameters after receiving these vague parameters.






\subsection{Editing Action Coverage}
%{Example Utterances}\sherry{This paragraph doesn't seem to make sense any more.}
%Combining operations, objects, and parameters, \sherry{search and replace ``editing''} editing actions can represent various utterances.
% An utterance may corresponds to multiple editing actions. 
% Here we show example utterances and the corresponding editing actions to further illustrate the use of editing actions. In Figure \ref{fig:examples}, the utterances are represent with one to four editing actions. These examples include object selectors,  vague parameters, and relational parameters.

% \begin{table}[ht]
% \centering
% \includegraphics[width=0.5\columnwidth]{pictures/example-utterances-1-cropped.pdf}
% \caption{Example utterances (left) and corresponding editing actions (right). One utterance may correspond to multiple editing actions.}
% \label{tab:examples}
% \end{table}

To verify our taxonomy, we examine whether or not it can help abstract existing natural language-based visualization systems and multimodal visualization tools, including DataTone \cite{gao2015datatone}, FlowSense \cite{yu2019flowsense}, Analyza \cite{dhamdhere2017analyza}, Orko \cite{srinivasan2017orko}, DataBreeze \cite{srinivasan2020interweaving}, InChorus \cite{srinivasan2020inchorus}, and Valletto \cite{kassel2018valletto}.
We manually read these papers, collected in a total of 75 unique example utterances that occur in their text content and the figures and, when possible, annotate the editing actions they translate to.
In total, 61 (81\%) utterances can be expressed with editing actions, showing that our framework can reasonably cover existing, application specific ones.

The remaining examples that are not covered falls into the two categories: (1) The utterance expresses an intent of data analysis, instead of visualization construction. For example, while ``What is the relationship between unemployment and family income for those families earning more than 20,000 and less than 150,000 between 2007 and 2010 for California and Michigan?'' \cite{gao2015datatone} can be visualized with a scatter plot to show the correlations, it does not directly describe the editing operation. 
(2) The utterance describes the operations conducted directly to the graphical user interface. For example, the utterance ``Highlight the selected cars in a parallel coordinates plot'' \cite{yu2019flowsense} is aimed to highlight the cars selected from one chart on another chart. This helps users conduct analysis through multiple linked views. This category of operations is not covered by our framework.

The utterances that can be expressed contain one to three editing actions. 
%In total, there are 50 data operations, 18 encoding ones, 3 for visual styling, 1 for layout, and 2 annotation operations. 
The operations covered by these work mostly focus on data operations (44 out of 71) and encoding operations (24 out of 71). 
This aligns with the visual analytic focuses of these systems. However, the natural language operations supported by different systems are quite diverse. For example, the operations extracted from utterances from \cite{gao2015datatone} are mostly data  operations (including retrieve, filter), while \cite{yu2019flowsense} involves data (including retrieve, filter, aggregate), encoding (encodeColor), and styling (setColor) operations. 
By considering mark, layout, styling, and annotation operations, the design space of our framework serves as a superset of existing work. This enables the NL interpreter to support a larger range of visualization systems.

















\subsection{Implementation Guideline for the Framework}\label{sec:guideline}
Below, we discuss some key considerations when instantiating our framework into actual NL interpreters and applications.





\subsubsection{NL Interpreter}
\label{sec:nguideline:nl}
\paragraph{Identify natural language understanding tasks.}
At the core of the interpreter is the ability to parse the natural language utterances into {\color{cop}operations}, {\color{cobj}objects}, and {\color{cpar}parameters}.
Operations are usually \emph{summarized} or \emph{abstracted} from utterances, whereas objects and parameters are directly \emph{extracted}.
As such, while there might be other alternatives, we recommend treating this step as two NLP sub-tasks:
(1) a multi-label classification task, to detect potentially multiple operations from an utterance; and 
(2) a sequence labeling task using BIO tagging~\cite{ramshaw1999text}, to recognize token chunks that represent objects and parameters from one sentence.

\paragraph{Choose the class of interpreter model.}
There are two common types of methods to fulfill natural language understanding, \ie rule-based methods and deep-learning models, each of which has its trade-offs.

Rule-based methods (\eg in FlowSense \cite{yu2019flowsense}) depend on part-of-speech (POS) tagging~\cite{li2012wiki}, named entity recognition (NER)~\cite{sang2003introduction}, and semantic parsing techniques~\cite{jia2016data}, and leverages a pre-defined grammar to capture NL input patterns.
They are much more precise when the expected space of input utterance is well-scoped; However, it is complicated to establish rules and analyze the syntax structure of the sentence. When the diversity of input utterances increase, the difficulty of maintaining a set of NL patterns and rules also substantially increased.

On the other hand, deep learning-based models can more flexibly in handling diverse utterances. 
One can easily extend the capability of the NL interpreter by adding training examples that express intended operations, objects, and parameters~\cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}.
That said, these models may not always be interpretable, and can behave more unstably compared to rule-based methods.
Moreover, being ``data hungry'' is also a significant bottleneck: 
to reach the best performance for deep learning models, a large amount of training data is required. 
To maximize the utility of such models, developers should either collect a large number of utterances, or rely on data augmentation techniques~\cite{malandrakis2019controlled} to accelerate the early collections of user intents.


\begin{comment}
\noindent\emph{NL Interpreter}
\wy{
Natural language understanding is the core component of a natural language-based system. The natural language interpreter bridges human utterances and editing actions in a general way. For an input utterance, NL interpreter aims to translate it to  a sequence of editing actions that can be executed by visualization applications. 


Usually, the understanding of natural language inputs takes two steps: first identifying users' intents in the utterances as operations; then extracting useful parts as objects and parameters for the targeting operations. After that, the operations, objects and parameters should be organized into a list of editing operations. 
The editing actions can be further ranked so that the applications can execute the actions one by one.

When the input utterances are well-scoped, rule-based methods are commonly used to conduct syntax analysis and semantic analysis to parse input utterances. For example, FlowSense \cite{yu2019flowsense} applies POS tagging, NER, and semantic parsing techniques, and leverages a pre-defined grammar to capture NL input patterns.
However, to establish rules and analyze the syntax structure of the sentence can be complicated. When the diversity of input utterances increases, the difficulty of maintaining a set of NL patterns and rules also substantially increased.
}
\end{comment}


%Therefore, to establish rules and analyze the syntax structure of the sentence is either complicated or low scalable. 
%Because the accuracy of these systems largely depends on the formulation of rules, the difficulty of maintaining a set of NL patterns and rules also substantially increased.
%If the input sentence is in a different form, we may have to add new rules to explain it. In addition, when the input is incomplete and ambiguous, it becomes harder to identify a set of NL patterns cover the input by rules. 
% Therefore, our example implementation of the natural language interpreter takes a deep learning-based method \cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}. Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy.
% We only need to add more sentences the training dataset to extend the capability of the NL interpreter. 
% This implementation of NL interpreter consists of three steps, namely, token recognition, editing intent and entity extraction, and editing action synthesis. Rule-based methods can also be adopted for NL interpreter.  




\subsubsection{Visualization Applications}

\paragraph{Execute Actions}
The visualization applications should implement an execution engine that processes the interpreted editing actions and executes the operations. If the operations are clearly specified, the execution engine blends the objects and calls the related functions. If the operation is not supported, the execution engine can return error messages to notice the users. If the operation is not supported but related operations are supported, the application can further show simple examples to help users understand the functions of the system. When the actions are not fully specified, the application could predefine a set of rules to recommend proper actions for under specified utterances. 

\paragraph{Manage Contexts}
The applications should manage users' sessions and maintain a list of objects on canvas with corresponding attributes. If the objects are clearly referred, the application simply looks for the objects and applies operations to the target objects.
For objects with selectors, applications can traverse through the object list and finds out all the objects with specific parameters. If the objects cannot be resolved, the application could return error messages to notify users.

%\textbf{Resolving Vague Parameters}
% three types of vague parameters: 
% VisTalk implement a wide range of dynamic widgets to deal with 
% Dynamic Widgets 
% change value (text box, +/- buttons)
% change category (select box)
% change color (color panel)
% choose color theme (select box)
% position (select box; +/- buttons)
% modify content
%Next, we identify the parameters from the output. The intents produced by the NL interpreter contain four types of paramters, namely, exact parameters, under specified parameters, vague parameters, and relational parameters. 
\paragraph{Resolve ambiguities}
The applications should build supports and disambiguate between the three types of parameters: exact, vague, and relational ones.
For exact parameters, applications can directly map the extracted parameters to the data value and check whether the value can be legally assigned. For example, \spar{10px} for height can be directly assigned to the objects. 
%For under specified parameters, VisTalk implements a wide range of dynamic widgets. For example, if a user inputs a statement, ``change the bar color'', the system highlights the keyword ``color'' and popups a color selector. 
For vague parameters, applications can develop a set of metadata or rules to explain vague parameters supported by the NL interpreter. For example, when users input a vague parameter, the application looks up the parameter \spar{red} and yields the color code RGB(255, 0, 0). 
For relational parameters, applications need to parse the parameters into the changing directions of parameter adjustment. For examples, \sutt{on the top} for \sutt{put it on the top of the \textit{China} bar}, means the object should be placed at a point that has smaller distance to the top border than the china bar, but with the same distance to the left/right border as the \textit{China} bar. Therefore, applications should extract the positions for the \textit{China} bar, and calculate a proper position number for the newly added object.

% \subsection{Reusable Chart Templates}
% export the charts as templates.
% Power BI





\section{Example Implementation}
To verify that our framework can be instantiated into useful tools, we build a deep learning-based natural language interpreter that extracts operations, objects, and parameters, and organizes them into a sequence of editing actions. We also build a proof-of-concept NL-based visualization editing system called VisTalk powered by the interpreter.



\subsection{Natural Language Interpreter}
%We model the natural language processing module as the conversion from natural language to our predefined domain-specific language. To do this, we model conversion problem as a natural language understanding problem in natural language processing.
%We formulate this problem as a semantic parsing problem \todo{?} that takes human utterances as input, and outputs executable editing actions. 
%As modeled in Section \ref{sec:model}, an input utterance may include multiple editing action intents. 
%In the visual human-computer interaction, understanding human queries is really important. 

%Natural language understanding is the core component of a natural language-based system. 


We design a multi-stage natural language interpreter to parse natural language utterances into editing actions:

\textbf{Stage 1: In-context data entry abstraction.}
To reduce the sparsity and uncertainty of intent recognition, we use a data entry recognizer to identify and abstract dataset-related data entries in the utterance.
The recognizer enumerates through the n-grams in the utterance to find entities (words or short phrases) that can be matched with the \emph{table names}, \emph{column names}, and \emph{cell values} of a dataset table.
We obtain the \emph{abstracted utterance} by replacing these entities with placeholders like \argu{<column>}, \argu{<value>}\footnote{In the case of special numbers and dates, we further specify value into \argu{<integer>}, \argu{<float>}, \argu{<date>}, and \argu{<year>}}.
%This way, the difficulties and uncertainties of understanding the editing intents can be reduced \cite{yu2018typesql, guo2019towards, dong2019data}. 
%\sherry{What is ``this way''? The whole abstraction, or just the number part?}{}
 
\begin{figure}[t]
\vspace{0px}
\centering
\includegraphics[width=\linewidth]{pictures/labels.pdf}

\vspace{-1px}\caption{A multi-stage natural language interpreter: A natural language utterance is first abstracted by replacing data-related entries. Then, we extract operation categories. Following the BIO (beginning, inside, outside) format\cite{ramshaw1999text}, we can map the words in the sentence into a sequence of labels, where B-, I-, and O represent begin, inside, and outside. The extracted parameters, objects, and operations are further synthesized into editing actions.}
\label{model_example}
\vspace{-5px}
\end{figure}



\textbf{Stage 2: Information extraction for the editing action.}
With the abstracted utterances, we identify users' intents by extracting the \emph{operations} from the utterance, as well as its corresponding \emph{objects}, and \emph{parameters}.
Following Section~\ref{sec:nguideline:nl}, we solve two sub-tasks in this step: (1) multi-label classification for operations, and (2) sequence labeling for objects and parameters.
%As illustrated by the exampled in Figure~\ref{model_example}, this step contains two sub-tasks:
%(1) a multi-label classification task, to detect potentially multiple intents from an utterance; and 
%(2) a sequence labeling task using BIO tagging~\cite{ramshaw1999text}, to recognize token chunks that represent objects and parameters from one sentence.
Inspired by Liu \etal~\cite{liu2016attention}, we design a neural model based on the encoder-decoder framework, attention mechanism \cite{vaswani2017attention}, and CRF algorithm\cite{lafferty2001conditional}. 
The models simultaneously perform the two tasks, outputting separated lists for operations, objects and parameters.
%Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy.
Our model is trained on an internal dataset, containing a mix of real and synthetic utterances expressing certain visualization editing intents:
We first crowdsource 1.3k utterances of 20 operations, covering every operation category.
We showed two visualizations to crowd workers and ask them to write short textual descriptions on how to edit from one to another.
We further augment the dataset by (1) paraphrasing these utterances through back translation and crowdsourcing~\cite{iyyer2018adversarial}, and (2) creating syntactic templates inspired by Malandrakis et al.~\cite{malandrakis2019controlled}.
In total, our dataset contains 7.8k utterances. We use 80\% of the data for model training, and the rest for testing.
%We first collected 1.3K human-labeled natural language utterances by \todo{crowdsourcing - paraphrasing}
%\sherry{Where do these 13k come from?}~\cite{zhong2017seq2sql, locascio2016neural}. Then, to increase the utterance variety, we augment the data by manually inducing a synchronous context-free grammar (SCFG) based on the human-labeled utterances, and use the SCFG to synthesize the rest data~\cite{jia2016data}.\sherry{SCFG is an overly complicated description here. Just say you abstract user intents into templates and use that for data augmentation, and give 1-2 template examples.} \wy{In total, we collected utterances for over 20 types of operations covering every operation category.}
%We evaluate our model performance on the this dataset. %Furthermore, to verify the generality of our model, we also conduct experiments on the ATIS dataset\cite{hemphill1990atis}. ATIS is the public benchmark dataset in natural language understanding, which has many characteristics of spoken language and is completely collected in the actual office environment. The results are shown in Table \ref{model_result}. 
%\todo{term-based prediction accuracy. we have ~20 intents}
Our model worked well on the test set: the operation classification accuracy and the tagging F1 scores for objects and parameters were 99.94\%, and 99.74\%, respectively.
%showing that our model works quite well. %The performance results on ATIS are very close to the state-of-the-art results. Moreover, our model is more adaptive to visualization editing tasks.
%\sherry{What is slot accuracy? BIO? Change the name.}

\textbf{Stage 3: Editing Action Synthesis}
Given the recognized information, we then map between the independently outputted operations, objects and parameters, so as to organize them into a sequence of editing actions.
Because each operation determines its expected parameters and objects (\eg \sop{setColor} would only accept colors as parameters), we traverse the operation list to find the corresponding parameters and objects among the candidates.
If there is no parameter or object for an operation, we fill it with a \texttt{*} mark to denote the default state. 
%The mapping outputs paired tuples, which essentially form a list of editing actions.
We further  heuristically rank these actions based on the category they belong to, prioritizing global operations, (\eg data operation, data encoding, view manipulation) over local operations (\eg changing the color or the title content).
%\sherry{ranking maybe something that can be put into 3.2; multi-label classification and BIO might also fit there.}






% \begin{table}[ht]
% \centering
% \begin{tabular}{p{2.5cm}<{\centering}|p{1.7cm}<{\centering}|p{1.7cm}<{\centering}}

% \toprule  %添加表格头部粗线
% Datasets & Visediting & ATIS   \\
% \hline
% Intent Accuracy & 99.94 & 97.08  \\
% Slot Accuracy  & 99.74 & 97.59 \\
% Slot F1 Score & 99.74 & 97.60  \\

% \bottomrule %添加表格底部粗线
% \end{tabular}
% \vspace{2px}
% \caption{The performance of our model on Visediting dataset and ATIS dataset. Intent accuracy represents the model performance in intent recognition, while slot accuracy and slot F1 score denote model performance in word role label detection.}
% \label{model_result}
% \end{table} 




==> sections/CHI_vistalk.tex <==





\begin{figure*}[tb]
    \centering
    \includegraphics[width=1\linewidth]{pictures/interface.PNG}
    \caption{VisTalk interface (a). Users can type in their natural language utterances in the text box (b) to customize their visualization design (c). Users can author different charts at the same time (d). The table view shows the underlying dataset. The underlying dataset (e). 
    Users can click the words as interactive widgets to resolve ambiguities (f). The auto-completion panel pops out during the input process (g).
    }
    \label{fig:interface}
    \vspace{-5px}
\end{figure*}
\subsection{Visualization Application: VisTalk}
VisTalk is an implementation of the \emph{application} component in our framework\footnote{\url{https://drive.google.com/file/d/1VDyTGw01NRZVWJmQ5yF-hQ-VPHJ1euXb/view?usp=sharing/}}.
As a proof-of-concept tool for visualization creating and editing, VisTalk currently supports bar charts, column charts, line charts, and pictographs. It takes users' natural language input through a simple text input box (Figure~\ref{fig:interface}B), and automatically re-renders visualizations to show changes accordingly (Figure~\ref{fig:interface}C). Importantly, the implementation of VisTalk does not concern about the textual inputs; these utterances are parsed by the interpreter described above. Rather, it focuses on executing the corresponding editing actions. This includes resolving object selectors, executing data queries, and converting vague parameters into accurate default values, following the guidelines in Section~\ref{sec:guideline}.


More specifically, following the research of chart recommendations \cite{setlur2019inferencing, mackinlay2007show}, the application can recommend visualizations from partial specifications of visual charts. For example, one common request is ``Sales by year''. This can be parsed into \texttt{\{BindX, x axis, data field="Year"\}} and \texttt{\{BindY, y axis, data field="Sales"\}}.  VisTalk recommends a bar chart based on the data types. 
To enhance user experience, VisTalk also tries to auto-complete users utterances, provide users with the ability to specify and fine-tune the parameters using interactive widgets (Figure \ref{fig:interface}).


\begin{comment}
\wy{
As shown in Figure \ref{fig:interface}, VisTalk provides a natural language interface for visualization creating and editing. 
The major parts of VisTalk are simply a text input box and the target visualization design. 
VisTalk takes users' natural language input and renders visualizations to show changes accordingly. While typing utterances, VisTalk auto-completes users utterances with a list of popular phrases (Figure \ref{fig:interface}g). Users can also modify existing utterances and the visualization updates automatically.
Currently, VisTalk supports bar charts, column charts, line charts, and pictographs. 
VisTalk parses the utterances sentence by sentence by executing editing operations and render visualization changes to the users (Figure \ref{fig:interface}c). Users can fine-tune their statements by clicking the keywords for icons, colors, chart types, and values. The system pops out interactive widgets (Figure \ref{fig:interface}f) that helps users further specify or modify the parameters.} %错的话
% \subsection{User Interface and Interaction}
% VisTalk provides a set of design views to support users' design. 
% For example, a user can input statements in the input box. Users input a list of sentences and VisTalk parses the input statements one by one. VisTalk 

% Finally, users can save the fine-tuned natural language for future replication. Users can ask VisTalk to ``export the authoring commands'' as a script. The system packs up the natural language utterances with the fine-tune values generated by system. The natural language-like script can be easily understood and modified for similar authoring tasks.

VisTalk is built upon the NL interpreter. Through VisTalk, users first upload datasets to the backend database. Then, they can author visualizations against an underlying dataset with NL utterances. The utterances are sent to the NL interpreter. After processing, the NL interpreter send back corresponding  editing actions. To execute an editing action, VisTalk resolve object selectors, execute data queries, and convert vague parameters into accurate default values following the guidelines in \ref{sec:guideline}. More specifically, following the research of chart recommendations \cite{setlur2019inferencing, mackinlay2007show}, the application can recommend visualizations from partial specifications of visual charts. For example, one common requests is ``Sales by year''. This can be parsed into \texttt{\{BindX, x axis, data field="Year"\}} and \texttt{\{BindY, y axis, data field="Sales"\}}.  The tool can recommend a bar chart based on the data types. 
\end{comment}

%Users then input natural language and the systems bind the data entities to the sentences, and output abstract utterances. For example, \todo{example}. After that, the abstract utterances are digested by the deep learning-based natural language interpreter, which extracts a list of intents, entities, and parameters. VisTalk then interprets the output intentions based on its' own visualization model and renders the visualizations through the visualization generator.


% The major parts of VisTalk are simply a text input box and the target visualization design. Users can upload the dataset in csv format and then start to type their commands. When one sentence is completed and the user presses ``enter'', the system parses the input and shows the change on the visualization directly. If there are vague descriptions, users can directly click on the text to make the command more accurate.

% \subsection{Design Considerations}
% We considered several factors of design considerations for developing a natural language-based visualization system. Different from traditional visualization authoring tools, natural language-based systems rely largely on users' text or speech input. The design of the systems should leverage the advantages of natural language and WIMP interactions.

% \begin{compactitem}
%     \item \textbf{Instant feedback of chart creations} The system should provide a prompt feedback to users' input. The  
%     \item \textbf{Easy to correct misunderstandings} The tool should support easy correction of misunderstanding between system and users. 
%     \item \textbf{Flexible switches between authoring paradigms} The misunderstandings come from the inadequate understanding 
%     \item \textbf{Smart reference and selection} Natural language contains ambiguity in referring objects. The system should support smart selection of visualizations.   \textbf{Name of the charts}
%     \item \textbf{Accurate or fuzzy parameter specifications.} A natural language-based system should support both accurate and fuzzy specifications. Usually, users may input a fuzzy description of the intention because they are not certain about the extent of their parameter specifications. The system should take advantage of the accuracy of direct specification with WIMP interface and fuzziness of natural language input.
% \end{compactitem}



% \subsection{VisTalk Implementation}
% We implemented VisTalk as a Web Application, and used a client-server architecture to distribute the NL interpreter and database operations on remote servers. VisTalk consists of three main components (1) NL interpreter (2) a program synthesis module (3) a visualization renderer...

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth,height=150px]{pictures/architecture.pdf}
%     \caption{vistalk architecture}
%     \label{fig:interface}
%     %\vspace{-10px}
% \end{figure}







% \subsection{VisTalk Functions}
% VisTalk supports the basic functions provided by the natural language interpreter to configure the data binding, style, and higher level operations that supports nested layouts, pictographs, and multiple facets.
% By implementing these visualization authoring operations, we support the building blocks of visualization authoring in a flexible way. 

% Implementation detail for natural language understanding

% Natural Language Operations + objects.
% All the basic operations.
% Smart operations: 




==> sections/UIST_appen-interpreter.tex <==
\section{NL-based Visualization Framework}
We consider the design of our natural language framework against the following requirements: (1)  The framework should be reusable for common visualization construction and configuration intents and support different visualization applications. (2) The framework should be easy to extend to cover more visualization commands and the capability can be improved over time. (3) The framework should support flexible natural language input with vague descriptions.

Based on these considerations, we introduce our natural language-based visualization editing framework (Figure \ref{fig:pipeline}). 
The framework consists of two parts, a \textbf{natural language interpreter} and an \textbf{visualization application}. 
When a user inputs a natural language sentence, the interpreter parses it into \textbf{editing actions} and sends the actions to the application. 
The editing actions are a list of structured descriptions of users' intents and can be executed by the application. \wy{Then, we provide a design guidelines of visualization applications based on the NL interpreter.}

%We design a natural language interpreter that parses human utterances to visualization authoring actions and can be applied across different authoring tools. %\sherry{First sentence is a bit duplicated with the last paragraph; And I think this paragraph needs a rewrite.}
% We model users' visualization editing intents as \textit{editing actions} and formulate an editing action as the combination of \textit{operation}, \textit{objects}, and \textit{parameters}. We summarize and categorize common editing actions into six categories that cover visualization authoring functions in authoring tools. 
%Users' natural utterances can be parsed into authoring actions and passed to applications to execute. 
%First, we define a domain-specific language (DSL) of visualization authoring, covering common operations for visualization authoring from 6 aspects. 
%The natural language processing module takes users' utterances as input, and outputs the program in the form of our DSL. The code can be further parsed and implemented by specific applications or code libraries to complete the specific tasks under different design environments.


\subsection{Editing Actions}\label{sec:model}
A wide variety of visualization creation systems \cite{Wongsuphasawat2016VoyagerEA, 6876042, Liu:2018:DIA:3173574.3173697}, code libraries \cite{bostock2011d3}, and declarative languages \cite{satyanarayan2016vega} have been developed to support visualization creation. Existing tools usually consider marks, data bindings, scales, axes, legends, and layout when specifying charts.
%Further, the visualization authoring systems are implemented with different models. Satyanarayan \etal \cite{satyanarayan2019critical} categorize them into three different types, namely, template editors, shelf construction, and visual builders. Common visualization authoring tools like Microsoft Excel, adopt template editors way. Shelf construction methods support more flexible mapping between encoding channels and data fields, and are adopted by Tableau, Polestar \cite{Pioch2006POLESTARCK}, and Voyager \cite{Wongsuphasawat2016VoyagerEA}. Visual builders like Charticulator \cite{Ren_2019_8440827} and iVisDesigner \cite{6876042} are more complicated and support fine control in specifying marks, glyphs, layouts, etc.
These tools have covered a wide range of functions to enable the composition of both standard charts and highly customized interactive visualizations. However, there was no common design model that can let us consistently describe visualization editing intents \cite{satyanarayan2019critical}.
We survey the functions of modern interactive authoring systems including Microsoft Excel, Tableau, Polestar and Voyager\cite{Wongsuphasawat2017Voyager2A}, Lyra \cite{satyanarayan2014lyra}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and declarative model Vega-lite \cite{satyanarayan2016vega} to recognize common authoring operations and functions. %We identified a set of common functions and categorize them into six categories. 


\wy{These visualization construction tools can be divided into three category \cite{satyanarayan2019critical}. Tools like Microsoft Excel supports \textit{template editor} style, where users may start with a chart type and further make extensive customization. Users may say ``Give me a bar chart for \textit{Sales} by \textit{Country}'' for a bar chart with y-axis encoded with Sales and x-axis encoded with different countries.  Tools like Tableau, Voyager \cite{Wongsuphasawat2017Voyager2A} constructs visualizations by mapping data fields to encoding channels (e.g., x, y, color, shape). An example utterance can be ``Bind \textit{Sales} to y-axis'' and ``Bind \textit{Country} to x-axis''. The tools might further automatically recommend rectangles as marks.  Tools like Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909}, construct visualizations from the fine control of marks, glyphs, coordinate systems, and layouts. Users might start with ``draw a rectangle'', and then, ``repeat it horizontally on \textit{Country}'', and finally ``bind height to \textit{Sales}'' to construct a similar bar chart. Therefore, to fit into these  different styles of visualization tools flexibly, we propose the notion of editing action as the combination of operation, object, and parameters, where users' authoring intents can be simplified as \textit{editing operation} and its \textit{target objects}, and the corresponding \textit{parameters}. }


We define \textit{editing actions} as the combination of authoring \textit{operations}, \textit{objects}, and \textit{parameters}. User utterances can be mapped to one or multiple editing actions. The authoring process of visualization is the execution of a sequence of editing actions. Formally, an authoring intention can be defined as a triple:
\begin{equation}\nonumber
    \texttt{editing~action := \{operation, objects, parameters\}}
\end{equation}

The definition of the editing action describes the actions the authors want to take to the visualizations.  The \textit{operation} identifies the type of the author's intent (e.g., ``change color'', ``add annotation''). The \textit{objects} are the targets that the operation applies to, such as the canvas area, the bars in a bar chart, the title text,etc. Finally, the \textit{parameters} indicate the degree or configurations of the operations.


\begin{table*}[!t]
    \centering
    \includegraphics[width=1\linewidth]{pictures/new-taxonomy-cropped.pdf}
    \vspace{0px}
    \caption{An editing action consists of three parts, operation, object, and parameter.  Operation are categorized into six major groups. Objects are categorized into chart components (e.g., axes, legends, title), mark channels (e.g., shape, color, size, position), and annotations (e.g., reference lines, reference bands, trend lines). \todo{remove this table and replace with a simpler image}}
    \label{fig:taxonomy}
    \vspace{-1px}
\end{table*}

\subsubsection{Operations}
%Our framework models the action of users' authoring requests as a sequence of operations %. %The basic operations are primitive operations (e.g., data binding, change color, change font, etc.). More complex operations can be combined with multiple primitive operations and are used to complete typical design tasks. For example, ``turn the bar chart to a pictograph.'' \todo{how to} %All the operations require target objects (e.g., axes, marks) and parameters. 
%Based on existing visualization authoring systems and taxonomies \cite{satyanarayan2016vega, Ren_2019_8440827, Liu:2018:DIA:3173574.3173697, Wang:2018:IEC:3173574.3173909, ren2017chartaccent}, 
%The most primitive operations that appear in visualization authoring tools 
%and 
%We categorize authoring operation into six major groups.
%, namely, data operations, visual encoding operations, layout operations, styling operations, view manipulations, and annotate operations.\todo{no need to list the names of the categories since they will be listed below...} 
%Different o
Operations may apply to different objects, depending on the properties of the objects. 
Table 1 lists the operations and the corresponding target objects and possible parameters. 
As discussed previously, operations are not exclusive because different tools support different design paradigm and human languages also express same meanings with different patterns. For example, binding a data field to x axis, has the same effect as encode the horizontal position of mark to the field.   
%We list common editing actions that are used in visualization authoring.
% \begin{compactitem}
%     \item \textbf{General operations}, like \textit{add}, \textit{remove}, \textit{copy}, are the operations that can be acted upon any object, including graphical elements (e.g., add an annotation) or data encoding (e.g., remove a filter).
%     \item \textbf{Data encoding} is the mapping between data and visual channels.
%     \item \textbf{Data transform} are the operations that are related to data query and calculation, such as \textit{select}, \textit{filter}, \textit{pivot}, and \textit{join}.
%     \item \textbf{Selectors} are the operations that are applied to the objects with visual properties, such as \textit{change color}, \textit{modify shape}. For example, users can change the color of the title; or change the color scheme for the marks in a chart. Users may even replace the marks with icons for expressive visualization design.
%     \item \textbf{Numerical operators} are the operations that are related to the numerical properties of objects. Change range, of something. For example, change the height and width.
%     \item \textbf{layout operators} are a special type of numerical operators that can be widely used for expressive visualization designs. Users may add labels, annotations, and configure the positions of them. They may \textit{move} up or left, \textit{change position} to a specific point, or even \textit{adjust z-order} for the graphical elements.
%     \item \textbf{Text operators} include the operations that are specifically related to text. For example, users may \textit{modify content} of titles, or \textit{change font} for the annotations.
% \end{compactitem}
% \begin{compactitem}
%     \item \textbf{Bind} is the mapping between data and visual channels; data transformation and data fields; data transformation and visual channels 
%     \item \textbf{Add/Remove/Modify} can be applied to graphical element on a visualization design. For example, ``add the legend'', ``modify the title''. They can also be applied to data encoding, such as ``add a filter''.
%     \item \textbf{Set value} is applicable to any object with numerical properties, such as size, height, opacity, etc. 
%     \item \textbf{Change category} is used for the visualization objects with only discrete value properties.
%     \item \textbf{Color} is a special, color related, color scheme 
%     \item \textbf{Font} font style
%     \item \textbf{Style}
%     \item \textbf{Place} (move, position)
% \end{compactitem}
%The operations are categorized by visual features of the target objects. 
%In a visualization design, different visual components may have different properties. These properties further specify the variables that characterize the target components. For example, encoding supports different encoding channels such as position(x, y), size, and color. Marks have properties including shape, color, etc. The shapes for marks are rectangles for bar charts, circles for bubble charts, symbols for scatter plots, etc. The properties for marks also depend on the implementation of the charts. For example, a more flexible authoring tool may support users to replace the basic geometric shapes with icons, or even images. Following the implementation of existing authoring systems, 
\wy{We summarize the authoring operations by going through the category of Vega-Lite grammar \cite{satyanarayan2016vega}, from which we collect a large number of visualization operations related to \textit{data, encoding, and mark}.
To support the construction of more expressive visualizations, we further include common styling operations, and collect operations from ChartAccent \cite{ren2017chartaccent}, Charticulator \cite{Ren_2019_8440827}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909} to develop three more categories related to \textit{layout, styling, and annotation}. } We summarize six main categories of operations:
\begin{compactitem}
    \item \textbf{Data operations} are the operations that retrieve and calculate data from datasets. Typical operations include filter, aggregate, bin, set time unit, and sort.  
    \item \textbf{Encoding operations} are the operations that bind data fields to different encoding channels. Users may also take operations to the axes or directly assign chart types to specify encoding.%, while the effects might be the same. %For example, ``bind Country to x axis'' and ``bind Country to the horizontal position of marks'' have different objects (i.e., x axis and position), while they have the same effects. 
    \item \textbf{Mark operations} include the configurations related to the configuration of marks. Users may change the shape, color, style of marks. The types of mark can be vector shapes, text, images, icons, etc. 
    \item \textbf{Layout operations} include the configurations related to position and offsets of chart elements, such as title, annotation, legend. Users can place an object at a designated position, or move it along a direction.
    \item \textbf{Styling operations} includes graphical operations and textual operations. Graphical operations are performed to color, size, shape, icon, and stroke of graphical elements, such ass axis lines, marks, reference line, etc. Textual operations are acted to text-related properties such as font (size, color, style, weight), content. They can be applied to title, labels, annotations, etc.
    %\item \textbf{View manipulation} refers to operations that create one visualization with multiple views. Chart views can be created into multiple or layered displays. %Multiple views can also be created by ``faceting'' the current view by one data column (e.g., facet the sales by country) or ``repeating'' one chart view to other data values (e.g., repeat the sales chart for US and Japan). 
    \item \textbf{Annotate operations} manipulate annotations (e.g., text, labels, embellishments) that enhance the charts. Annotations can be bound with data. For example, trend lines can show the trend between two time points. Common types of annotations include labels, annotation text, reference line/band, trend line, average line, etc.
    %can show aggregated values by the marks\todo{do we have the corresponding operation for adding labels?} . 
\end{compactitem}



%Based on these operations, more complex high-level operations can be combined. For example, "change the style" usually means the combination of graphic properties and textual properties. This may even apply to the color coding of the marks, further impacting data encoding properties. ``Sales by year'' usually means create a chart, bind x axis with Sales, and bind y axis with Year.

% \begin{compactitem}
%     \item \textbf{Change Chart} removes the current chart encoding and applys new encoding to change the chart into a new one.
%     %ll\item \textbf{Repeat and partition}  
%     \item \textbf{View composition} (facets) applies all the settings and further modifys the data encoding properties.
%     \item \textbf{Fill percentage} adds a background icon with the same foreground icon but different colors.
%     \item \textbf{Interaction} specifies different sets of properties based on users' interaction conditions. Users need to specify the condition and the effects of the interactions.
% \end{compactitem}




\subsubsection{Objects}
Objects are the components that the operations target. 
%For an authoring operation, users usually need to specify the targeting object they want to create, modify, or remove. 
In \wy{WIMP (Window, Icon, Menu, Pointing)} interfaces, users usually click on the menus or select the targeting objects on canvas. For a natural language environment, users need to specify the objects through NL utterances.
For a basic visual chart, the objects include marks, axes, title, legend, gridlines, etc. More advanced objects include annotations such as trend line, reference line, reference band, text annotations, and embellishments.  

\wy{The objects are corresponding to different operations. For example, the objects of \textit{data operations} include data fields, data points, data type, data range etc. The objects of \textit{encoding operations} include the data fields, chart components such as axes, legends, title, and mark channels such as mark size, mark shape, mark position. The objects of \textit{styling operations} include visual properties such as opacity, stroke, text font, text color, and so on.}
% \wy{\begin{compactitem}
%     \item \textbf{Data/Datasets} include data fields, data points, data type, data range etc. When users conduct data operations, they need to assign parameters to these objects.
%     \item \textbf{Chart Components} are the basic parts of charts. This category includes plot area, axes, legends, title, etc.
%     \item \textbf{Mark channels} are targeted by encoding operations. Users need to encode data fields with different channels of marks, such as mark shape, mark color, and mark size.  
%     \item \textbf{Annotations} are additional graphical or textual elements to the charts. Annotations can be bound with data value or data points. For example, reference lines, reference bands are directed related to data; text annotations, image annotations can be placed near one certain data point; data labels can be shown at near each data point to show the values.
%     \item \textbf{Configs} are the properties of visual elements that styling operations take effects, including text font, stoke, opacity, width, and so on.
%     \item \textbf{Layout} are position-related visual properties. Users may need to change position, alignment, offset, z-index of the elements when position is not encoded with data.
% \end{compactitem}
% }

The objects in an editing action can be under specified. For example, a user may say ``give me a chart'' after uploading a dataset. An intelligent system can recommend a best encoding to users, or ask users to clarify the command.
We directly models users intention and use a special notation ``*'' to represent  the under specified objects. The implementation of visualization systems cam further decide definite reference strategies.

%Clearly, a target component may support more than one target operations\todo{???}. %A mark may simultaneously support encoding operations and styling operations. 

% To describe an authoring operation, users usually need to specify the targeting object they want to create, modify, or remove. 
% In graphical user interface systems, users usually click on the menus, or select the targeting objects on visualization canvas. For natural language environment, users need to specify the objects through their utterances.

% \textbf{Objects} are the components that the operations targeted to. For example, for a basic visual chart, the components include marks, axes, title, legend, encoding, etc. Authoring tools for standard charts usually only support limited number of target properties. Supported components can further include annotations such as trend line, reference line, text annotations, etc., depending on the implementation of different authoring tools.  
% Clearly, a target component may support more than one target properties. An implementation of visualization mark may simultaneously support general properties, graphic properties, and data encoding properties. 
% For example, the rectangles in a bar chart can be configured to different color and widths. The rectangle mark can also be replaced with other shapes to reach expressive visualization designs. While different target properties are handled by corresponding operations. The parameters further configure how to change these objects. 

%Once users obtain a chart, they may further say ``turn it to red''. The systems may infer the intention of the users is ``turn the marks to red''. We 

\textbf{Object Selectors.}
As discussed in Section 3, users show special patterns when referring to objects with natural language. 
They may refer to objects through \textit{object properties}. 
%For example, users may ask the system to ``turn the red line blue'', which means ``turn the line in red color to blue color''. Therefore, w
We support an object selector for users to filter the objects. For example, the intention ``turn the red line blue''  does not directly specify the object because there is no component named ``red line''. %The ``red line'' can be selected as \texttt{[shape=line,~ color=red]}, 
The statement can be presented as \sact{SetColor}{[shape=line,color=red]}{color=blue}, meaning to select objects the properties, ``line'' and ``red''. 
%The similar pattern can also be applied if visualization components are clearly referred to, but users would like to select parts of them. For example, ``add black stroke to the blue bar'' for a colored bar chart can be translated to \texttt{setStroke, [shape=bar, color=blue], color=black])\}}, meaning users wants to change the style of the mark with blue color and the operation is \texttt{setStroke}. 
The properties that users describe should exist in the predefined library of property and parameters. Otherwise, the natural language interpreter may not be able to match them and leave quotation marks to the text phrases. %Further, the natural language interpreter may not be able to understand the attribute type and leave a star mark as placeholder. Applications may further parse the attributes based on the context of authoring.
For example, ``add black stroke to the abc bar'' can be translated to 
\sact{setStroke}{[shape=bar,*=`abc']}{stroke=black}.

\textbf{Object Naming.}
We support object naming to enable easy reference. For example, after applying a filter ``US'' and ``2020'' to the chart, users can simply name the chart as ``US2020''. This helps them easily refer to this chart. Object naming further enables nested design of visualizations. For example, users may put two visualizations together by opening up a new canvas and saying ``put US2019 and US2020 side by side.'' This also helps enable creative visualization design. Figure \ref{fig:examples}c shows an example where the user  use two icons to create a pictograph and reuse it in another chart to create novel visualization design.



\subsubsection{Parameters}
Parameters are specific configurations of the operations. The parameters correspond to the operations and objects. It describes what extents the operations are performed, or how the operations are applied to the objects. Based on the object properties, we need to further define a library of parameters. By defining the forms of these parameters,  users' free-form natural language can be translated into machine-understandable commands. Table 1 shows example parameters corresponding to different chart objects. 
When users specify their requirements in natural language, the parameters can be clear and definite. For example, ``please set the chart 10px wide and 13px height.''
The parameters can be implemented as numerical values for chart width and height, enumerations for font style and encoding channels, boolean values for adding or removing components.



\textbf{Vague Parameters}
Natural languages might be rough and vague. We define a set of vague parameters for different operation types. For example, for color values, we support e a list of color names (e.g., \texttt{color=red}, \texttt{color=navy~blue}). We also define a number of extent keywords, ranging from ``extremely'', ``very'', ``moderate'', ``a little'', to ``very little''. Users can therefore describe the adjustments of size as ``make it really large'', which will be mapped to ``very large'' and can be parsed as \texttt{\{setSize, *, size=very.large\}}.
Authoring tools can further interpret them into machine-understandable values based on design environments.



\textbf{Relational Parameters}
With a well-defined parameter set, we can further turn the vague description of the intention to concrete parameters. We support two types of relational parameter that can converse users utterances such as ``make it larger'', or ``set the color of the title darker than the bars''. For each relational parameter, users need to specify the objects it compared to, and the direction of change. For example, ``make the title darker'' is explained as make ``itself'' darker, where the object is the title; ``place the legend on the right of the plot area'' is explained as ``right'' to the ``plot''. Formally, the utterances are interpreted to \texttt{\{setColor, title, color=self[+]\}} and 
\texttt{\{place, legend, position=plot[right]\}}. \texttt{self[+]} means the value larger than it self while \texttt{plot[right]} means on the right of the plot. Applications should further determine the exact values of these parameters after receiving these vague parameters.






\subsubsection{Example Utterances}
Combining operations, objects, and parameters, authoring actions can represent various authoring utterances. An utterance may corresponds to multiple authoring actions. 
Here we show example utterances and the corresponding authoring actions to further illustrate the use of authoring actions. In Table \ref{tab:examples}, the utterances are represent with one to four authoring actions. These examples include object selectors (d, e),  vague parameters (b, c, d, e, f), and relational parameters (b, d).

\begin{table}[ht]
\centering
\includegraphics[width=0.5\columnwidth]{pictures/example-utterances-1-cropped.pdf}
\caption{Example utterances (left) and corresponding authoring actions (right). One utterance may correspond to multiple authoring actions.}
\label{tab:examples}
\end{table}


\textbf{Editing Action Coverage}
\wy{To verify our taxonomy, we go through natural language-based visualization systems and multimodal visualization tools which include speech or text as input, including DataTone \cite{gao2015datatone}, FlowSense \cite{yu2019flowsense}, Analyza \cite{dhamdhere2017analyza}, Orko \cite{srinivasan2017orko}, DataBreeze \cite{srinivasan2020interweaving}, InChorus \cite{srinivasan2020inchorus}, and Valletto \cite{kassel2018valletto}. We collect 58 example utterances from the examples of these papers to examine the coverage of the framework. In total, 47 utterances can be covered. \todo{how we are more than them: how ambiguity operators are exist in the examples? how are these papers cover the taxonomy? further data analysis} The remaining examples that are not covered falls into the two categories: (1) The utterance expresses an intent of data analysis, instead of visualization construction. For example, while ``What is the relationship between unemployment and family income for those families earning more than 20000 and less than 150000 between 2007 and 2010 for California and Michigan?'' \cite{gao2015datatone} can be visualized with a scatter plot to show the correlations, it does not directly describe the editing operation. 
(2) The utterance describe the operations conducted directly to the graphical user interface. For example, the utterance ``Highlight the selected cars in a parallel coordinates plot'' \cite{yu2019flowsense} is aimed to highlight the cars selected from one chart on another chart. This helps users conduct analysis through multiple linked views. This category of operations is not covered by our framework.
}




\subsection{Implementation Guideline for the Framework}\label{sec:guideline}
\textbf{NL Interpreter}

Pros and cons**
**

\todo{what are the guidelines}

\textbf{Visualization Applications}
Visualization applications should implement an execution engine that processes the interpreted editing actions and executes the operations. If the operations are clearly specified, the execution engine blends the objects and calls the related functions. If the operation is not supported, the execution engine can return error messages to notice the users. If the operation is not supported but related operations are supported, the application can  further show simple examples to help users understand the functions of the system. When the actions are not fully specified, the application could predefine a set of rules to recommend proper actions for under specified utterances. 

The visualization applications should manage users' session and maintains a list of objects on canvas with corresponding attributes. If the objects are clearly referred, the application can simply looks for the objects and applies the operations to the target objects.
For objects with selectors, applications can traverse through the object list and finds out all the objects with specific parameters. If the objects cannot be resolved, the application could return error messages to notify users.

%\textbf{Resolving Vague Parameters}
% three types of vague parameters: 
% VisTalk implement a wide range of dynamic widgets to deal with 
% Dynamic Widgets 
% change value (text box, +/- buttons)
% change category (select box)
% change color (color panel)
% choose color theme (select box)
% position (select box; +/- buttons)
% modify content
%Next, we identify the parameters from the output. The intents produced by the NL interpreter contain four types of paramters, namely, exact parameters, under specified parameters, vague parameters, and relational parameters. 
There are three types of parameters, exact parameters, vague parameters, and relational parameters.
For exact parameters, we directly map the extracted parameters to the data value. We just check whether the value can be legally assigned. For example, `10px' for height can be simply assigned to the objects. 
%For under specified parameters, VisTalk implements a wide range of dynamic widgets. For example, if a user inputs a statement, ``change the bar color'', the system highlights the keyword ``color'' and popups a color selector. 
For vague parameters, VisTalk maintains a list of explanations to the vague parameters supported by the NL interpreter. Whenever users input a vague parameter, VisTalk lookups the descriptive parameters and finds the corresponding accurate value. For example, the parameter ``red'' yields the color code RGB(255, 0, 0). For ``high'' values, VisTalk infers it to the range (average, max).
For relational parameters, VisTalk also empirically maintains a set of predefined rules to adjust the value. For examples, ``on the top'' for ``put it on the top of the china bar'', means putting the item 10px away from the rectangle; ``make it bigger'', means increasing the size by 20\%. For relational parameters, VisTalk also highlights the parameters in the original utterances to enable users to do modifications through interactive widgets.



% \subsection{Reusable Chart Templates}
% export the charts as templates.
% Power BI





\section{Example Implementation}
To assess the design of our natural language framework, we build an a deep learning-based natural language interpreter that extracts operations, objects, and parameters and organized into a sequence of editing actions. Building upon this natural language interpreter, we build a proof-of-concept NL-based visualization authoring system in the form of VisTalk. 



\subsection{Natural Language Interpreter}
%We model the natural language processing module as the conversion from natural language to our predefined domain-specific language. To do this, we model conversion problem as a natural language understanding problem in natural language processing.
%We formulate this problem as a semantic parsing problem \todo{?} that takes human utterances as input, and outputs executable authoring actions. 
%As modeled in Section \ref{sec:model}, an input utterance may include multiple authoring action intents. 
%In the visual human-computer interaction, understanding human queries is really important. 
Natural language understanding is the core component of a natural language-based system. 
Usually, the understanding of natural language inputs takes two steps: first identifying users' intents in the utterances as functions; then extracting useful parts as parameters for the targeting functions. We design a multi-stage  natural language interpreter from natural language utterances to editing actions. First, we recognize data entities and outputs representations of utterance with data entities replaced with abstract arguments. After that, we design a deep learning-based natural language processing module that extracts intents and entities from the utterances \cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}.  Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy. We only need to add more sentences the training dataset to extend the capability of the NL interpreter.  Finally, the intents and entities are mapped to operations, objects, and parameters and organized into a sequence of editing actions. 

% The natural language interpreter bridges human utterances and authoring applications in a general way. For an input utterance, NL interpreter aims to translate it to  a sequence of editing actions that can be executed by visualization authoring applications. 


%To automatically understanding the input sentence and taking operations in the application accordingly, we need to firstly recognize the user’s entire intent. With obtained intent, we should further extract the useful parts in the sentence as references and parameters of the operation functions. 

%Therefore, to establish rules and analyze the syntax structure of the sentence is either complicated or low scalable. 
%Because the accuracy of these systems largely depends on the formulation of rules, the difficulty of maintaining a set of NL patterns and rules also substantially increased.
%If the input sentence is in a different form, we may have to add new rules to explain it. In addition, when the input is incomplete and ambiguous, it becomes harder to identify a set of NL patterns cover the input by rules. 
% Therefore, our example implementation of the natural language interpreter takes a deep learning-based method \cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}. Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy.
% We only need to add more sentences the training dataset to extend the capability of the NL interpreter. 
% This implementation of NL interpreter consists of three steps, namely, token recognition, authoring intent and entity extraction, and editing action synthesis. Rule-based methods can also be adopted for NL interpreter.  




\textbf{Token Recognition} Before the interpretation of user utterances, we recognize dataset-related entities in the utterance as the first step. These entities are table names, column names, and cell values in a table. The natural language interpreter is therefore aware of the data context. %For example, for a dataset ``CarSales.csv'', we identify data column names like ``Sales'' and ``Brand'', and data values like ``Ford'' and ``Honda'' in users' natural language utterances. To do this, we enumerate all the n-grams and check against the table entities in the input query in descending order of length. Once a k-gram is recognized (k may be different from n), we remove all the remaining n-grams that has overlapping parts with it. %We assign these entities as \textit{exact match} or \textit{partial match} of dataset entities for typo tolerance. 
After that, we replace these recognized tokens with abstract arguments like $<column>$, $<value>$ as input for the next stage. 
Further, we also link entities like number and date as special entities through similar ways. We assign numbers and dates into four categories: $<integer>$, $<float>$, $<date>$, and $<year>$.
This way, the difficulties and uncertainties of understanding the authoring intents can be reduced \cite{yu2018typesql, guo2019towards, dong2019data}. 
The token recognition phase outputs representations of user utterance with data entities replaced with abstract arguments.

\textbf{\wy{Intent and Entity Extraction}}
The purpose of this stage is to identify  \wy{objects and parameters} corresponding to the operations. They can be further organized into editing actions through a synthesis stage. An NL utterance for visualization authoring may involve multiple intents.
For instance, the sentence in Figure \ref{model_example} expresses four visualization authoring intents. Similar to NLP tasks such as semantic role labeling, sequence labeling, and named entity recognition, extracting objects and parameters in an utterance is actually a BIO tagging problem~\cite{ramshaw1999text}. In our task, we define the entities as the utterance parts which act as objects and parameters in editing actions. We create a series of labels following the BIO format to indicate the role of each utterance parts (Figure \ref{model_example}). We train a neural network-based model to recognize intents and entities from input utterances.  Rule-based methods can also be applied. Specifically, on the basis of the work of Liu \etal \cite{liu2016attention}, we design a joint model for intent detection and entity recognition based on encoder-decoder framework, attention mechanism \cite{vaswani2017attention}, and CRF algorithm\cite{lafferty2001conditional}. Through our neural model, the predicted intent tags and entity labels of each words can be obtained.

\begin{figure}[t]
\vspace{0px}
\centering
\includegraphics[width=0.5\linewidth]{pictures/labels.pdf}

\vspace{-1px}\caption{Intent tags and word labels of an example NL utterance. We regard color, chart type, y field (the data field bind to y axis), and x field (the data field bind to x axis) as entities in our model. Following the BIO (beginning, inside, outside) format\cite{ramshaw1999text}, we can map the words in the sentence into a sequence of labels, where B-, I-, and O represent begin, inside, and outside, respectively.}
\label{model_example}
\end{figure}


%The model takes user utterance as the input and recognizes its intent and entities. For example, in Figure \ref{model_example}, after passing through the token recognition module, the given sentence is fed into the neural model. We can obtain the predicted intent tag, \textit{SetChartType}, \textit{SetColor}, \textit{BindX}, \textit{BindY}, and entity labels of each words, O, O, B-Color, B-ChartType, I-ChartType , O, B-YField, O, B-XField.
%We implement a neural network-based model to recognize the intent and entities of the sentence. Compared with traditional rule-based models with syntax analysis and semantic analysis, neural network-based model is simpler to maintain \cite{chen-etal-2016-sentence, pasupat2015compositional}. It is also more scalable to new data because there is no requirement to make changes to existing rules or set more extra rules.
%Based on the modeling of authoring actions, we treat all the parameters and objects as entities in a NL utterance. Together with intents (operations), we organize entities (objects and parameters) into authoring actions.
% \begin{figure}[!t]
% \centering
% \includegraphics[width=\columnwidth]{pictures/model_arch2.pdf}
% \caption{The architecture of our model for intent and entity extraction.}
% \label{model_arch}
% \end{figure}
% As shown in Figure \ref{model_arch}, o

%Our deep learning model is based on encoder-decoder framework. Specifically, we employ Bi-LSTM\cite{hochreiter1997long} as the encoder and LSTM cell as the decoder\cite{liu2016attention}. \todo{remove this part but add the model figure?: In the encoder part, the input words are mapped into an embedding space and represented as vectors, which are used in decoder to generate the target output. At a time step $t$, we use the hidden state $H_t$ to represent the input word $x_t$. $H_t$ is obtained by concatenating $h_t$ and $h_t’$, the hidden states of forward and backward LSTM networks. The last state of the forward and backward LSTM network carries information of the entire sentence, so we concatenate $h_n$ and $h_n’$ as the intent vector of the whole sequence. The intent vector and word representations will then be sent into the decoder. } For intent recognition, due to the fact that a sentence may contain multiple intents, we predict the probability of all intents. If the probability of an intent is greater than 0.5, we consider it as one intent of the given utterance. For entity extraction, the attention mechanism is incorporated for better representation of each input word before determining the entity labels\cite{liu2016attention,vaswani2017attention}. To address the problem of inaccurate entity sequence prediction, we further apply Conditional Random Field (CRF) algorithm in the prediction process\cite{xu2013convolutional,zhang2016joint,huang2015bidirectional}, so that during tagging a word, we can adopt the previously labeled information and Viterbi algorithm to get the optimal entity sequence prediction. Finally, we extract the intention category and labels for all segments $Y = (y_1, ..., y_n)$. The parameters of the LSTM and CRF are jointly trained.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\linewidth]{pictures/interface.PNG}
    \caption{VisTalk interface (a). Users can type in their natural language utterances in the text box (b) to customize their visualization design (c). Users can author different charts at the same time (d). The table view shows the underlying dataset. The underlying dataset (e). 
    Users can click the words as interactive widgets to resolve ambiguities (f). The auto-completion panel pops out during the input process (g).
    }
    \label{fig:interface}
    \vspace{-5px}
\end{figure*}

\sherry{I feel the description of the dataset is still useful; The acc table, and some sample utterances?} \todo{discuss how to clarify the }
We collect a VisAuthoring dataset to train our model. It contains about 78K visualization authoring utterances, covering data operations, encoding operations, annotate operations, styling operations and view manipulations. As a first step, this dataset is composed of two main sources. First, we obtain the dataset by collecting more than 13K human-labeled natural language utterances \cite{zhong2017seq2sql, locascio2016neural}. Second, we manually induce a synchronous context-free grammar (SCFG) based on the human-labeled utterances and use the SCFG to synthesize the rest data \cite{jia2016data}. The dataset consists of natural language sentences and their corresponding intent tag, entity labels of each word in the sentences. %In total, there are \todo{31} kinds of intents, covering all the operation types. Additionally, there are \todo{32} kinds of entity tags, such as {B-mark.Mark, I-sort.Sort, B-unit.NumberUnit, B-text.String} and so on.
We evaluate our model performance on the VisAuthoring dataset. %Furthermore, to verify the generality of our model, we also conduct experiments on the ATIS dataset\cite{hemphill1990atis}. ATIS is the public benchmark dataset in natural language understanding, which has many characteristics of spoken language and is completely collected in the actual office environment. The results are shown in Table \ref{model_result}. 
\todo{term-based prediction accuracy. we have ~20 intents}
We assess from three aspects: intent accuracy, slot accuracy, and slot F1 score. The accuracy is 99.94\%, 99.74\%, and 99.74\%, respectively, showing that our model works quite well. %The performance results on ATIS are very close to the state-of-the-art results. Moreover, our model is more adaptive to visualization authoring tasks.


% \begin{table}[ht]
% \centering
% \begin{tabular}{p{2.5cm}<{\centering}|p{1.7cm}<{\centering}|p{1.7cm}<{\centering}}

% \toprule  %添加表格头部粗线
% Datasets & VisAuthoring & ATIS   \\
% \hline
% Intent Accuracy & 99.94 & 97.08  \\
% Slot Accuracy  & 99.74 & 97.59 \\
% Slot F1 Score & 99.74 & 97.60  \\

% \bottomrule %添加表格底部粗线
% \end{tabular}
% \vspace{2px}
% \caption{The performance of our model on VisAuthoring dataset and ATIS dataset. Intent accuracy represents the model performance in intent recognition, while slot accuracy and slot F1 score denote model performance in word role label detection.}
% \label{model_result}
% \end{table} 


\textbf{Editing Action Synthesis}
Given intents and entities, we then perform program synthesis to organize them into a sequence of editing actions. Editing actions consist of three parts, operation, objects, and parameters. For extracted intents and entities, the intents are mapped to operations, while the entities are mapped to objects and parameters. 

We synthesize editing actions by traversing the intent list. The intent obtained can be directly mapped to the operation types. Based on operation types, we can determine the corresponding objects and parameters. 
%The matching process works as follows: For each intent of an utterance, we traverse the extracted entity list one by one. We map the intent to an operation. If the entity belongs to the operation, it can be matched to the operation and directly filled into the object or parameter. Once an entity is successfully matched to an operation, we delete it from the entity list, which means each entity in the list can only belong to one operation. 
If there is no parameter or object for an operation, we fill it with a ``*'' mark, meaning the default state. After this process, we will obtain a list of editing actions.
%From remaining entities, there are two possible situations. One is that an intent is reused in the utterance. For example, in the case “change color of china and US bar to green and blue”, the entities “china” and “green” are left and haven’t been matched to any intent because the intent “change color” is reused. In this circumstance, we assume users specify the objects and parameters in order, so we fill the residual entities into the closest intent based on entity name and type. The other situation is that the residual entity exists as the selector of the object. For these cases, we check the list of objects and their supported properties, and fill the entity type and entity value into the selector of the object with proximity principle. If such matching object cannot be found, for example, users may only say ``red'' or ``bar'' as an utterance, then these entities are packaged one by one as editing actions without operations.
After getting a list of editing actions, we further rank them based on the category they belong to. Considering the operation types in the editing actions, we sort the editing actions from global operations, such as data operation, data encoding, view manipulation to local operations, such as changing the color, changing the title content.



==> sections/UIST_conclusion.tex <==

\section{Conclusion}
\revise{
In this paper, we explore a natural language-based visualization editing framework, which supports the understanding of chart editing. We propose definitions of editing actions that describes users' unstructured statements with multiple structured expressions, defined as tuples of operations, objects, and parameters. The editing actions bridge between NL interpreter and visualization applications.
To assess our framework, we implement an NL interpreter based on a deep neural network to extract operations, objects, and parameters from users' utterances. From the extracted information, we further synthesize the editing actions. Based on the NL interpreter, we developed two example applications, a Chart Editor add-in for Excel, and a NL-based chart construction tool, VisTalk. The applications take editing actions as inputs, and further parses the expressions to update the charts along with users' editing process. We further conduct a user study with VisTalk to understand how users edit visualizations through natural language interfaces. Our study is a first step towards a generic framework for NL-based chart editing.
}
 

\begin{comment}
\sherry{

\textbf{How to keep the interpreters unified, and the applications specified?}
In contrast to prior visualization creating and editing systems that follow specific design paradigms~\cite{satyanarayan2019critical}, our framework envision a one-method-for-all schema.
As a result, we alleviate the need for getting familiar with the visualization concept models, and therefore lower the learning curve for users of different backgrounds.
That said, precisely because we avoid shaping users' mental model towards a specific editing behavior, unified interface comes with challenges:

First, \emph{how to account for people's different expressions with the same aims?}
Users that have different backgrounds, or are familiar with different visualization tools, can submit utterances that are too flexible to disambiguate.
Section~\ref{sec:model} enumerates the different visualization creation types: to create the chart from scratch, the utterances can be as high level as just mentioning the data columns (and the system is expected to automatically infer the chart type); 
It can also go as low-level as binding each specific mark channel (\eg rectangles) individually.
Second, To achieve the seamless switch between these types, we need to build \emph{interpreters} that understand all the different commands.
Assuming we follow the deep learning approach as in our sample implementation, a crucial step would be to collect a diverse set of training utterances that express the same intent in various level of details.
This can be achieved by feeding crowd labelers with different \emph{visualization objectives}.
For example, users are more likely to say \sutt{sales by country} if we ask them to create a chart that inspect the correlation between ``sale'' and ``country'';
However, they may be intrigued to say \sutt{bind country to x-axis}, if we ask them to treat ``country'' as an independent factor in a series of analyses.
Alternative, we can diversify utterances by constraining them on \emph{construction workflows.}
In this case, we will ask expert users to write utterances, \emph{as if their utterances can only be parsed into a serial of actions in one of the three construction workflows} (template editor, shelf-construction, or visual builders).
We can then further augment the dataset by paraphrasing these commands.

On the other hand, users' more flexible NL input poses challenges for NL-based applications. First, While the capability of parsing natural language utterances increase, our applications might be \emph{designed} to only focus on a subset visualization creation and a editing actions.
For example, how should a system react to \sutt{change the rectangle to circle}, if it only want to support analytical interactions, and therefore does not allow mark customization?
Would it disappoint people, if by design an application ignore more utterances than another tool, even when the interpreter parses it correctly?
User studies on how users react to the boundary of applications is interesting. 
Alternatively, we can improve command recommendation, make suggestions to users when their utterance does not belong to the supported function type, and let people understand the scope of application functions.
}
\end{comment}
% \textbf{Visualization Literacy}
% Users' behaviors towards natural language-based authoring systems may vary a lot based on their visualization literacy. Similar to the results of our formative study, the user study further confirms the differences among users with different background. Users with or without visualization expertise may have totally different mental models of creating charts \cite{}. However, natural language interfaces support unified interface for different users, which provides a better learnability. Users can simply switch among different creation process of visualizations.  



% \wy{
% \textbf{Designing Novel Visualization Tools to Support Multimodal Experiences.} 
% The design of natural language interpreter decouples the parsing tasks from the application that implements the commands. This method eases the difficulties of implementing natural language-based applications. It may help visualization researchers better focus on the design of more natural interaction experience. 
% In the future, we plan to collect more data on visualization editing and release the NL interpreters. This could lower the barriers of designing and developing novel natural language-based visualization construction techniques and tools.
% For example, the authoring systems could design better experience for users to understand the vagueness and under-specification in their natural language input. It can also be challenging for users to understand system functions and how to describe their intents, a better natural language interaction experience should help users  enhance the recommendation of possible future actions to take.
% Obviously, natural language is not always the best choice of input when conducting visualization editing. Other forms of input, such as speech, mouse, touch, pen, etc., could also be combined together to support more multimodal interactions, leveraging the strengths of one modality to complement the weaknesses of others. 
% }




%One user (P9) learned to take advantage of the vagueness of natural language and said, ``When I am not sure what I want, I can try some vague descriptions and see what the system can give me. '' However, users also felt VisTalk interface gave them less sense of control. As P11 said, ``After getting used to the GUI interfaces, I am quite sure what will happen after I click one button. However, sometimes I am not sure what it turns out when I say a long sentences'' 

%\todo{for example, selector, fine-tuning can be conducted by mouse ... while users can use voice to state their requests}
%\cp{Users also mentioned that they wanted to have control of the precision of selections. In addition, we observed that users utilized the sliders to tweak effects. The sliders also served as a feedback mechanism for exploring the capabilities of the system (e.g., moving the slider swiftly back-and-forth between extremes)..}
%GUI - everything's in control. who's fault? judgement (fault notice/error message/let me know how to improve, or change)/Precision control


==> sections/UIST_discussion.tex <==
\section{Discussion}
\sherry{
This current discussion reads more like re-iterating many things we've already said before, e.g., editing actions as a bridge should be something section 3 already talked about extensively.
Some points I can think of:

\begin{compactenum}
\item Address the recommendation point in user study. Collect real world utterances to understand how people (with different backgrounds) give command in different tasks, different datasets, how to incorporate them into the framework.
\item Define finer-grained operation, so higher level operations can be a chain of lower-leveled ones, so we have a definitive set of operations (setChartType can be interpreted as xaxis, yaxis, etc.)
\item To help viz researchers better focus on the application part, release NL interpreters
\item Extension - more intents - can be more difficult to correctly parse the intents. Make use context to better understand users' intents 
\end{compactenum}
}
% \textbf{Editing Actions as a Bridge.}
% Due to the implementation challenges, prior natural language-based systems have to compromise the diversity and complexity of users' utterances.
% The design of natural language interpreter decouples the parsing tasks from the application that implements the commands. This method eases the difficulties of implementing natural language-based applications. NL-based authoring systems no longer need to implement a semantic parser themselves. Moreover, this also simplifies the maintenance of the natural language interpreter and improves the parsing performance. 
% %Our study of natural language-based authoring tools have demonstrated the effectiveness of using natural language to improve authoring experience. 

\wy{
\textbf{Understanding Utterances from People with Different Background}
From our user study, we find users may describe visualization design intents based on their own mental model of the design process. As mentioned in Section \ref{sec:model}, to create a chart from scratch, users can bind data columns to axes, so the chart type can be automatically inferred; users can start from a chart type and then modify the data fields, so the data binding and corresponding mark channels are obviously reflects; users can even start from a specification of mark (e.g., rectangle) and bind the data columns to different mark channels. To support better visualization creation experience, it might be interesting to understand different users' chart editing behaviors and the corresponding utterances. Editing actions can be further inferred more accurately. Moreover, the editing actions can be analyzed as sequences, so that users' follow-up editing actions can be predicted by the previous actions. 

\textbf{Visualization Design Paradigm.}
Visualization creating and authoring systems are usually designed based on different visualization conceptual models and design paradigms \cite{satyanarayan2019critical}. Users need to understand different design paradigms and get familiar with the user interfaces before making good use of authoring tools. 
However, different from WIMP systems, natural language authoring systems can provide a unified interface for different users. 
This makes the visualization creation experience more flexible and scalable. Expert users may easily switch between different mental models to optimize the process of creating typical chart, or more expressive visualizations. 
It also lowers the learning curve for users of different background. Novice users can start with basic chart and further modify and  customize the charts based on their needs.
However, this has poses new challenges for the implementation of such visualization creation tools to support seamless switch between different chart models. 
As future research, we consider to incorporate NL interpreter to multiple more advanced authoring systems to understand how the interpreters performs across different visualization systems.
}

% \textbf{Visualization Literacy}
% Users' behaviors towards natural language-based authoring systems may vary a lot based on their visualization literacy. Similar to the results of our formative study, the user study further confirms the differences among users with different background. Users with or without visualization expertise may have totally different mental models of creating charts \cite{}. However, natural language interfaces support unified interface for different users, which provides a better learnability. Users can simply switch among different creation process of visualizations.  



\wy{
\textbf{Designing Novel Visualization Tools to Support Multimodal Experiences.} 
The design of natural language interpreter decouples the parsing tasks from the application that implements the commands. This method eases the difficulties of implementing natural language-based applications. It may help visualization researchers better focus on the design of more natural interaction experience. 
In the future, we plan to collect more data on visualization editing and release the NL interpreters. This could lower the barriers of designing and developing novel natural language-based visualization construction techniques and tools.
For example, the authoring systems could design better experience for users to understand the vagueness and under-specification in their natural language input. It can also be challenging for users to understand system functions and how to describe their intents, a better natural language interaction experience should help users  enhance the recommendation of possible future actions to take.
Obviously, natural language is not always the best choice of input when conducting visualization editing. Other forms of input, such as speech, mouse, touch, pen, etc., could also be combined together to support more multimodal interactions, leveraging the strengths of one modality to complement the weaknesses of others. 
}
%One user (P9) learned to take advantage of the vagueness of natural language and said, ``When I am not sure what I want, I can try some vague descriptions and see what the system can give me. '' However, users also felt VisTalk interface gave them less sense of control. As P11 said, ``After getting used to the GUI interfaces, I am quite sure what will happen after I click one button. However, sometimes I am not sure what it turns out when I say a long sentences'' 

%\todo{for example, selector, fine-tuning can be conducted by mouse ... while users can use voice to state their requests}
%\cp{Users also mentioned that they wanted to have control of the precision of selections. In addition, we observed that users utilized the sliders to tweak effects. The sliders also served as a feedback mechanism for exploring the capabilities of the system (e.g., moving the slider swiftly back-and-forth between extremes)..}
%GUI - everything's in control. who's fault? judgement (fault notice/error message/let me know how to improve, or change)/Precision control




\textbf{Limitations.}
%- chart type-based (template based)
\sherry{This part is really implementation limitations, but as demonstrations they don't matter. I think we will want to discuss the potential limitations of frameworks, and how we want to address them in future work.}
\wy{More fine-grained taxonomy?}
As a first step, our current implementation of the natural language interpreter supports a set of common visualization operations. More operations can be included to support different visualization applications. Based on the deep learning model, the supporting operations can be expanded by extending the corpora with more users' utterances and the structured expressions corresponding to the functions of diverse visualization systems. Further enhancements are possible to cover more operations supported by popular authoring tools.
Similarly, the VisTalk prototype has a limited number of functions. VisTalk does make mistakes when encountering unfamiliar natural language patterns that are not covered in the training data. In the future, we plan to explore a method to automatically optimize the natural language model in the process of using the system. The system may learn from user inputs to improve its performance and the coverage of language patterns.

\todo{The current implementation binds table-related information before the intent and entity extraction. However, it may happen that data binding mistakenly bind tokens that are not related to tables. This method trades off the size of training dataset and improves the accuracy of the model for intent and entity extraction. In the future, we plan to collect a larger dataset and train a more robust end-to-end model. }

\wy{However, the capability of natural language understanding is still limited. %For example, the participants still hope to input more complex sentences that can help them process multiple table, or nested visualizations. This poses more challenges to understanding natural language. 
Our future research direction would involve more robust natural language interpreter that facilitate understanding of more complex utterances.}


==> sections/UIST_introduction-CHI.tex <==
\section{Introduction}
Natural language (NL) interfaces are becoming mainstream for modern applications thanks to their usability and learnability.
%seek better usability and learnability by supporting natural language 
%and have attracted visualization researchers' attention. 
Compared with traditional WIMP interfaces with complex menu items and mouse interactions, natural language-based systems require less prior knowledge on user interfaces, and users are not restricted to the locations of menus and buttons to create and edit visualizations~\cite{hoque2017applying, setlur2016eviza}. 

While the benefits are evident, the use of natural language interfaces for chart editing has yet to be ubiquitous. 




This is mainly because, for each individual visualization tool, it may take a                                                                              significant amount of work to support different sets of editing intents for users to construct visualizations with natural language. 
%supporting different set of edit operations and enabling users to construct their visualizations with natural language may take a significant amount of work for each individual visualization tool.

In fact, the laborious one-on-one mapping between the NL interface and the visualization tools may not be necessary.
While the low-level implementations are diverse, users' high-level intents of creating and editing visualizations are largely shared across applications.
For example, users typically need to change the underlying dataset, specify visual encodings, and adjust visual presentations (e.g., axes, legends, marks, layouts).
If we can model such intents as an intermediate layer between the natural language and the visualization tool, we can easily supply multiple tools with one universal natural language interface.

However, \emph{there has yet to be comprehensive guidance on how to model the intents of visualization editing.}
Existing visualization tools that support natural language interfaces \cite{dhamdhere2017analyza, gao2015datatone, setlur2016eviza, yu2019flowsense, srinivasan2017natural} 
only cover subsets of visualization editing operations, mostly for visual analytics purposes.
As a result, a richer set of flexible data binding and visual configurations in modern visualization creation toolkits~\cite{bostock2011d3, satyanarayan2016vega} and authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} are largely ignored. To enable the use of natural languages in more applications and scenarios, we need to first build a sufficient-enough set of ``intents-to-support.''

In this paper, we propose a framework for building natural language-based visualization systems (Figure~\ref{fig:pipeline}). 
Our framework has two main goals. First, to alleviate the burden of re-designing NL-interfaces per application, we decouples the natural language understanding (with \emph{a natural language interpreter}) and visualization editing command execution (by a \emph{visualization application}).
At the core of the framework is a set of \emph{editing actions}. 
These actions are machine-executable commands for modeling the aforementioned visualization editing intents.
They bridge users and visualization applications:
%These editing actions are pivotal and bridges users' NL utterances and applications' functions: \sherry{change authoring function to something else?}
the natural language interpreter parses users' utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.

Second, to provide a super set of what user intents to support, we  categorize common \emph{editing operations} based on extensive surveys on visualization construction tools.
By doing so, we can map each authoring action into well-defined \textit{editing operation} and its \textit{target objects}, and the corresponding \textit{parameters}. We validate our design by examining its compatibility with utterances for existing NL-based visualization tools.
With this framework, we highlight key factors to consider when implementing interpreters and applications, and demonstrate possible solutions of executing authoring actions and resolving the ambiguities in NL inputs.

We implement a proof-of-concept interpreter and a prototype application:
the interpreter takes the form of a deep sequence-labeling model, trained on a dataset that contains internally collected user utterances, as well as synthetic augmentations. The prototype application, VisTalk, supports natural language-based visualization authoring by integrating the interpreter.
%To assess our framework, we implement a deep-learning based natural language interpreter. The NL interpreter takes an NL utterance as input and ouputs a sequence of authoring actions.
%The interpreter can be integrated by different authoring tools to bring in natural language capabilities. 
%Further, we build a prototype application, VisTalk, which integrates the NL interpreter to support natural language-based visualization authoring. 
With VisTalk, we conduct an exploratory user study, where participants complete visualization reconstruction tasks with natural utterances.
Our observations shed light on future work:
we should consider how the interpreters can cope with users with different backgrounds, and how the applications can resolve ambiguities and make recommendations when users' initial command is not supported.
The contributions of this work are summarized as follows:





\begin{figure}[!t]
    \centering
    \includegraphics[width=0.45\textwidth]{pictures/workflow-new.pdf}
    \vspace{-10px}
    \caption{NL-based visualization construction framework. }
    \label{fig:pipeline}
    \vspace{-10px}
\end{figure}




\begin{compactitem}
    \item We summarize and formulate users' visualization editing intents as \textit{editing actions}, which are atomic units executable by applications. The introduction of such pivotal editing actions helps bridge the gap between natural languages and visualization applications.
    \item We propose an NL-based visualization editing framework that is equipped with a natural language interpreter to parse NL utterances into editing actions, and an authoring application to execute the editing actions.
    \item To illustrate the usage of the framework, we implement an example natural language interpreter that consists of three stages: data entry abstraction, information extraction, and editing action synthesis. We further build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. 
\end{compactitem} 




==> sections/UIST_introduction-UIST.tex <==
%With their intuitive interaction supports, flexible, easy-to-learn, 
\section{Introduction}
Natural language interfaces (NLIs), with their supports on intuitive, flexible, and easy-to-learn interactions, are becoming a mainstream for modern applications. 
%due to their usability, flexibility, and learnability. 
%Extensive research has been devoted to support natural language input and design better natural language interfaces for visualization applications. 
%For example, Analyza~\cite{dhamdhere2017analyza} parses analytic queries (\sutt{top three imdb rating movies in france}); 
%Orko~\cite{srinivasan2017orko} enables users to specify encodings (\sutt{color by country}); 
%FlowSense \cite{yu2019flowsense} lets users change the design (\sutt{set blue color});
%DataBreeze \cite{srinivasan2020interweaving} allows users to present charts with annotations (\sutt{add labels to the public schools}). 
%To augment NLIs, it requires not only deep understanding about both natural language processing knowledge and users’ possible natural language input to evoke system functions, but also a significant amount of efforts to develop the internal program. 
Various systems have been built to support natural language inputs in various data analysis and visualization scenarios, such as interactive analysis (\sutt{top three IMDB rating movies in france}~\cite{dhamdhere2017analyza}), chart annotations for presentations (\sutt{add labels to the public schools}~\cite{srinivasan2020interweaving}), encoding specification (\sutt{color by country}~\cite{srinivasan2017orko}), and design exploration (\sutt{set blue color}~\cite{yu2019flowsense}).
At the core of these systems are  the natural language (NL) interpreters that are \emph{tailored} to only process application-specific utterances.
Unfortunately, the interpreters are hard to design and implement, as they require deep understanding about both natural language processing knowledge and users’ possible natural language input to evoke system functions. 

However, the NL interpreter does not have to be application-specific, as users’ intents of interacting with visualizations are largely shared across applications.
% \wy{For example, users may want to specify colors in design \emph{and} in analysis and annotations (e.g., for highlighting parts of the charts.)} As such, 
Recent studies have explored adopting reusable NL interpreters to alleviate the burden of redesigning NL-interfaces per application.
In specific, NL4DV~\cite{narechania2020nl4dv} provides a framework and a toolkit that generates reusable analytic specifications from NL inputs. 
It defines chart specifications as an intermediate layer between its NL interpreter and various visualization tools to decouple the two, such that the interpreter only needs to translate user utterances to the analytic specifications independent of downstream visualization implementations, whereas the downstream tools only need to create the visualizations based on the specifications, without concerning the NL inputs.

%In fact, users’ intents of creating visualizations are largely shared across applications. The laborious one-on-one implementations of NLIs for the visualization tools may not be necessary. Recent study has suggested to support application systems with reusable NL interpreters, so that the significant amount of work to support NLIs can be saved \cite{sarmah2020geno} . For example, NL4DV \cite{narechania2020nl4dv} has provided a toolkit for generating analytic specifications from NL input. This approach supports the translation of  users’ utterances to analytic tasks (e.g., correlation, filter) and the related data attributes. Chart specifications are then generated by heuristic rules that maps analytic tasks to chart types. The output specifications serve as an intermediate layer between natural language and visualization tools where visualization applications can reuse the natural language interface.

%Such way of decoupling the natural language understanding and visualization applications is promising, but the automatically generated charts may not be perfect to cater diverse needs. 
%Users may require to conduct \textit{chart editing} to adjust the data encoding and attributes of the charts to facilitate their understanding about data \cite{srinivasan2021collecting}. 
%Moreover, when charts used for data presentation and communications, users may enhance the expressiveness of data charts by adjusting the styles (e.g., change color schemes), and add annotations (e.g., trendlines).
%When conducting chart editing with WIMP interfaces, users need to understand the complex menu items and mouse interactions. The interactions are restricted to the locations of menus and buttons to edit visual charts~\cite{hoque2017applying, setlur2016eviza}. Augmenting the systems with NLIs can reduce the learning curve and enhance accessibility of the chart editing functions.

While such decoupling is promising, the design of general-purpose NLI framework only focuses on the \emph{generation} of the visualization based on analytic tasks. We argue that an equally essential, yet currently missing, usage scenario of NLI is on \emph{editing} of existing charts.
Chart editing is ubiquitous, as users frequently explore and understand their data by adjusting the data encoding and chart attributes~\cite{srinivasan2021collecting}.
In the case of data presentation and communications, users may enhance the expressiveness of data charts by adjusting the styles (\eg change color schemes) and adding annotations (\eg trendlines).
Most \emph{status-quo} chart editing is completed with WIMP interfaces (``windows, icons, menus, pointer''), where users are required to understand complex menu items and mouse interactions~\cite{hoque2017applying, setlur2016eviza}. 
Augmenting systems with NLIs can reduce the learning curve and enhance the accessibility of the chart editing functions~\cite{laput2013pixeltone}.

Extending the NLI support from chart generation to chart editing is nontrivial. 
The primary challenge is that there has yet to be a shared abstraction of user intents on chart editing. On the one hand, widely-adopted visualization grammars such as Vega-Lite \cite{satyanarayan2016vega}  describe static charts, and cannot represent chart editing intents. 
On the other hand, existing visualization applications for chart creation and editing (e.g., Excel, Tableau, Charticulator \cite{Ren_2019_8440827}) do not explicitly formulate the editing operations as extensible and reusable representations.
Even with a formal representation, interpreting user intents from utterances is challenging, as the utterances can be vague (e.g., \sutt{change color to navy blue}) and frequently depend on the existing visualization (e.g., \sutt{on the top of the blue bar}) \cite{metoyer2012understanding}. 



In this paper, we extend the NLI framework to chart editing, by designing (1) formal abstractions of chart editing intents that can be executable across visualization applications, as well as (2) disambiguation methods for handling vague user utterances.
First, through extensive surveys on common editing operations in existing visualization tools, we present the abstraction as a set of \emph{editing actions}, which can be mapped to well-defined editing operations, their target objects, and the corresponding parameters (Figure~\ref{fig:taxonomy}).
Similar to specifications in NL4DV, the editing actions effectively bridge users and visualization applications by  decoupling the natural language understanding and chart editing execution.
%the natural language interpreter parses users’ utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.
Additionally, to characterize the implicit reference of objects, we define object selectors and object naming representations; to characterize ambiguous properties, we design vague parameters and relational parameters so that user intents can be described in a finer granularity. 
%We validate our design by examining its compatibility with utterances for existing NL-based visualization tools.
We compare our taxonomy with existing NL-based visualization tools, and show that we comprehensively cover a wide range of editing operations. 
We further discuss the scope differences between prior work and ours.

%In this paper, we present a set of editing actions, which are machine executable commands for modeling the chart editing intents. The editing actions bridge users and visualization applications by decoupling the natural language understanding and chart editing execution: the natural language interpreter parses users’ utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.

%We categorize common editing operations based on extensive surveys on chart creation tools. \wy{add our formative study?} By doing so, we can map each editing action into well-defined editing operation and its target objects, and the corresponding parameters. To characterize the implicit and ambiguous natural language input, we design object selectors, vague parameters, and relational parameters so that users' intents can be described in a finer granularity. We validate our design by examining its compatibility with utterances for existing NL-based visualization tools. 

Based on the editing actions, we design and implement a proof-of-concept NL interpreter for chart editing. The interpreter takes the form of a multi-stage pipeline: 
it first recognize data entities and replace them with abstract arguments; 
then, it uses a deep sequence-labeling model to extract intents and entities from the abstracted utterances; 
finally, it synthesizes the extracted information into a sequence of editing actions.
With the deep model, we envision that the interpreter can be easily extended as we collect a larger knowledge base of editing utterances.
%We view the supporting editing actions in the interpreter as a starting point of an evolving knowledge base of editing utterances that can be extended. 

We demonstrate the utility of our interpreter with two example applications, \ie a natural language-based chart creation tool called VisTalk, and an Excel add-in for chart specification. We further conduct an exploratory user study, where participants complete chart reconstruction tasks with natural utterances. Our observations shed light on future work: we should consider how the interpreters can cope with users with different backgrounds, and how the applications can resolve ambiguities and make recommendations when users’ initial command is not supported. The contributions of this work are summarized as follows:

\begin{compactitem}
\item We summarize and formulate users’ chart editing intents as editing actions executable by applications. The introduction of such pivotal editing actions helps bridge the gap between natural languages and chart editing scenarios.
\item We develop a natural language interpreter to parse NL utterances into editing actions. We then demonstrate the utility of the NL interpreter with two visualization applications.
\item We conduct a user study to understand how users can construct and edit data charts through natural language. We further discuss the strengths and limitations of NL-based chart editing based on our observations.
\end{compactitem}

==> sections/UIST_introduction.tex <==

%NL interfaces are widely used
%however, different systems support different visaulization edit and authoring operations
%we propose a framework to decouple the nl understanding and application execution
% advantage: nl interpreter can be reused and easily extended
% we build example nl interpreter and application
% in the future, we will collect more data and release nl interpreter.



\section{Introduction}

Natural language (NL) interfaces are becoming mainstream for modern applications thanks to their usability and learnability.
%seek better usability and learnability by supporting natural language 
%and have attracted visualization researchers' attention. 
Compared with traditional interfaces with complex menu items and mouse interactions, natural language-based systems require less prior knowledge on user interfaces, and users are not restricted to the locations of menus and buttons~\cite{hoque2017applying, setlur2016eviza}. %Therefore, fewer efforts are taken for users to interpret their intentions into the system's allowed functions. 
%\sherry{Is ``visualization editing operations'' a well-defined term across the viz community? If not, we might need to add a one sentence description for it? Also, this phrase is making both sentences exceptionally long.}
\srevise{
Despite the benefit, the use of natural language interface has yet to be ubiquitous in visualization tools due to two challenges.

First, \emph{there has yet to be a comprehensive guidance on what interactions an NL interface should supply.}
Existing visualization tools that support natural language interfaces \cite{dhamdhere2017analyza, gao2015datatone, setlur2016eviza, yu2019flowsense, srinivasan2017natural} 
only cover subsets of visualization editing operations (mostly for visual analytics purposes).
As a result, a richer set of flexible data binding and visual configurations in modern visualization creating toolkits~\cite{bostock2011d3, satyanarayan2016vega} and authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} are largely ignored.
Conversely, to enable the use of natural languages in more scenarios, we need to first build a well-scoped set of ``operations-to-support.''
Second, with each tool following different design paradigms~\cite{satyanarayan2019critical}, \emph{it is challenging to consider the space of acceptable utterance per application.}
In other words, customizing NL interfaces for each visualization application can  take a significant amount of work.
That said, we note that the one-on-one mapping between the NL interface and the visualization tools may not be necessary.
While the low-level implementations are diverse, users' high-level intents of creating, editing, and authoring visualizations are largely shared across applications.
For example, users typically need to change the underlying dataset, specify visual encodings, and adjust visual presentations (e.g., axes, legends, marks, layouts).
As a result, if we can model such intents as an intermediate layer between the raw natural language and the visualization tool, we can easily supply multiple tools with one universal NL interface.
}



\begin{comment}
%%% new commented
Usually existing visualization tools that support natural language interfaces \cite{dhamdhere2017analyza, gao2015datatone, setlur2016eviza, yu2019flowsense, srinivasan2017natural} only cover subsets of visualization editing operations for visual analytics purposes, largely ignoring a richer set of flexible data binding and visual configurations in modern visualization creating toolkits~\cite{bostock2011d3, satyanarayan2016vega} and authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827}. Supporting this broader set of edit operations and enabling users to construct their visualizations with natural language may take a significant amount of work for each individual visualization tool.
\end{comment}
%Extending the existing NL-based systems to understand more operations through natural language, or enabling existing visualization tools to understand natural language, both requires great amount of efforts to design natural language understanding modules according the requirement of these tools.
%than traditional visualization tools. 
%Nevertheless, they involve complicated GUIs and incur a steep learning curve, especially for novice users. While natural language interfaces are promising in lowering the barrier of using advanced visualization authoring tools, unfortunately none of these systems currently support natural language interfaces.

%more flexible data binding and configurations for marks, layouts, annotations, and so on. Users can manipulate visualizations and graphical elements by pointing to the objects, finding configuration menus, and applying predefined functions.

%Contrary to the visualization analytics systems for data analysis, recent authoring systems \cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support more flexible data binding and configurations for marks, layouts, annotations, and so on. Users can manipulate visualizations and graphical elements by pointing to the objects, finding configuration menus, and applying predefined functions. %Theses systems support flexible and advanced authoring requests by direct manipulation of graphical elements and user menus. Users can point to the objects, find the configuration menus, and apply predefined functions carefully.  However,
%learning such complicated functions and adapt-ing to new user interfaces is often time-consuming and cumbersome,especially for novices.
%However, learning such complicated functions and adapting to new user interfaces is often time-consuming and cumbersome, especially for novices. Unfortunately, none of these systems support the usages of natural language.

% One major challenge of applying natural language interfaces for visualization authoring systems is the complexity of authoring operations. Various authoring systems may employ different visualization models and take notably different approaches to optimizing authoring interactions. A same authoring intent is defined as different internal functions across applications~\cite{satyanarayan2019critical}. \todo{very different cannot lead to the huge gap?}With a lack of a unified representation or grammar of visualization authoring intents, there is a huge gap to convert high-level natural language inputs from users to low-level authoring operations implemented by applications.


%One major challenge of applying natural language interfaces for visualization authoring systems is the huge gap between high-level natural language inputs from users and low-level authoring operations implemented by applications. Advanced authoring systems may employ notably different visualization models to optimize authoring interactions. A same authoring intent may be defined as different internal functions across applications~\cite{satyanarayan2019critical}. Without a widely-adopted representation or grammar of visualization authoring intents, it is difficult to model users' natural language authoring utterances.

\begin{comment}
%%% new commented
In fact, the one-on-one mapping between the NL interface and the visualization tools may not be necessary.
While the low-level implementations are diverse, users' high-level intents of creating, editing, and authoring visualizations are largely shared across applications.
For example, users typically need to change the underlying dataset, specify visual encodings, and adjust visual presentations (e.g., axes, legends, marks, layouts).
As a result, if we can model such intents as an intermediate layer between the raw natural language and the visualization tool, we can easily supply multiple tools with one universal NL interface.
\end{comment}

%While the low-level implementation of visualization tools and systems are diverse, users' intents of creating, editing, and authoring visualizations share a large set of overlaps across applications. 
%For example, users typically needs to change the underlying dataset, adjust visual encodings, and conduct changes on visualization styles of axes, legends, marks, layouts, and annotations.

\srevise{
Based on these observations, we propose a framework for building natural language-based visualization systems (Figure~\ref{fig:pipeline}). 
Our framework has two main goals:
First, to alleviate the burden of re-designing NL-interfaces per application, we \textbf{decouples the natural language understanding (with \emph{a natural language interpreter}) and visualization editing command execution (by a \emph{visualization application}).}
At the core of the framework is a set of \emph{editing actions}. 
These actions are machine-executable commands for modeling the aforementioned visualization editing intents.
They bridge users and visualization applications:
%These editing actions are pivotal and bridges users' NL utterances and applications' functions: \sherry{change authoring function to something else?}
the natural language interpreter parses users' utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.

Second, to provide a checklist on what user intents to support, we \textbf{explicitly categorize common \emph{editing operations} abased on extensive surveys on visualization construction tools.}
By doing so, we can map each authoring action maps users' editing intent can into well-defined \textit{editing operation} and its \textit{target objects}, and the corresponding \textit{parameters}.
\srevise{We validated our design by ensuring it is compatible with the utterances in existing NL-based visualization tools.}
}

\begin{comment}
%%% new comment
Based on these observations, we propose a framework for building natural language-based visualization systems (Figure~\ref{fig:pipeline}). 
It decouples the natural language understanding (with \emph{a natural language interpreter}) and visualization editing command execution (by a \emph{visualization application}). 
At the core of the framework is a set of \emph{editing actions}. 
%\wy{After surveying a number of visualization construction tools, we define editing actions as the combination of operations, objects, and parameters. }
These actions are machine-executable commands for modeling the aforementioned visualization editing intents.
They bridge users and visualization applications:
%These editing actions are pivotal and bridges users' NL utterances and applications' functions: \sherry{change authoring function to something else?}
the natural language interpreter parses users' utterances into a sequence of such editing actions, and the actions can then be adapted and executed by the applications.
%explore the usage of natural language interfaces for visualization authoring systems. 
%We design a natural language-based authoring framework with a natural language interpreter that can parse users' utterances into a sequence of authoring actions. 
%, which are used as an abstract layer to bridge users' utterances and different authoring applications. 
\end{comment}


%\sherry{I moved/rephrased the first half of this paragraph above, but dont know what to do with the second part. I think we can just cut it? I assume because you cut some additional model stuff, ``first step'' doesn't make sense anymore; Plus for short paper we don't need to go into such detail?}
%We summarize common editing interactions and formulate them into \textit{editing actions} in the forms of operation, objects, and parameters to model natural language intents into machine-executable commands. As a first step, we summarize the most common authoring operations and categorize them into six major groups, namely data operations, encoding operations, annotate operations, styling operations, layout operations, and view manipulations. 

%On the top of the model, we design a deep learning-based natural language interpreter that parses users' utterances into a list of authoring actions, which can be further adapted and executed by authoring applications. 
%Authoring actions can be further adapted and executed by authoring applications' internal functions.
%This could result in different experiences of using natural language to describe authoring requirements, which may confuse users and decrease the learnability of natural language-based authoring systems.
As a proof-of-concept, we implement a sample interpreter and a prototype application:
The interpreter takes the form of a deep sequence labeling model, trained on a dataset that contains internally collected user intents, as well as synthetic augmentations.
The prototype, VisTalk, supports natural language-based visualization authoring by integrating the interpreter.
%To assess our framework, we implement a deep-learning based natural language interpreter. The NL interpreter takes an NL utterance as input and ouputs a sequence of authoring actions.
%The interpreter can be integrated by different authoring tools to bring in natural language capabilities. 
%Further, we build a prototype application, VisTalk, which integrates the NL interpreter to support natural language-based visualization authoring. 
\srevise{
With VisTalk, we highlighted key factors to consider when implementing interpreters and applications, and demonstrated possible solutions of executing authoring actions and resolving the ambiguities in NL inputs. 
We further used VisTalk in an exploratory user study, where participants completed visualization reconstruction tasks with natural utterances.
Our observations shed light on future work:
We should consider how the interpreters can cope with users with different backgrounds, and how the applications can make recommendations when users' initial command is not supported.
}
The contributions of this work are summarized as follows:





\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\columnwidth]{pictures/workflow-new.pdf}
    \vspace{-10px}
    \caption{NL-based visualization construction framework. }
    \label{fig:pipeline}
    \vspace{-10px}
\end{figure}




%We leverage VisTalk to conduct a user study to understand the effectiveness of natural language-based authoring systems. Our results confirm the effectiveness of natural language-based authoring for novice users. The study also reveals space of improvement for future research on natural language-based visualization authoring systems.

\begin{compactitem}
    \item We summarize and formulate users' intents as \textit{editing actions}, which are atomic units executable by applications. The introduction of such pivotal editing actions helps bridge the gap between natural languages and visualization applications.
    \item We propose an NL-based visualization editing framework that is equipped with a natural language interpreter to parse NL utterances into editing actions, and an authoring application to execute the editing actions.
    \item To illustrate the usage of the framework, we implement an example natural language interpreter that consists of three stages: data entry abstraction, information extraction, and editing action synthesis. We further build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. 
\end{compactitem} 






















% %with rule-based methods, which can be hard to generalize. 
% %Modern authoring tools however require the support of much more abundant and complex functions. The intents from human users can thus be more complex and diverse. This poses new challenges for the design of natural language tools. 



% % {\fontfamily{helveticaneue}\selectfont \{place, legend, position=[plot]right\}}\\
% % {\fontfamily{helvet}\selectfont \{place, legend, position=[plot]right\}}\\
% % {\fontfamily{lmss}\selectfont \{place, legend, position=[plot]right\}}

% %Visualization becomes increasingly popular for storytelling. There are growing interests of create visualization for communication and presentation. 
% A number of visualization authoring systems have emerged to enable the authoring of expressive visualizations. Contrary to the traditional visualization systems for data analysis, recent visualization authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support more flexible data binding and configurations for marks, layouts, annotations, and so on. 
% %\todo{how complex are the authoring operation?}
% %For example, data-driven guides \cite{Kim_2017_7536218}, DataInk \cite{xia2018dataink}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909} support data binding with hand-drawn or vector shapes; %InfoNice \cite{Wang:2018:IEC:3173574.3173909} enables the creation of expressive visualizations through mark customization; 
% %Data illustrator \cite{Liu:2018:DIA:3173574.3173697} proposes repeat and partition features for creative design of visualizations.
% These systems support flexible and advanced authoring requests by direct manipulation of graphical elements and user menus. Users can point to the objects, find the configuration menus, and apply predefined functions carefully. However, learning such complicated functions and adapting to new user interfaces is often time-consuming and cumbersome, especially for novices. 
% %Mouse and touch interaction can also be inefficient for complex visualization design%, especially when the interfaces themselves are also complex
% %\cite{hoque2017applying}. 
% %There are many barriers to learning and adapting to new user interfaces especially for novices.
% %However, they have restricted the target users to "graphic designers". General users without visualization design knowledge are hard to understand visual encoding. InfoNice adopts a "mark customization" approach. However, ...Users still need to learn and get familiar with the interface to implement their design. 

% %As a promising interaction paradigm, natural language has the potential to offer advantages to address these issues. 
% In contrast, natural language interfaces have attracted researchers' attention thanks to its learnability and usability. Compared with traditional interfaces with complex --- but sometimes still insufficient --- menu and mouse interactions~\cite{hoque2017applying}, natural language-based systems require less prior knowledge \cite{setlur2016eviza}. Users are not restricted to the functions and locations of the buttons. Therefore, fewer efforts are taken for users to interpret their intentions into the system's allowed functions. Researchers have conducted research on natural language interfaces for visual analytics \cite{dhamdhere2017analyza, gao2015datatone, yu2019flowsense}. 
% However, most of them focus on visual data exploration and support basic natural language data query with rule-based methods, which can be hard to generalize. 
% Modern authoring tools however require the support of much more abundant and complex functions. The intents from human users can thus be more complex and diverse. This poses new challenges for the design of natural language tools. 
% %support the natural language module by NL-based data query. 

% To fill this gap, we explore the usage of natural language interfaces for visualization authoring systems. 
% Prior work of authoring tools have emerged to provide powerful authoring interactions for users. However, 
% these systems take notably different approaches to optimizing authoring interactions and ease the creation of expressive visualizations \cite{satyanarayan2019critical}. With different menus and interactions, authoring operations are defined as different internal functions across applications. This could result in different experiences of using natural language to describe authoring requirements, which may confuse users and decrease the learnability of natural language-based authoring systems.
% %difficulties of natural language interactions. For instance, the same keyword ``highlight'' may result in different interpretation for different platforms, 


% In response, we explore a natural language-based authoring framework
% with a unified authoring action grammar. To achieve this, we conduct a formative study to understand how users might express their authoring intents. %There are three main findings from the study. First, users might use different workflows for different types of authoring scenarios. Second, natural language utterances may contain fuzzy reference and vague modifiers for parameters. Third, users tend to mix multiple intents in one sentence. 
% Based on the study, we formulate common authoring features into authoring actions in the form of operation, object, and parameter to model natural language intents into machine-executable commands. As a first step, we list most common authoring operations and categorize them into six major groups.  
% %On the top of the model, we design a deep learning-based natural language interpreter that parses users' utterances into a list of authoring actions, which can be further adapted and executed by authoring applications. 
% Authoring actions can be further adapted and executed by authoring applications. 
% The authoring actions are used as an abstract layer to bridge users' utterances and different authoring applications.

% We implement an natural language interpreter with a deep learning-based model, that takes human utterances as input and ouputs a sequence of authoring actions. The interpreter can be integrated by different authoring systems to bring in natural language interfaces. Authoring systems can adapt and execute authoring actions with local authoring functions.  This
% helps enhance the capability of natural language understanding for authoring tools. For users especially novices, this approach reduces the barriers of learning and using visualization authoring systems for different users across applications. %The framework takes natural language as input and parses users' utterances through the natural language interpreter and outputs a list of \textit{authoring actions}. The output can be further executed by visualization authoring systems to respond to users' input and make changes to the visualizations.



% % To evaluate our framework, 
% % We then conducted user study to understand how users interact with the NL-based visualization authoring system.
% % Through our study, we show the benefits and pitfalls of using NL-based method for visualization authoring.

% To assess this framework, we build an example web authoring system, VisTalk, based on the natural language interpreter. We demonstrate the possible ways of executing authoring actions and resolve ambiguities in users' natural language inputs.
% Further, we leverage VisTalk to conduct a user study to understand the effectiveness of natural language-based authoring systems. Results reveal the benefits and weaknesses of VisTalk \todo{expand a bit}, inspiring future research directions for natural language-based authoring systems.
% %Users need to practice using the GUIs to accelerate their design process.
% %Drawbacks for the GUI for visualization authoring systems:
% %Users need to learn the different design process/logic behind the system one by one The GUI changes significantly across systems to support different user groups/needs. As a result, users need to switch between tools, learn different interface when they have different needs
% %In this paper, we explore a natural language framework for Visualization authoring. 
% The contributions of this work are summarized as follows:
% \begin{compactitem}
%     \item We conduct a formative study on how users express their visualization authoring intents with natural language. We summarize and formulate authoring intents as \textit{authoring actions}, which are atomic units executable by applications, to bridge the gap between natural languages and authoring applications.
%     \item We build a deep learning-based natural language interpreter to parse from their input utterances into authoring actions. The natural language interpreter consists of three stage, token recognition, intent and entity extraction, authoring action synthesis.
%     \item To illustrate the usage of the framework, we build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. With this system, we conducted a user study to understand the effectiveness of NL-based authoring experience. 
% \end{compactitem} 




==> sections/UIST_related-work.tex <==

\section{Related Work}

\subsection{Natural Language Interfaces for Visualization}
Natural language interfaces have been widely adopted to improve the usability of visualization systems. 
Extensive research has been devoted to a better experience of using natural language for data analytics~\cite{srinivasan2017natural}. 
To complete the analytical tasks, they treat user input utterances as natural language queries, and translate them to logic query languages~\cite{androutsopoulos1995natural}, such as XML~\cite{li2007nalix}, and SQL~\cite{zhong2017seq2sql}. 
Researchers further study the interactive visual analytic systems that support natural language queries.
Wen \etal~\cite{wen2005optimization} designed a system to update the visualizations based on user queries dynamically. 
Articulate~\cite{aurisano2016articulate2} generates a graph to select proper visualizations to answer users' natural language questions and complete analytic tasks.
Orko~\cite{srinivasan2017orko} is a natural language system for network data exploration.
FlowSense~\cite{yu2019flowsense} applies natural language techniques to dataflow visualization systems.
Commercial tools like IBM Watson Analytics~\cite{ibm}, Microsoft Power BI~\cite{pbi}, ThoughtSpot~\cite{ThoughtSpot}, and Google Spreadsheet~\cite{dhamdhere2017analyza} also  automatically translate the natural language questions to data queries. \revise{The systems present query results with visualizations based on heuristics, but limit NL interactions to data queries. We propose the abstractions of editing actions and develop the NL interpreters, so that applications can further extend the capability of NLIs to chart editing. }

%to address ambiguity problems in natural language
Researchers also try to address ambiguity problems through different means. On the one hand, researchers try to address ambiguity problems through the design of interactive systems to invite users to clarify their requests. For example, DataTone \cite{gao2015datatone} introduces interactive widgets to address ambiguity problems.
Eviza \cite{setlur2016eviza} further enhances interactions by providing graphical answers that can be directly manipulated. 
Iris~\cite{fast2018iris} is a conversational interface that enables users to combine commands through many rounds of question-answering.
%pragmatics principles
On the other hand, design principles are also summarized to improve the understanding of users' utterances.
To enhance natural language interactions, Hoque \etal \cite{hoque2017applying} apply pragmatics principles and propose a theoretical framework for interaction with visual analytics.
Hearst \etal \cite{hearst2019toward} conduct an empirical study to explore default visualizations for vague expressions in natural language queries. Similarly, Setlur \etal \cite{setlur2019inferencing} explore inferring underspecified natural language queries and propose a systematic approach to resolve partial utterances. We propose abstractions of editing actions to represent underspecified utterances in a structured form. Visualization applications that executes the editing actions can follow the design rules to resolve ambiguities in these utterances.

%we are different from natural language query 
Existing work enables natural language interfaces in a case by case manner. \revise{To support easier development of visualization systems with NLIs, recent work by Narechania et al. \cite{narechania2020nl4dv} provides a toolkit for generating analytic specifications from natural language queries. Visualization applications can generate visualization by executing the JSON output of NL4DV.
However, chart editing intents, including modifying and specifying chart types, encoding, and design are also ubiquitous in the process of chart construction \cite{srinivasan2021collecting}. There is still a lack of support of NLIs for chart editing. }
To fill this gap, we design a general natural language framework for chart editing, which aims to enable common visualization tools to understand natural language-based chart editing commands. With natural language interfaces supported, users can simply state their editing goals without learning the graphical interfaces. The design and implementation of the natural language interpreter can be reused across applications and tools. 
\revise{To achieve this goal, we design editing actions to depict users' utterances of chart editing. We further develop a natural language interpreter that parses NL utterances into executable editing actions.}
%to let users give commands on the "editing operations" to the visualization and do the customization for their visualization design.




\subsection{Visualization Creation Tools}
A variety of visual authoring approaches have been proposed to facilitate visualization creation. For example, Polaris~\cite{Stolte2000PolarisAS}, Tableau~\cite{tableau}, and Many Eyes~\cite{ibm} help users to conduct data encoding with visual channels in a visualization. These tools enable users to create visualizations in a short time, but they are less flexible. The resulting visualizations are usually standard visual charts. More advanced techniques, such as Lyra~\cite{satyanarayan2014lyra} and iVisDesigner~\cite{6876042}, have been proposed to enable more expressive visualization designs. With these systems, users can easily specify properties of graphical marks and bind them with data. However, these systems only support the modifications of properties by adjusting a set of style parameters. Later, data illustrator~\cite{Liu:2018:DIA:3173574.3173697} uses repetition and partition operators for multiplying marks and generating data-driven expressive visualizations. Charticulator~\cite{Ren_2019_8440827} also adopts a bottom-up approach to bind data fields to vector graphics and build visualization with an emphasis on visualization layouts.
Recently, Data-Driven Guides~\cite{Kim_2017_7536218} have allowed users to draw and design graphical shapes to achieve creative designs. Similarly, DataInk~\cite{xia2018dataink} and InfoNice~\cite{Wang:2018:IEC:3173574.3173909} also bind graphical elements with data fields to facilitate the generation of creative visualizations.

Researchers have explored the design of visualization authoring systems and supported the creation from different perspectives. \revise{However, they have different design of graphical user interfaces. This requires additional efforts for users to learn the graphical user interface across various chart design applications. Integrating natural language interfaces into chart editing process of visualization systems can enhance the learnability and usability of these tools.}
%To support visualization creation, the systems have different internal logics.
%, which can be basically divided into three categories, namely template editors, shelf construction, and visual builders \cite{satyanarayan2019critical}.
We summarize and categorize the most common functions used in the systems, and further formulate the functions as editing actions, which is an abstract layer that bridges human intents and chart editing functions. \revise{The NL interpreter can translate user utterances to editing actions that can be executed by different visualization tools.}

% % Visualization systems have been proposed to ease the creation of visualizations

% % - template editors
% % - shelf construction
% % - visual builders

==> sections/VIS_appendices.tex <==
\section{Editing actions} \label{app:actions}

Operations may apply to different objects, depending on the properties of the objects. 
Table 1 lists the operations and the corresponding target objects and possible parameters. 
Operations are not exclusive because human languages may express same meanings with different patterns. For example, binding a data field to x axis, has the same effect as encode the horizontal position of mark to the field. Note the operations are not exhaustive.  

\begin{table*}[h]
    \centering
    \includegraphics[width=1\linewidth]{pictures/new-taxonomy-cropped.pdf}
    \vspace{0px}
    \caption{An authoring action consists of three parts, operation, object, and parameter. The table shows example authoring operations and the  corresponding objects and parameters. Operation are categorized into six major groups. Objects are categorized into chart components (e.g., axes, legends, title), mark channels (e.g., shape, color, size, position), and annotations (e.g., reference lines, reference bands, trend lines). }
    \label{fig:taxonomy1}
    \vspace{-1px}
\end{table*}


==> sections/VIS_conclusion.tex <==

\section{Conclusion}
In this paper, we explore a natural language-based authoring framework, which supports the understanding of authoring commands. The framework is motivated by a formative study with novice and professional users. In the study, the users make use of natural language to indicate the visual charts they want to create, and the changes they would like to make to author the expressive visualizations. Visualization authoring is a difficult and complex task. The visualization model and language of visualization manipulation are varied across users and authoring systems. Therefore, the natural language tends to be ambiguous and subjective. Therefore, we propose a visualization authoring grammar that describes users' unstructured statements with multiple structured expressions.
Our natural language-based authoring framework adopts a state-of-the-art deep learning model, to extract multiple intents and arguments from users' utterances and synthesis the executable expressions.
To demonstrate the usage of our framework, we further design a natural language-based visualization authoring tool, VisTalk. VisTalk takes the expressions as inputs, and further parses the expressions based on the visualization model and the states of users' authoring. By integrating a number of dynamic widgets, VisTalk implements a multimodal interface that can help users naturally and easily clarify their intentions. Through a user study with VisTalk, we find that the natural language interface provides a flexible mechanism to obtain users' desired authoring results. 

==> sections/VIS_discussion.tex <==
\section{Discussion}
\textbf{NL Interpreter as a Bridge.}
Due to the implementation challenges, prior natural language-based systems have to compromise the diversity and complexity of users' utterances.
The design of natural language interpreter decouples the parsing tasks from the application that implements the commands. This method eases the difficulties of implementing natural language-based applications. NL-based authoring systems no longer need to implement a semantic parser themselves. Moreover, this also simplifies the maintenance of the natural language interpreter and improves the parsing performance. 
Our study of natural language-based authoring tools have demonstrated the effectiveness of using natural language to improve authoring experience. 
However, the capability of natural language understanding is still limited. For example, the participants still hope to input more complex sentences that can help them process multiple table, or nested visualizations. This poses more challenges to understanding natural language. Thus, a future research direction would involve more robust natural language interpreter that facilitate understanding of more complex utterances.


% \textbf{Visualization Literacy}
% Users' behaviors towards natural language-based authoring systems may vary a lot based on their visualization literacy. Similar to the results of our formative study, the user study further confirms the differences among users with different background. Users with or without visualization expertise may have totally different mental models of creating charts \cite{}. However, natural language interfaces support unified interface for different users, which provides a better learnability. Users can simply switch among different creation process of visualizations.  


\textbf{Visualization Design Paradigm.}
Visualization authoring systems are usually designed based on different visualization conceptual models and design paradigms\cite{satyanarayan2019critical}. Users need to understand different design paradigms and get familiar with the user interfaces before making good use of authoring tools. Different from WIMP systems, natural language authoring systems can provide a unified interface to simultaneously support operations under multiple design model.
For example, users can bind a data column to an axis, or bind the data column to the mark channel; users can start from a chart type and then modify the data binding and chart components, or start from a specification of mark and let it serve as a component of another chart.
This makes the authoring experience more flexible and scalable. It also lowers the learning curve for users of different background. Users can easily switch among different design paradigms, which significantly eases the authoring process.
As a first step, current implementation of NL interpreter only covers basic authoring operations. As future research, we consider to incorporate more advanced authoring operations and support a more complete set of authoring operations for common visualization authoring systems.


\textbf{Designing Novel Tools and Experiences.}
For natural language interfaces, it can be challenging for users to think of what to say and how to say \cite{srinivasan2019discovering}.  
The design of a natural language interpreter enhances the semantic parsing of users' intents, resulting into better understanding of users' input. One user (P9) learned to take advantage of the vagueness of natural language and said, ``When I am not sure what I want, I can try some vague descriptions and see what the system can give me. '' However, users also felt VisTalk interface gave them less sense of control. As P11 said, ``After getting used to the GUI interfaces, I am quite sure what will happen after I click one button. However, sometimes I am not sure what it turns out when I say a long sentences''  Researchers have designed novel multimodal systems that combine mouse, voice, touch, or even pen. As a further step, novel designs of multimodal authoring tools have the potentials to improve the experience of authoring and address the issues brought by the ambiguities of human language. With the improvement of the natural language interpreter, novel authoring techniques and tools should be explored in the future. 
%\todo{for example, selector, fine-tuning can be conducted by mouse ... while users can use voice to state their requests}
%\cp{Users also mentioned that they wanted to have control of the precision of selections. In addition, we observed that users utilized the sliders to tweak effects. The sliders also served as a feedback mechanism for exploring the capabilities of the system (e.g., moving the slider swiftly back-and-forth between extremes)..}
%GUI - everything's in control. who's fault? judgement (fault notice/error message/let me know how to improve, or change)/Precision control




\textbf{Limitations.}
%- chart type-based (template based)
As a firs step, our current implementation of the natural language interpreter supports a set of basic common visualization authoring operations. However, more operations can be included to support different visualization authoring systems. Based on the deep learning model, the supporting operations can be expanded. The model can be further trained by a corpora consisting of more users' utterances and the structured expressions corresponding to the functions supported by the authoring systems. Further enhancements are possible to cover more operations supported by popular authoring tools.

Similarly, the VisTalk prototype has a limited number of functions. Although the performance of the system is quite high, there might be more ambiguity problems with the increase of system complexity. Nonetheless, VisTalk does make mistakes when encountering unfamiliar natural language patterns that are not covered in the training data. In the future, we plan to explore a method to automatically optimize the natural language model in the process of using the system. The system may learn from user inputs to improve its performance and the coverage of language patterns.

The current implementation binds table-related information before the intent and entity extraction. However, it may happen that data binding mistakenly bind tokens that are not related to tables. This method trades off the size of training dataset and improves the accuracy of the model for intent and entity extraction. In the future, we plan to collect a larger dataset and train a more robust end-to-end model. 

==> sections/VIS_evaluation.tex <==

\textbf{Example Gallery}
To demonstrate the usability of our VisTalk system, we produce a variety of charts with example natural language utterances that specify the visualizations as shown in Figure \ref{fig:examples}. %For each graph, the created chart is below, and the above is the natural language utterances of user to generate it. 
Figure \ref{fig:examples} shows five examples from our gallery. 
These visualizations cover cover a wide range of operations that users may take in real world visualization authoring scenarios. 
The VisTalk system can enable the creation of basic charts with simple operations such as data operations, encoding operations, and annotate operations with natural language utterances. For example, Figure \ref{fig:examples}a shows a generated line chart with trend lines and reference band added. Users can accurately specify the time ranges of trendlines and reference bands. 
Figure \ref{fig:examples}b demonstrates a column chart in descending order with an average line. It further highlights the “Ford” column with red color.
The column is set to red color by referring to the data label ``Ford''.
VisTalk system also supports more complex operations, such as layout operations, view manipulation, and styling operations. For example, in Figure \ref{fig:examples}c, the user set the woman and man icons as marks to create a pictograph and name it ``my mark''. The height of the color shows the value of \textit{Attacks}. Further, the user 
replace the original rectangle mark with this specified mark, and created a new visualization chart with position showing the total number, and fill color showing women and men percentages.
Figure \ref{fig:examples}d shows an example of leveraging icons to replace marks and changing the color to cyan. 
%Since our system can support various operations, users can easily create charts with abundant information and data analysis effect using natural language\todo{???}. For example, 
Figure \ref{fig:examples}e shows a case of multiple views generated by the combination of a series simple operations. The user first create a Ford Sales and highlight top 2 models. Then a reference band from 0 to 200K was added as a rectangle. The chart was sorted. After that, the user repeat the operations by ``Brand'' field and apply the operations to all the brands in Brand column. The user further remove charts of BMW, Ford, Toyota, and Honda and place the charts into two columns.  




% To demonstrate the usability of our VisTalk system, we produced a variety of charts, with example natural language utterances that specify the visualizations. Different natural language descriptions are also supported. 




























\section{User Study: Visualization Reproduction}
To understand how users can produce expressive visualizations through VisTalk, we conduct a qualitative user study. Through the study we validate whether users are able to smoothly use natural language to create charts. Further, we aim to understand the advantages and disadvantages of natural language-based visualization authoring systems.

We recruited 12 participants (3 female and 9 males, age ranging from 22 to 45) who had normal or corrected-to-normal vision. The participants include undergraduate and graduate students, data analysts, researchers, and software engineers. They are general users who need to create visualizations to present data in daily work. All of the participants had used Excel to create charts before, while five of them had used Tableau or Power BI to create charts. %Two had experience in using design tools like Adobe Illustrator. 
Two of them had experience employing natural language functions to do data exploration with general data visualization tools like Tableau and Power BI. 
None of them had used advanced expressive visualization building tools like Charticulator \cite{Ren_2019_8440827}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, etc. All of them had used natural language agents like Siri, Alexa to complete simple tasks. 


\subsection{Study Procedure}
We prepared five visualization reproduction tasks, including one basic charts, two charts with annotations, one pictograph, and one chart with multiple views. The tasks are ordered by complexity. %Two of the visualizations are simple and standard chart where participants need to encode data correctly. 
%x of the target visualizations further include chart designs with formatting. Participants need to change color, gap, border, font or the charts. x of the visualizations have more complex design with mark customization (similar to InfoNice), so participants need to further understand how to add embellishments, and replace marks with built-in icons.
First, we asked participants to fill out a pre-experiment questionnaire to collect their background information. Then, the participants received a 10-minute tutorial. In the tutorial, every participant watched a video that walks through two examples of using natural language to design a visualization. Then each of them is encouraged to have a quick try using the tools with one sample dataset to understand the features of the system.
After that, we showed the five target charts and described the underlying dataset. When the participants are ready, they pressed a ``start button'' to load the dataset and begin the creation of the visualizations. When they finish each task, they pressed an ``end'' button. Participants can ask the experimenter for help and clarification during the experiment. %\todo{We prepare a ``guide sheet'' to show them in case users cannot remember the operations and ask for help. To understand users' natural behavior of learning and using natural language systems, we do not provide the guidance by default.}
We observed the participants' interaction process and recorded the log of participants operation process. After finishing the tasks, participants filled out a questionnaire about the experience. We conducted a semi-structured interview to further understand their overall impressions, difficulties they encountered, and other feedback and thoughts. 
The study is carried out through web conferencing systems with participants sharing their screens with the experimenter.
The participants join the study using a web browser on their own machines. Each session lasted for about one hour.   

%\cp{To normalize expertise effects, we gave users one minute to do whatever they wished to accomplish for each task. After one minute, everyone received a “guide sheet” that showed them the operations for completing the task. For example, the guide sheet for a task could include the operations “brightness”, “sharpen”, and “vibrance.” Debrief. We debriefed the participants after they completed their tasks. We asked them for their overall impressions, the differences they encountered between the two types of interactions, and their overall feedback. In addition, we also asked the participants to complete a short questionnaire.}


\subsection{Results}

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=1\linewidth,height=130px]{pictures/sample.pdf}
%     \caption{completion time}
%     \label{fig:time}
%     %\vspace{-10px}
% \end{figure}



\textbf{Quantitative Analysis} 
Overall, the participants are positive about the system. Users highly rated the experience of using VisTalk (M = 4.36, SD = 0.69). Figure 7 lists the feedback of VisTalk. Twelve and eleven users agree VisTalk is easy to learn and easy to use. Eleven users think VisTalk has improved their productivity. Twelve users felt satisfied. The feedback also reveals space of improvement. Our participants rated it relatively low in terms of the powerfulness of the system and the effectiveness of completing their jobs. It maybe helpful to design more functions and interactions for VisTalk for future work.

To understand the complexity of utterances, we use mean length of utterances (MLU) \cite{oviatt1997mulitmodal}.
The number of words used ranged from 1 to 11.
The average MLU across 12 users is 3.61 words per utterance (SD=1.26).
In average, the participants used 2.4 utterances to complete a visualization creation task (SD=0.72)
The average time of creating one chart was 139s.


%Number and complexity of utterances varied a lot from user to user. Some participants tend to use single intent statements. (this may caused by their experience of using other natural language tools), some other participants tend to use long and complex statements. (Average word count, max and min) (number of intents each sentence) We observed that all our participants successfully completed tasks purely with text input box alone, whether or not the examples are available to them. 
%Some other participants rely more on the dynamic widgets to achieve their goals.



%\cp{We approximate the complexity of utterances using the mean length of utterances (MLU) measure [20] (Figure 5b). From a total of 386 utterances, the number of words used ranged from 1 to 6, and the average MLU across 14 users was 1.89 words per utterance (SD=1.10). Novices averaged 1.83 words per utterance (SD=1.14), compared to 1.94 words per utterance among experts (SD=1.07). }


%\cp{Speech engine implementation obtained high accuracy.We transcribed all user utterances and compared them with PIXELTONE’s speech-to-text output (Figure 5a). The accuracy was calculated by comparing the Levenshtein distance (expressed as a percentage) between PIXELTONE’s speechto-text output and the actual transcribed utterance. From a total of 386 utterances across 14 users, our two-tiered speech recognition implementation obtained an average accuracy of 84\% (SD=29\%).  For native English speakers, we obtained an accuracy of 90\% (SD=20\%) compared to 70\% for non-native speakers (SD=38\%) This finding was statistically significant (p<0.001) using a t-test. In addition, PIXELTONE was 84\% accurate for more experienced users (SD=27\%) compared to 82\% for novices (SD=31\%).}

\begin{figure}[!tbp]
    %\vspace{px}
    \centering
    \includegraphics[width=1\linewidth]{pictures/ratings.pdf}
    \caption{User ratings of VisTalk system with a 5-point Likert scale.}
    \label{fig:time}
    \vspace{-5px}
\end{figure}


\textbf{Qualitative Results}
Our participants were overall have a very positive experience authoring with natural language. All of them said they would recommend VisTalk to their friends or use it in the future if they need to explore data and design visual charts. Compared with WIMP interfaces for chart creations, the participants prefer the natural language-based one because it is easy to learn.
For simple tasks, users usually only type in some keywords to see how the systems can parse their intentions. For example, after one user (P2) tried ``trend'' and then ``add trend'', the system automatically added a trend line to the line chart. The participant said, ``It worked well. Natural language makes the thing easy.''
Participants also mentioned that it is easy to accomplish complex tasks with natural language, because it allows them to combine many operations within a simple sentence in the way that meets their needs. One user (P3) commented, ``The experience is very good! In the past I need to search the menus and click the right buttons to perform the tasks. Sometimes it costs a long time to find the right menu item. Now I don't need to think of where they are.'' 

%high efficiency
The majority of participants (10/12) mentioned that the natural language interface saves their time and efforts. The majority of participants (8/12) said they will use natural language as their first choice if their familiar systems support similar functions. P9 said, ``To design a simple chart, using one simple sentence is enough. It is completely different from using mouse to select menus, select the data field from the dataset, specify chart types, and do further adjustments.'' Impressed by the parsing capability of VisTalk, P1 mentioned ``It is surprising that the system could perform correctly even when the sentence was very short and I misspelled some words and had grammatical errors.''

%easy to learn 
The participants (12/12) find the system interactions easy to learn even for those without much experience in visualization. One participants stated, ``I can quickly understand the effects of the commands.'' One of the participants who was not familiar with visualization creation tools said, ``Now I don't have motivations to learn to use traditional visualization tools. I will come to VisTalk if I need to create charts. It seems much easier to learn.'' P3 also mentioned, ``It is friendly to non-expert like me. I don't find difficulties of learning to use this tool. It gives me prompt feedback while I am typing and I feel I can complete the tasks easily. The overall experience is quite smooth.'' 

%default recommendations can help 
Although the chart recommendation functions are took simple strategies, many of our participants (7/12) mentioned the system recommendation is helpful. One participant said, ``The default charts were well-designed and I don't think I need to do further modifications.'' Three  participants mentioned they enjoyed using short phrases to interact with systems' default recommendations. P9 said, ``I am using these keywords to explore this system, similar to the experience of using search engines. I enjoy the way this system gives me surprises.''


%discovery - cold start
Participants also found difficulties when using natural language interfaces. Some participants felt they couldn't express their requirements especially at the beginning of the tasks. ``sometimes I forgot the words and felt hard to describe my requirements.'' One user applied to open and read the examples in the tutorial again at the start of the tasks. Another user opened search engine to look for a correct word. 
Although all of them got used to the natural language experience after a while. We find that cold start can be a problem for users that are not familiar with the system. This might because users are dim about how much the system could tolerate their vague or inaccurate expressions. To solve this problem, we believe more sufficient guidance and feedback can address this issue.

==> sections/VIS_introduction.tex <==
\firstsection{Introduction}
\maketitle

Natural language (NL) interfaces are becoming mainstream for modern applications thanks to their usability and learnability.
%seek better usability and learnability by supporting natural language 
%and have attracted visualization researchers' attention. 
Compared with traditional interfaces with complex menu items and mouse interactions, natural language-based systems require less prior knowledge on user interfaces, and users are not restricted to the locations of menus and buttons~\cite{hoque2017applying, setlur2016eviza}. %Therefore, fewer efforts are taken for users to interpret their intentions into the system's allowed functions. 
Recently, active research has been devoted to natural language interfaces for visual analytics systems \cite{dhamdhere2017analyza, gao2015datatone, setlur2016eviza, yu2019flowsense, srinivasan2017natural}. 
However, most of them only focus on data analysis and exploration tasks. Though these systems present data query results with visualizations, they generally do not support expressive chart customization.% via natural language. 

On the other hand, modern visualization authoring systems have emerged to enable creation of expressive visualizations. Recent authoring systems \cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support a much richer set of visualization authoring capabilities for flexible data binding and enable configurations of axes, legends,  marks, layouts, and annotations.
%than traditional visualization tools. 
Nevertheless, they involve complicated GUIs and incur a steep learning curve, especially for novice users. While natural language interfaces are promising in lowering the barrier of using advanced visualization authoring tools, unfortunately none of these systems currently support natural language interfaces.
 

%more flexible data binding and configurations for marks, layouts, annotations, and so on. Users can manipulate visualizations and graphical elements by pointing to the objects, finding configuration menus, and applying predefined functions.

%Contrary to the visualization analytics systems for data analysis, recent authoring systems \cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support more flexible data binding and configurations for marks, layouts, annotations, and so on. Users can manipulate visualizations and graphical elements by pointing to the objects, finding configuration menus, and applying predefined functions. %Theses systems support flexible and advanced authoring requests by direct manipulation of graphical elements and user menus. Users can point to the objects, find the configuration menus, and apply predefined functions carefully.  However,
%learning such complicated functions and adapt-ing to new user interfaces is often time-consuming and cumbersome,especially for novices.
%However, learning such complicated functions and adapting to new user interfaces is often time-consuming and cumbersome, especially for novices. Unfortunately, none of these systems support the usages of natural language.

% One major challenge of applying natural language interfaces for visualization authoring systems is the complexity of authoring operations. Various authoring systems may employ different visualization models and take notably different approaches to optimizing authoring interactions. A same authoring intent is defined as different internal functions across applications~\cite{satyanarayan2019critical}. \todo{very different cannot lead to the huge gap?}With a lack of a unified representation or grammar of visualization authoring intents, there is a huge gap to convert high-level natural language inputs from users to low-level authoring operations implemented by applications.

One major challenge of applying natural language interfaces for visualization authoring systems is the huge gap between high-level natural language inputs from users and low-level authoring operations implemented by applications. Advanced authoring systems may employ notably different visualization models to optimize authoring interactions. A same authoring intent may be defined as different internal functions across applications~\cite{satyanarayan2019critical}. Without a widely-adopted representation or grammar of visualization authoring intents, it is difficult to model users' natural language authoring utterances.

In this paper, we make a first attempt to model visualization authoring intents as \emph{authoring actions}.
The authoring actions serve as an abstraction layer to bridge NL utterances from users and authoring functions from applications. 
We further propose a natural language-based visualization authoring framework (Figure \ref{fig:pipeline}) with a natural language interpreter that can parse users' utterances into a sequence of such authoring actions. These authoring actions can then be adapted and executed by visualization authoring applications.
%explore the usage of natural language interfaces for visualization authoring systems. 
%We design a natural language-based authoring framework with a natural language interpreter that can parse users' utterances into a sequence of authoring actions. 
%, which are used as an abstract layer to bridge users' utterances and different authoring applications. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{pictures/workflow.pdf}
    \vspace{-10px}
    \caption{NL-based visualization authoring framework.}
    \label{fig:pipeline}
    \vspace{-10px}
\end{figure}


%To achieve this,
We start with a formative study to understand how users express their authoring intents. %There are three main findings from the study. First, users might use different workflows for different types of authoring scenarios. Second, natural language utterances may contain fuzzy reference and vague modifiers for parameters. Third, users tend to mix multiple intents in one sentence.
Based on the study, we summarize common authoring interactions and formulate them into \textit{authoring actions} in the forms of operation, objects, and parameters to model natural language intents into machine-executable commands. As a first step, we summarize the most common authoring operations and categorize them into six major groups.  
%On the top of the model, we design a deep learning-based natural language interpreter that parses users' utterances into a list of authoring actions, which can be further adapted and executed by authoring applications. 
%Authoring actions can be further adapted and executed by authoring applications' internal functions.
%This could result in different experiences of using natural language to describe authoring requirements, which may confuse users and decrease the learnability of natural language-based authoring systems.



We then implement a deep-learning based natural language interpreter. The NL interpreter takes an NL utterance as input and ouputs a sequence of authoring actions.   The  interpreter can  be  integrated  by different authoring tools to bring in natural language capabilities. For users especially novices, this approach reduces the barriers of learning authoring operations across authoring applications.

To assess our framework, we build a prototype system, VisTalk, which integrates the NL interpreter to support natural language-based visualization authoring. We demonstrate possible solutions of executing authoring actions and resolving the ambiguities in NL inputs.
We leverage VisTalk to conduct a user study to understand the effectiveness of natural language-based authoring systems. Our results confirm the effectiveness of natural language-based authoring for novice users. The study also reveals space of improvement for future research on natural language-based visualization authoring systems.

The contributions of this work are summarized as follows:
\begin{compactitem}
    \item We conduct a formative study on how users express their visualization authoring intents with natural language. We summarize and formulate authoring intents as \textit{authoring actions}, which are atomic units executable by applications. The introduction of authoring actions helps bridge the gap between natural languages and authoring applications.
    \item We propose an NL-based visualization authoring framework that is equipped with a deep learning-based natural language interpreter to parse NL utterances into authoring actions. The natural language interpreter consists of three stages: token recognition, intent and entity extraction, and authoring action synthesis.
    \item To illustrate the usage of the framework, we build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. Through VisTalk, we conduct a user study to further understand the experience of authoring with natural language. 
\end{compactitem} 






















% %with rule-based methods, which can be hard to generalize. 
% %Modern authoring tools however require the support of much more abundant and complex functions. The intents from human users can thus be more complex and diverse. This poses new challenges for the design of natural language tools. 



% % {\fontfamily{helveticaneue}\selectfont \{place, legend, position=[plot]right\}}\\
% % {\fontfamily{helvet}\selectfont \{place, legend, position=[plot]right\}}\\
% % {\fontfamily{lmss}\selectfont \{place, legend, position=[plot]right\}}

% %Visualization becomes increasingly popular for storytelling. There are growing interests of create visualization for communication and presentation. 
% A number of visualization authoring systems have emerged to enable the authoring of expressive visualizations. Contrary to the traditional visualization systems for data analysis, recent visualization authoring systems~\cite{Kim_2017_7536218, satyanarayan2014lyra, xia2018dataink, Wang:2018:IEC:3173574.3173909, Liu:2018:DIA:3173574.3173697, Ren_2019_8440827} support more flexible data binding and configurations for marks, layouts, annotations, and so on. 
% %\todo{how complex are the authoring operation?}
% %For example, data-driven guides \cite{Kim_2017_7536218}, DataInk \cite{xia2018dataink}, and InfoNice \cite{Wang:2018:IEC:3173574.3173909} support data binding with hand-drawn or vector shapes; %InfoNice \cite{Wang:2018:IEC:3173574.3173909} enables the creation of expressive visualizations through mark customization; 
% %Data illustrator \cite{Liu:2018:DIA:3173574.3173697} proposes repeat and partition features for creative design of visualizations.
% These systems support flexible and advanced authoring requests by direct manipulation of graphical elements and user menus. Users can point to the objects, find the configuration menus, and apply predefined functions carefully. However, learning such complicated functions and adapting to new user interfaces is often time-consuming and cumbersome, especially for novices. 
% %Mouse and touch interaction can also be inefficient for complex visualization design%, especially when the interfaces themselves are also complex
% %\cite{hoque2017applying}. 
% %There are many barriers to learning and adapting to new user interfaces especially for novices.
% %However, they have restricted the target users to "graphic designers". General users without visualization design knowledge are hard to understand visual encoding. InfoNice adopts a "mark customization" approach. However, ...Users still need to learn and get familiar with the interface to implement their design. 

% %As a promising interaction paradigm, natural language has the potential to offer advantages to address these issues. 
% In contrast, natural language interfaces have attracted researchers' attention thanks to its learnability and usability. Compared with traditional interfaces with complex --- but sometimes still insufficient --- menu and mouse interactions~\cite{hoque2017applying}, natural language-based systems require less prior knowledge \cite{setlur2016eviza}. Users are not restricted to the functions and locations of the buttons. Therefore, fewer efforts are taken for users to interpret their intentions into the system's allowed functions. Researchers have conducted research on natural language interfaces for visual analytics \cite{dhamdhere2017analyza, gao2015datatone, yu2019flowsense}. 
% However, most of them focus on visual data exploration and support basic natural language data query with rule-based methods, which can be hard to generalize. 
% Modern authoring tools however require the support of much more abundant and complex functions. The intents from human users can thus be more complex and diverse. This poses new challenges for the design of natural language tools. 
% %support the natural language module by NL-based data query. 

% To fill this gap, we explore the usage of natural language interfaces for visualization authoring systems. 
% Prior work of authoring tools have emerged to provide powerful authoring interactions for users. However, 
% these systems take notably different approaches to optimizing authoring interactions and ease the creation of expressive visualizations \cite{satyanarayan2019critical}. With different menus and interactions, authoring operations are defined as different internal functions across applications. This could result in different experiences of using natural language to describe authoring requirements, which may confuse users and decrease the learnability of natural language-based authoring systems.
% %difficulties of natural language interactions. For instance, the same keyword ``highlight'' may result in different interpretation for different platforms, 


% In response, we explore a natural language-based authoring framework
% with a unified authoring action grammar. To achieve this, we conduct a formative study to understand how users might express their authoring intents. %There are three main findings from the study. First, users might use different workflows for different types of authoring scenarios. Second, natural language utterances may contain fuzzy reference and vague modifiers for parameters. Third, users tend to mix multiple intents in one sentence. 
% Based on the study, we formulate common authoring features into authoring actions in the form of operation, object, and parameter to model natural language intents into machine-executable commands. As a first step, we list most common authoring operations and categorize them into six major groups.  
% %On the top of the model, we design a deep learning-based natural language interpreter that parses users' utterances into a list of authoring actions, which can be further adapted and executed by authoring applications. 
% Authoring actions can be further adapted and executed by authoring applications. 
% The authoring actions are used as an abstract layer to bridge users' utterances and different authoring applications.

% We implement an natural language interpreter with a deep learning-based model, that takes human utterances as input and ouputs a sequence of authoring actions. The interpreter can be integrated by different authoring systems to bring in natural language interfaces. Authoring systems can adapt and execute authoring actions with local authoring functions.  This
% helps enhance the capability of natural language understanding for authoring tools. For users especially novices, this approach reduces the barriers of learning and using visualization authoring systems for different users across applications. %The framework takes natural language as input and parses users' utterances through the natural language interpreter and outputs a list of \textit{authoring actions}. The output can be further executed by visualization authoring systems to respond to users' input and make changes to the visualizations.



% % To evaluate our framework, 
% % We then conducted user study to understand how users interact with the NL-based visualization authoring system.
% % Through our study, we show the benefits and pitfalls of using NL-based method for visualization authoring.

% To assess this framework, we build an example web authoring system, VisTalk, based on the natural language interpreter. We demonstrate the possible ways of executing authoring actions and resolve ambiguities in users' natural language inputs.
% Further, we leverage VisTalk to conduct a user study to understand the effectiveness of natural language-based authoring systems. Results reveal the benefits and weaknesses of VisTalk \todo{expand a bit}, inspiring future research directions for natural language-based authoring systems.
% %Users need to practice using the GUIs to accelerate their design process.
% %Drawbacks for the GUI for visualization authoring systems:
% %Users need to learn the different design process/logic behind the system one by one The GUI changes significantly across systems to support different user groups/needs. As a result, users need to switch between tools, learn different interface when they have different needs
% %In this paper, we explore a natural language framework for Visualization authoring. 
% The contributions of this work are summarized as follows:
% \begin{compactitem}
%     \item We conduct a formative study on how users express their visualization authoring intents with natural language. We summarize and formulate authoring intents as \textit{authoring actions}, which are atomic units executable by applications, to bridge the gap between natural languages and authoring applications.
%     \item We build a deep learning-based natural language interpreter to parse from their input utterances into authoring actions. The natural language interpreter consists of three stage, token recognition, intent and entity extraction, authoring action synthesis.
%     \item To illustrate the usage of the framework, we build a proof-of-concept authoring tool, VisTalk, based on the natural language interpreter. With this system, we conducted a user study to understand the effectiveness of NL-based authoring experience. 
% \end{compactitem} 




==> sections/VIS_nl-interpreter.tex <==
\section{NL-based Visualization Authoring Framework}
Based on the formative study, we consider the design of our natural language authoring framework against the following requirements: (1) The framework should be easy to extend to cover more authoring commands and the capability can be improved over time. (2) The framework should support flexible natural language input with vague descriptions. (3) The framework should be reusable for common authoring intents and support different authoring applications.

Based on these considerations, we introduce our natural language-based visualization authoring framework (Figure \ref{fig:pipeline}). The framework consists of two parts, a \textbf{natural language interpreter} and an \textbf{authoring application}. When a user inputs a sentence, the interpreter parses natural language inputs into \textbf{authoring actions} and sends them to the application. The authoring actions are a list of structured information that describes operations and can be executed by the application. The authoring application maintains an editing session of users' authoring context. Based on the context, authoring applications can call internal functions corresponding to the authoring actions.


%We design a natural language interpreter that parses human utterances to visualization authoring actions and can be applied across different authoring tools. 
We model users' visualization authoring intents as \textit{authoring actions} and formulate an authoring action as the combination of \textit{operation}, \textit{objects}, and \textit{parameters}. We summarize and categorize common authoring actions into six categories that cover visualization authoring functions in authoring tools. 
%Users' natural utterances can be parsed into authoring actions and passed to applications to execute. 
%First, we define a domain-specific language (DSL) of visualization authoring, covering common operations for visualization authoring from 6 aspects. 
We design a multi-stage  natural language interpreter from natural language utterances to authoring actions. First, we recognize data entities and outputs representations of utterance with data entities replaced with abstract arguments.
After that, we design a deep learning-based natural language processing module that extracts intents and entities from the utterances. 
Finally, the intents and entities are mapped to operations, objects, and parameters and organized into a sequence of authoring actions. %The natural language processing module takes users' utterances as input, and outputs the program in the form of our DSL. The code can be further parsed and implemented by specific applications or code libraries to complete the specific tasks under different design environments.


\subsection{Authoring Actions}\label{sec:model}
A wide variety of visualization creation systems \cite{Wongsuphasawat2016VoyagerEA, 6876042, Liu:2018:DIA:3173574.3173697}, code libraries \cite{bostock2011d3}, and declarative languages \cite{satyanarayan2016vega} have been developed to support visualization authoring. Existing authoring tools usually consider marks, data bindings, scales, axes, legends, and layout when specifying charts.
%Further, the visualization authoring systems are implemented with different models. Satyanarayan \etal \cite{satyanarayan2019critical} categorize them into three different types, namely, template editors, shelf construction, and visual builders. Common visualization authoring tools like Microsoft Excel, adopt template editors way. Shelf construction methods support more flexible mapping between encoding channels and data fields, and are adopted by Tableau, Polestar \cite{Pioch2006POLESTARCK}, and Voyager \cite{Wongsuphasawat2016VoyagerEA}. Visual builders like Charticulator \cite{Ren_2019_8440827} and iVisDesigner \cite{6876042} are more complicated and support fine control in specifying marks, glyphs, layouts, etc.
These tools have covered a wide range of functions to enable the composition of both standard charts and highly customized interactive visualizations. However, there was no common design model that can let us consistently design visualizations \cite{satyanarayan2019critical}, which have posed challenges to the design of extensible and flexible natural language understanding framework. 
We survey the functions of modern interactive authoring systems including Microsoft Excel, Tableau, Polestar and Voyager\cite{Wongsuphasawat2017Voyager2A}, Lyra \cite{satyanarayan2014lyra}, Data Illustrator \cite{Liu:2018:DIA:3173574.3173697}, Charticulator \cite{Ren_2019_8440827}, chartAccent \cite{ren2017chartaccent}, and declarative model Vega-lite \cite{satyanarayan2016vega} to recognize common authoring operations and functions. %We identified a set of common functions and categorize them into six categories. 

We define \textit{authoring actions} as the combination of authoring \textit{operations}, \textit{objects}, and \textit{parameters}. User utterances can be mapped to one or multiple authoring actions. The authoring process of visualization is the execution of a sequence of authoring actions. Formally, an authoring intention can be defined as a triple:
\begin{equation}\nonumber
    \texttt{authoring~action := \{operation, objects, parameters\}}
\end{equation}

The definition of the authoring action describes the actions the authors want to take to the visualizations.  The \textit{operation} identifies the type of the author's intent (e.g., ``change color'', ``add annotation''). The \textit{objects} are the targets that the operation applies to. This could be global (i.e., the canvas area), a set of components (e.g., the bars in a bar chart), or a specific component (e.g., the title text). Finally, the \textit{parameters} indicate the degree or configurations of the operations.


\begin{table*}[!t]
    \centering
    \includegraphics[width=1\linewidth]{pictures/new-taxonomy-cropped.pdf}
    \vspace{0px}
    \caption{An authoring action consists of three parts, operation, object, and parameter. The table shows example authoring operations and the  corresponding objects and parameters. Operation are categorized into six major groups. Objects are categorized into chart components (e.g., axes, legends, title), mark channels (e.g., shape, color, size, position), and annotations (e.g., reference lines, reference bands, trend lines). }
    \label{fig:taxonomy}
    \vspace{-1px}
\end{table*}

\subsubsection{Operations}
%Our framework models the action of users' authoring requests as a sequence of operations %. %The basic operations are primitive operations (e.g., data binding, change color, change font, etc.). More complex operations can be combined with multiple primitive operations and are used to complete typical design tasks. For example, ``turn the bar chart to a pictograph.'' \todo{how to} %All the operations require target objects (e.g., axes, marks) and parameters. 
%Based on existing visualization authoring systems and taxonomies \cite{satyanarayan2016vega, Ren_2019_8440827, Liu:2018:DIA:3173574.3173697, Wang:2018:IEC:3173574.3173909, ren2017chartaccent}, 
%The most primitive operations that appear in visualization authoring tools 
%and 
%We categorize authoring operation into six major groups.
%, namely, data operations, visual encoding operations, layout operations, styling operations, view manipulations, and annotate operations.\todo{no need to list the names of the categories since they will be listed below...} 
%Different o
Operations may apply to different objects, depending on the properties of the objects. 
Table 1 lists the operations and the corresponding target objects and possible parameters. 
Operations are not exclusive because human languages may express same meanings with different patterns. For example, binding a data field to x axis, has the same effect as encode the horizontal position of mark to the field. Note the operations are not exhaustive.  
%We list common authoring actions that are used in visualization authoring.
% \begin{compactitem}
%     \item \textbf{General operations}, like \textit{add}, \textit{remove}, \textit{copy}, are the operations that can be acted upon any object, including graphical elements (e.g., add an annotation) or data encoding (e.g., remove a filter).
%     \item \textbf{Data encoding} is the mapping between data and visual channels.
%     \item \textbf{Data transform} are the operations that are related to data query and calculation, such as \textit{select}, \textit{filter}, \textit{pivot}, and \textit{join}.
%     \item \textbf{Selectors} are the operations that are applied to the objects with visual properties, such as \textit{change color}, \textit{modify shape}. For example, users can change the color of the title; or change the color scheme for the marks in a chart. Users may even replace the marks with icons for expressive visualization design.
%     \item \textbf{Numerical operators} are the operations that are related to the numerical properties of objects. Change range, of something. For example, change the height and width.
%     \item \textbf{layout operators} are a special type of numerical operators that can be widely used for expressive visualization designs. Users may add labels, annotations, and configure the positions of them. They may \textit{move} up or left, \textit{change position} to a specific point, or even \textit{adjust z-order} for the graphical elements.
%     \item \textbf{Text operators} include the operations that are specifically related to text. For example, users may \textit{modify content} of titles, or \textit{change font} for the annotations.
% \end{compactitem}
% \begin{compactitem}
%     \item \textbf{Bind} is the mapping between data and visual channels; data transformation and data fields; data transformation and visual channels 
%     \item \textbf{Add/Remove/Modify} can be applied to graphical element on a visualization design. For example, ``add the legend'', ``modify the title''. They can also be applied to data encoding, such as ``add a filter''.
%     \item \textbf{Set value} is applicable to any object with numerical properties, such as size, height, opacity, etc. 
%     \item \textbf{Change category} is used for the visualization objects with only discrete value properties.
%     \item \textbf{Color} is a special, color related, color scheme 
%     \item \textbf{Font} font style
%     \item \textbf{Style}
%     \item \textbf{Place} (move, position)
% \end{compactitem}
%The operations are categorized by visual features of the target objects. 
%In a visualization design, different visual components may have different properties. These properties further specify the variables that characterize the target components. For example, encoding supports different encoding channels such as position(x, y), size, and color. Marks have properties including shape, color, etc. The shapes for marks are rectangles for bar charts, circles for bubble charts, symbols for scatter plots, etc. The properties for marks also depend on the implementation of the charts. For example, a more flexible authoring tool may support users to replace the basic geometric shapes with icons, or even images. Following the implementation of existing authoring systems, 

We summarize six main categories of operations:
\begin{compactitem}
    \item \textbf{Data operations} are the operations that retrieve and calculate data from datasets. Typical operations include aggregate, bin, set time unit, and sort. These operations are applied directly to data. 
    \item \textbf{Encoding operations} are the manipulations of data fields and data values, and aggregate functions to the values assigned to visualization attributes. Users may take operations to the axes or marks to specify encoding.%, while the effects might be the same. %For example, ``bind Country to x axis'' and ``bind Country to the horizontal position of marks'' have different objects (i.e., x axis and position), while they have the same effects. 
    \item \textbf{Layout operations} include the configurations related to position and offsets of chart components, such as title, annotation, legend. Users can place an object at a designated position, or move it along a direction.
    \item \textbf{Styling operations} includes graphical operations and textual operations. Graphical operations are performed to color, size, shape, icon, and stroke of graphical elements, including axis lines, marks, reference line, etc. Textual operations are acted to text-related properties such as font (size, color, style, weight), content. They can be applied to title, labels, annotations, etc.
    \item \textbf{View manipulation} refers to operations that create one visualization with multiple views. Chart views can be created into multiple or layered displays. %Multiple views can also be created by ``faceting'' the current view by one data column (e.g., facet the sales by country) or ``repeating'' one chart view to other data values (e.g., repeat the sales chart for US and Japan). 
    \item \textbf{Annotate operations} manipulate annotations (e.g., text, labels, embellishments) that enhance the charts. Annotations can be bound with data. For example, trend lines can show the trend between two time points.
    %can show aggregated values by the marks\todo{do we have the corresponding operation for adding labels?} . 
\end{compactitem}



%Based on these operations, more complex high-level operations can be combined. For example, "change the style" usually means the combination of graphic properties and textual properties. This may even apply to the color coding of the marks, further impacting data encoding properties. ``Sales by year'' usually means create a chart, bind x axis with Sales, and bind y axis with Year.

% \begin{compactitem}
%     \item \textbf{Change Chart} removes the current chart encoding and applys new encoding to change the chart into a new one.
%     %ll\item \textbf{Repeat and partition}  
%     \item \textbf{View composition} (facets) applies all the settings and further modifys the data encoding properties.
%     \item \textbf{Fill percentage} adds a background icon with the same foreground icon but different colors.
%     \item \textbf{Interaction} specifies different sets of properties based on users' interaction conditions. Users need to specify the condition and the effects of the interactions.
% \end{compactitem}




\subsubsection{Objects}
Objects are the components that the operations target. 
%For an authoring operation, users usually need to specify the targeting object they want to create, modify, or remove. 
In WIMP interfaces, users usually click on the menus or select the targeting objects on canvas. For a natural language environment, users need to specify the objects through NL utterances.
For a basic visual chart, the components include marks, axes, title, legend, gridlines, etc. More advanced objects include annotations such as trend line, reference line, reference band, text annotations, and embellishments.  

The objects in an authoring action can be under specified. For example, a user may say ``give me a chart'' after uploading a dataset. An intelligent authoring system should recommend a best encoding to users. 
We directly models users intention and use a special notation ``*'' to represent  the under specified objects. The implementation of authoring systems should further decide definite reference strategies.


%Clearly, a target component may support more than one target operations\todo{???}. %A mark may simultaneously support encoding operations and styling operations. 

% To describe an authoring operation, users usually need to specify the targeting object they want to create, modify, or remove. 
% In graphical user interface systems, users usually click on the menus, or select the targeting objects on visualization canvas. For natural language environment, users need to specify the objects through their utterances.

% \textbf{Objects} are the components that the operations targeted to. For example, for a basic visual chart, the components include marks, axes, title, legend, encoding, etc. Authoring tools for standard charts usually only support limited number of target properties. Supported components can further include annotations such as trend line, reference line, text annotations, etc., depending on the implementation of different authoring tools.  
% Clearly, a target component may support more than one target properties. An implementation of visualization mark may simultaneously support general properties, graphic properties, and data encoding properties. 
% For example, the rectangles in a bar chart can be configured to different color and widths. The rectangle mark can also be replaced with other shapes to reach expressive visualization designs. While different target properties are handled by corresponding operations. The parameters further configure how to change these objects. 

%Once users obtain a chart, they may further say ``turn it to red''. The systems may infer the intention of the users is ``turn the marks to red''. We 

\textbf{Object Selectors.}
As discussed in Section 3, users show special patterns when referring to objects with natural language. 
They may refer to objects through \textit{object properties}. 
%For example, users may ask the system to ``turn the red line blue'', which means ``turn the line in red color to blue color''. Therefore, w
We support an object selector for users to filter the objects. For example, the intention ``turn the red line blue''  does not directly specify the object because there is no component named ``red line''. %The ``red line'' can be selected as \texttt{[shape=line,~ color=red]}, 
The statement can be presented as \texttt{\{SetColor, [shape=line,~ color=red], color~name=blue\}}, meaning to select objects the properties, ``line'' and ``red''. 
%The similar pattern can also be applied if visualization components are clearly referred to, but users would like to select parts of them. For example, ``add black stroke to the blue bar'' for a colored bar chart can be translated to \texttt{setStroke, [shape=bar, color=blue], color=black])\}}, meaning users wants to change the style of the mark with blue color and the operation is \texttt{setStroke}. 
The properties that users describe should exist in the predefined library of property and parameters. Otherwise, the natural language interpreter may not be able to match them and leave quotation marks to the text phrases. %Further, the natural language interpreter may not be able to understand the attribute type and leave a star mark as placeholder. Applications may further parse the attributes based on the context of authoring.
For example, ``add black stroke to the abc bar'' can be translated to 
\texttt{\{setStroke, [shape=bar, *=`abc'], stroke=black)\}}.

\textbf{Object Naming.}
We support object naming to enable easy reference. For example, after applying a filter ``US'' and ``2020'' to the chart, users can simply name the chart as ``US2020''. This helps them easily refer to this chart. Object naming further enables nested design of visualizations. For example, users may put two visualizations together by opening up a new canvas and saying ``put US2019 and US2020 side by side.'' This also helps enable creative visualization design. Figure \ref{fig:examples}c shows an example where the user  use two icons to create a pictograph and reuse it in another chart to create novel visualization design.
%This also enables flexible graphical designs.
%For example, users may use two simple shapes to create an icon. After that, users can name it ``icon1'' and use it to customize charts. We support this by a special operation ``setChartName'' that can be applied to any object.


\subsubsection{Parameters}
Parameters are specific configurations of the operations. The parameters correspond to the operations and objects. It describes what extents the operations are performed, or how the operations are applied to the objects. Based on the object properties, we need to further define a library of parameters. By defining the forms of these parameters,  users' free-form natural language can be translated into machine-understandable commands. Table 1 shows example parameters corresponding to different chart objects. 
When users specify their requirements in natural language, the parameters can be clear and definite. For example, ``please set the chart 10px wide and 13px height.''
The parameters can be implemented as numerical values for chart width and height, enumerations for font style and encoding channels, boolean values for adding or removing components.



\textbf{Vague parameters}
Natural languages might be rough and vague. We define a set of vague parameters for different operation types. For example, for color values, we support e a list of color names (e.g., \texttt{color=red}, \texttt{color=navy~blue}). We also define a number of extent keywords, ranging from ``extremely'', ``very'', ``moderate'', ``a little'', to ``very little''. Users can therefore describe the adjustments of size as ``make it really large'', which will be mapped to ``very large'' and can be parsed as \texttt{\{setSize, *, size=very.large\}}.
Authoring tools can further interpret them into machine-understandable values based on design environments.



\textbf{Relational Parameters}
With a well-defined parameter set, we can further turn the vague description of the intention to concrete parameters. We support two types of relational parameter that can converse users utterances such as ``make it larger'', or ``set the color of the title darker than the bars''. For each relational parameter, users need to specify the objects it compared to, and the direction of change. For example, ``make the title darker'' is explained as make ``itself'' darker, where the object is the title; ``place the legend on the right of the plot area'' is explained as ``right'' to the ``plot''. Formally, the utterances are interpreted to \texttt{\{setColor, title, color=self[+]\}} and 
\texttt{\{place, legend, position=plot[right]\}}. \texttt{self[+]} means the value larger than it self while \texttt{plot[right]} means on the right of the plot. Applications should further determine the exact values of these parameters after receiving these vague parameters.






\subsubsection{Example Utterances}
Combining operations, objects, and parameters, authoring actions can represent various authoring utterances. An utterance may corresponds to multiple authoring actions. 
Here we show example utterances and the corresponding authoring actions to further illustrate the use of authoring actions. In Table \ref{tab:examples}, the utterances are represent with one to four authoring actions. These examples include object selectors (d, e),  vague parameters (b, c, d, e, f), and relational parameters (b, d).

\begin{table}[ht]
\centering
\includegraphics[width=1\columnwidth]{pictures/example-utterances-1-cropped.pdf}
\vspace{1px}
\caption{Example utterances (left) and corresponding authoring actions (right). One utterance may correspond to multiple authoring actions.}
\label{tab:examples}
\end{table}













\subsection{Natural Language Interpreter}
%We model the natural language processing module as the conversion from natural language to our predefined domain-specific language. To do this, we model conversion problem as a natural language understanding problem in natural language processing.
%We formulate this problem as a semantic parsing problem \todo{?} that takes human utterances as input, and outputs executable authoring actions. 
%As modeled in Section \ref{sec:model}, an input utterance may include multiple authoring action intents. 
Our natural language interpreter bridges human utterances and authoring applications in a general way. For an input utterance, NL interpreter aims to translate it to  a sequence of authoring actions that can be executed by visualization authoring applications. NL interpreter consists of three steps, namely, token recognition, authoring intent and entity extraction, and authoring action synthesis.  


%Conversation agents like Siri, Cortana, or natural langauge interfaces for visualization only support one standalone command. In other words, users have to make their requests like sending multiple standalone commands. These standalone commands are effective for simple goals. However, visualization authoring requests are usually complex. Users may naturally combine multiple commands in one simple sentence. For example, ``give me a blue bar chart for sales by year.'' includes the requests of ``draw a chart for sales by year'', ``make it a bar chart'', ``turn the bar to blue''.  Therefore, the NL interpreter needs to take the users' utterances and parses multiple intent expressions if needed. To tackle this challenge, we take a state-of-the-art deep learning-based model that supports multiple intent parsing for natural language conversion.


%\cp{Why does Siri fail? The root of the issue is that Siri (and similar agents) employ a simple model of conversation. While humans engage in complex conversations, interactions with today’s agents can be described by the following algorithm: (1) determine which command a user wants, (2) ask for any missing arguments, and (3) execute it. In other words, every conversation you have with an agent today is equivalent to executing a standalone command. These standalone commands are effective for simple goals such as setting a timer or finding directions, but they restrict agents to tasks that a system has been explicitly designed to handle.}



\subsubsection{Token Recognition}
Before the interpretation of user utterances, we recognize dataset-related entities in the utterance as the first step. These entities are table names, column names, and cell values in a table. The natural language interpreter is therefore aware of the data context. For example, for a dataset ``CarSales.csv'', we identify data column names like ``Sales'' and ``Brand'', and data values like ``Ford'' and ``Honda'' in users' natural language utterances. To do this, we enumerate all the n-grams and check against the table entities in the input query in descending order of length. Once a k-gram is recognized (k may be different from n), we remove all the remaining n-grams that has overlapping parts with it. %We assign these entities as \textit{exact match} or \textit{partial match} of dataset entities for typo tolerance. 
After that, we replace these recognized tokens with abstract arguments like $<column>$, $<value>$ as input for the next stage. 
Further, we also link entities like number and date as special entities through similar ways. We assign numbers and dates into four categories: $<integer>$, $<float>$, $<date>$, and $<year>$.
This way, the difficulties and uncertainties of understanding the authoring intents can be reduced \cite{yu2018typesql, guo2019towards, dong2019data}. 
The token recognition phase outputs representations of user utterance with data entities replaced with abstract arguments.
%Our approach can be regarded as an implementation of entity linking on the concrete task, because general entity linking (Shen et al., 2015; Kolitsas et al., 2018) approaches fail to handle particular challenges in our scenario. On the one hand, there are lots of cases cannot be handled by the deterministic entity linking method which only relies on measuring the similarity; on the other hand, there is no labeled data for the learning-based entity linking method.


\subsubsection{Authoring Intent and Entity Extraction} 
The purpose of this stage is to identify the intents and a list of entities which serve as parameters corresponding to the intents, which can be further organized into authoring actions through a synthesis stage. A NL utterance for visualization authoring may involve multiple intents.
For instance, the sentence in Figure \ref{model_example}g expresses four visualization authoring intents. 

Similar to NLP tasks such as semantic role labeling, sequence labeling, and named entity recognition, extracting objects and parameters in an utterance is actually a BIO tagging problem~\cite{ramshaw1999text}. In our task, we define the entities as the utterance parts which act as objects and parameters in authoring actions. We create a series of labels following the BIO format to indicate the role of each utterance parts (Figure \ref{model_example}).

\begin{figure}[t]
\vspace{0px}
\centering
\includegraphics[width=\linewidth]{pictures/labels.pdf}

\vspace{-1px}\caption{Intent tags and word labels of an example NL utterance. We regard color, chart type, y field (the data field bind to y axis), and x field (the data field bind to x axis) as entities in our model. Following the BIO (beginning, inside, outside) format\cite{ramshaw1999text}, we can map the words in the sentence into a sequence of labels, where B-, I-, and O represent begin, inside, and outside, respectively.}
\label{model_example}
\end{figure}


%, such as B-color.Color, B-chart.ChartType and so on. For intent, we define 31 different intents which cover the intentions of user utterances. 


%Users may naturally combine multiple commands in one simple sentence. For example, ``give me a blue bar chart for sales by year.'' includes the requests of ``draw a chart for sales by year'', ``make it a bar chart'', ``turn the bar to blue''.  Therefore, the NL interpreter needs to take the users' utterances and parses multiple intent expressions if needed. To tackle this challenge, we take a state-of-the-art deep learning-based model that supports multiple intent parsing for natural language conversion.


%To extract authoring actions from the utterance, we first recognize the intent and entities in the utterance. 

Instead of using rule-based methods, we train a neural network-based model to recognize intents and entities from input utterances. Specifically, on the basis of the work of Liu \etal \cite{liu2016attention}, we design a joint model for intent detection and entity recognition based on encoder-decoder framework, attention mechanism \cite{vaswani2017attention}, and CRF algorithm\cite{lafferty2001conditional}. After passing through the token recognition stage, the input utterances are fed into our neural model, and we can obtain the predicted intent tags and entity labels of each words, as shown in Figure \ref{model_example}.



%The model takes user utterance as the input and recognizes its intent and entities. For example, in Figure \ref{model_example}, after passing through the token recognition module, the given sentence is fed into the neural model. We can obtain the predicted intent tag, \textit{SetChartType}, \textit{SetColor}, \textit{BindX}, \textit{BindY}, and entity labels of each words, O, O, B-Color, B-ChartType, I-ChartType , O, B-YField, O, B-XField.


%We implement a neural network-based model to recognize the intent and entities of the sentence. Compared with traditional rule-based models with syntax analysis and semantic analysis, neural network-based model is simpler to maintain \cite{chen-etal-2016-sentence, pasupat2015compositional}. It is also more scalable to new data because there is no requirement to make changes to existing rules or set more extra rules.


%Based on the modeling of authoring actions, we treat all the parameters and objects as entities in a NL utterance. Together with intents (operations), we organize entities (objects and parameters) into authoring actions.

\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{pictures/model_arch2.pdf}
\caption{The architecture of our model for intent and entity extraction.}
\label{model_arch}
\end{figure}

\textbf{Deep Learning Model.}
%when a user enters a textual query $X’ = (x’_1, ..., x’_n)$, such as ``use cars with x sales with y axis'', the sentence will firstly pass through the token recognition module. We then feed the processed sentence X = ($x_1$, ..., $x_n$), ``bind $<column>$ with x $<column>$ with y axis'', into the deep learning model%, 
As shown in Figure \ref{model_arch}, our deep learning model is based on encoder-decoder framework. Specifically, we employ Bi-LSTM\cite{hochreiter1997long} as the encoder and LSTM cell as the decoder\cite{liu2016attention}. In the encoder part, the input words are mapped into an embedding space and represented as vectors, which are used in decoder to generate the target output. At a time step $t$, we use the hidden state $H_t$ to represent the input word $x_t$. $H_t$ is obtained by concatenating $h_t$ and $h_t’$, the hidden states of forward and backward LSTM networks. The last state of the forward and backward LSTM network carries information of the entire sentence, so we concatenate $h_n$ and $h_n’$ as the intent vector of the whole sequence. The intent vector and word representations will then be sent into the decoder. For intent recognition, due to the fact that a sentence may contain multiple intents, we predict the probability of all intents. If the probability of an intent is greater than 0.5, we consider it as one intent of the given utterance. For entity extraction, the attention mechanism is incorporated for better representation of each input word before determining the entity labels\cite{liu2016attention,vaswani2017attention}. To address the problem of inaccurate entity sequence prediction, we further apply Conditional Random Field (CRF) algorithm in the prediction process\cite{xu2013convolutional,zhang2016joint,huang2015bidirectional}, so that during tagging a word, we can adopt the previously labeled information and Viterbi algorithm to get the optimal entity sequence prediction. Finally, we extract the intention category and labels for all segments $Y = (y_1, ..., y_n)$. The parameters of the LSTM and CRF are jointly trained.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{pictures/interface.PNG}
    \caption{VisTalk interface (a). Users can type in their natural language utterances in the text box (b) to customize their visualization design (c). Users can author different charts at the same time (d). The table view shows the underlying dataset. 
    Users can click the words as interactive widgets to choose icons, change colors, or adjust number (f). The auto-completion panel pops out during the input process (g). }
    \label{fig:interface}
    \vspace{-5px}
\end{figure*}

\textbf{VisAuthoring Dataset} 
%position as a first step
We collect a VisAuthoring dataset to train our model. It contains about 78K visualization authoring utterances, covering data operations, encoding operations, annotate operations, styling operations and view manipulations. As a first step, this dataset is composed of two main sources. First, we obtain the dataset by collecting more than 13K human-labeled natural language utterances. Second, we create more than 1100 authoring statement templates to generate a synthetic part for the dataset. The dataset consists of natural language sentences and their corresponding intent tag, entity labels of each word in the sentences. %In total, there are \todo{31} kinds of intents, covering all the operation types. Additionally, there are \todo{32} kinds of entity tags, such as {B-mark.Mark, I-sort.Sort, B-unit.NumberUnit, B-text.String} and so on.

\textbf{Results}
We evaluate our model performance on the VisAuthoring dataset. Furthermore, to verify the generality of our model, we also conduct experiments on the ATIS dataset\cite{hemphill1990atis}. ATIS is the public benchmark dataset in natural language understanding, which has many characteristics of spoken language and is completely collected in the actual office environment. The results are shown in Table \ref{model_result}. We assess from three aspects: intent accuracy, slot accuracy, and slot F1 score. The results show that our model works quite well. The performance results on ATIS are very close to the state-of-the-art results. Moreover, our model is more adaptive to visualization authoring tasks.



\begin{table}[ht]
\centering
\begin{tabular}{p{2.5cm}<{\centering}|p{1.7cm}<{\centering}|p{1.7cm}<{\centering}}

\toprule  %添加表格头部粗线
Datasets & VisAuthoring & ATIS   \\
\hline
Intent Accuracy & 99.94 & 97.08  \\
Slot Accuracy  & 99.74 & 97.59 \\
Slot F1 Score & 99.74 & 97.60  \\

\bottomrule %添加表格底部粗线
\end{tabular}
\vspace{2px}
\caption{The performance of our model on VisAuthoring dataset and ATIS dataset. Intent accuracy represents the model performance in intent recognition, while slot accuracy and slot F1 score denote model performance in word role label detection.}
\label{model_result}
\end{table} 


\subsubsection{Authoring Action Synthesis}
Given intents and entities, we then perform program synthesis to organize them into a sequence of authoring actions. As is defined in section 4.1, the authoring action consists of three parts, operation, objects, and parameters. For extracted intents and entities, the intents are mapped to operations, while the entities are mapped to objects and parameters. 

We synthesize authoring actions by traversing the intent list. The intent obtained from the deep learning model can be directly mapped to the operation types. Based on intent type, we can determine the corresponding objects and parameters it supports. The matching process works as follows:
For each intent of an utterance, we traverse the extracted entity list one by one. We map the intent to an operation. If the entity belongs to the operation, it can be matched to the operation and directly filled into the object or parameter. Once an entity is successfully matched to an operation, we delete it from the entity list, which means each entity in the list can only belong to one operation. If there is no parameter or object for an operation, we fill it with a ``*'' mark, meaning the default state. After this process, we will obtain a list of authoring actions.

From remaining entities, there are two possible situations. One is that an intent is reused in the utterance. For example, in the case “change color of china and US bar to green and blue”, the entities “china” and “green” are left and haven’t been matched to any intent because the intent “change color” is reused. In this circumstance, we assume users specify the objects and parameters in order, so we fill the residual entities into the closest intent based on entity name and type. The other situation is that the residual entity exists as the selector of the object. For these cases, we check the list of objects and their supported properties, and fill the entity type and entity value into the selector of the object with proximity principle. If such matching object cannot be found, for example, users may only say ``red'' or ``bar'' as an utterance, then these entities are packaged one by one as authoring actions without operations.

Finally, after getting a list of authoring actions, we further rank them based on the category they belong to. Considering the operation types in the authoring actions, we sort the authoring actions from global operations, such as data operation, data encoding, view manipulation to local operations, such as changing the color, changing the title content.



% Using the deep learning model to extract intents and entities, we perform program synthesis to organize them into a sequence of authoring actions. The intent types can directly mapped to the operation types. 
% For different intents, we maintain the applicable parameter names to match proper entities in the sentence. For example, an intent  
% Start from the list of intents,

% The deep learning model outputs the classification of the intents in user utterances, and the object, parameter labels of the words in the input statements. Further, we organize the labels into intents and output the intents as the a list machine executable expressions. When there are multiple intents in a sentence, we need to match operation, objects, and parameters. As is analyzed in section 3, objects usually only support particular parameter types and operation types. Therefore, we leverage object properties to correspond parameters and operations. 
% It also happens that the objects cannot differentiate the operations and parameters. For example, users may say ``Turn the title to red and axis title to blue''. In this case, title and axis title are both objects with color properties. For these cases, we assume users specify the parameters in order. So we apply red to the chart title and apply blue to the axis title.  











% DL model的输出是一个intent list + entity list
% intent type是可以直接对应到operation的。
% 所以根据intent，也就是每个operation的类型，能确定它所支持的object和parameter列表；
% 一个intent 对应一个authoring action。


% 遍历intent list
% 在entity list中根据预测结果一个一个match，如果是这个operation的，就能匹配到这个operation上，可以直接填到object或者parameter。如果一直没找到，这个authoring action的 parameter和object缺省。如果找到了，就从authoring object/parameter list去除掉这个entity。

% 最后会得到一个list of authoring action （每个intent对应一个authoring action）
% 但有可能有一些entity多出来了。对于entity多出来的情况有两种可能，一种可能是某一个intent/operation被重复使用了 把change color to china and US bar to green and blue - 多出来了china和green/change color被重用了。这个时候我们就根据entity name和entity type来把entity填到最近的intent中
%另一种情况是entity作为object的selector存在，这个时候检查object的list和他们支持的properties，就近把entity type和entity value填到这个object的selector
%如果找不到这样匹配的object，比如用户整句话就输了一个``red''或者就输了一个``bar'', 那么根据它们的entity type和entity value， 打包作为没有intent的authoring action


 

% 最后我们会给出一个authoring action list。 我们进一步根据它们属于的category给他们排序。

%排序的方法根据authoring action中的operation类型：从大到小排序，先做global的- data operation, data encoding, view manipulation)；再做小的，比如改颜色，改标题内容









%dependency
%global knowledge - chart type, color, position, 
%(local knowledge - literal string - icon name)





%find a line with red color...
%give me a red column chart of sales by year
%intention - parameter 
%set color, map x, map y, chart type (no enough labeled data)
%object (condition = ?) parameters ...
%parameter can be * (under specified)
%naming of the object groups

==> sections/VIS_related-work.tex <==

\section{Related Work}
\subsection{Visualization Authoring Tools}
A variety of visual authoring approaches have been proposed to facilitate visualization creation. For example, Polaris \cite{Stolte2000PolarisAS}, Tableau \cite{tableau}, and Many Eyes \cite{ibm} help users to conduct data encoding with visual channels in a visualization. These tools enable users to create visualizations in a short time, but they are less flexible. The resulting visualizations are usually standard visual charts. More advanced techniques, such as Lyra \cite{satyanarayan2014lyra} and iVisDesigner \cite{6876042}, have been proposed to enable more expressive visualization designs. With these systems, Users can easily specify properties of graphical marks and bind them with data. However, these systems only support the modifications of properties by adjusting a set of style parameters. Later, data illustrator\cite{Liu:2018:DIA:3173574.3173697} uses repetition and partition operators for multiplying marks and generating data-driven expressive visualizations. Charticulator\cite{Ren_2019_8440827} also adopts a bottom-up approach to bind data fields to vector graphics and build visualization with an emphasis on visualization layouts.
Recently, Data-Driven Guides \cite{Kim_2017_7536218} allows users to draw and design graphical shapes to achieve creative designs. Similarly, DataInk\cite{xia2018dataink} and InfoNice \cite{Wang:2018:IEC:3173574.3173909} also bind graphical elements with data fields to facilitate the generation of creative visualizations.

Researchers have explored the design of visualization authoring systems and supported creation from different perspectives. To support visualization creation, the systems have different internal logics.
%, which can be basically divided into three categories, namely template editors, shelf construction, and visual builders \cite{satyanarayan2019critical}.
With these systems, we summarize and categorize most common functions used. We further formulate the functions as authoring actions, which is an abstract layer that bridges human intents and authoring functions. The authoring actions can be explained and executed by the functions supported by different tools.

% Visualization systems have been proposed to ease the creation of visualizations

% - template editors
% - shelf construction
% - visual builders

\subsection{Natural Language Interfaces for Visualization}
Natural language interfaces have been adopted extensively to improve the usability of visualization systems. 
Commercial tools like IBM Watson Analytics \cite{ibm}, Microsoft Power BI \cite{pbi}, ThoughtSpot \cite{ThoughtSpot}, and Google Spreadsheet \cite{dhamdhere2017analyza} automatically translate the natural language questions to data queries and present query results with visualizations. However, these systems limit natural language interactions to data queries and corresponding standard charts.

%Instead of simply showing data query results with numerical answers, visualizations are more readable and understandable. 
Extensive research has been devoted to a better experience of using natural language for visual analytics~\cite{srinivasan2017natural}. 
To complete the analytical tasks, they treat user input utterances as natural language queries, and translate them to logic query languages \cite{androutsopoulos1995natural}, such as XML \cite{li2007nalix}, and SQL \cite{zhong2017seq2sql}. Researchers further study the interactive visual analytic systems that support natural language queries.
Wen \etal \cite{wen2005optimization} design a system to update the visualizations based on user queries dynamically. 
Articulate \cite{aurisano2016articulate2} generates a graph to select proper visualizations to answer users' natural language questions and complete analytic tasks.
Orko \cite{srinivasan2017orko} is a natural language system for network data exploration.
FlowSense \cite{yu2019flowsense} applies natural language techniques to dataflow visualization systems.



%to address ambiguity problems in natural language
Researchers also try to address ambiguity problems through different means. On the one hand, researchers try to address ambiguity problems through the design of interactive systems to invite users to clarify their requests. For example, DataTone \cite{gao2015datatone} introduces interactive widgets to address ambiguity problems.
Eviza \cite{setlur2016eviza} further enhances the interactions by providing graphical answers that can be directly manipulated. 
Iris~\cite{fast2018iris} is a conversational interface that enables users to combine commands through many rounds of question-answering.
%pragmatics principles
On the other hand, design principles are also summarized to improve the understanding of users' utterances.
To enhance natural language interactions, Hoque \etal \cite{hoque2017applying} apply pragmatics principles and propose a theoretical framework for interaction with visual analytics.
Hearst \etal \cite{hearst2019toward} conduct an empirical study to explore default visualizations for vague expressions in natural language queries. Similarly, Setlur \etal \cite{setlur2019inferencing} explore the way of inferring underspecified natural language queries and propose a systematic approach to resolve partial utterances.

%we are different from natural language query 
Most of existing work focuses on data analysis and exploration tasks. In comparison, our natural language framework is designed for visualization authoring tasks, which includes not only data querying and data operations, but more importantly, the specification and customization of visual encoding and visualization components.
%to let users give commands on the "editing operations" to the visualization and do the customization for their visualization design.


\subsection{Natural Language Understanding}
%In the visual human-computer interaction, understanding human queries is really important. 
Natural language understanding is the core component of a natural language-based system. 
Usually, the understanding of natural language inputs takes two steps: first identifying users' intents in the utterances as functions; then extracting useful parts as parameters for the targeting functions.
%To automatically understanding the input sentence and taking operations in the application accordingly, we need to firstly recognize the user’s entire intent. With obtained intent, we should further extract the useful parts in the sentence as references and parameters of the operation functions. 
Previously, visual analytics systems like \cite{yu2019flowsense, dhamdhere2017analyza, gao2015datatone} leverage rule-based methods to conduct complex syntax analysis and semantic analysis to parse input utterances. For example, FlowSense\cite{yu2019flowsense} applies POS tagging, NER, and semantic parsing techniques, and leverages a pre-defined grammar to capture NL input patterns. %, which achieves explicit effect on the improvement of natural language interface.
For visualization authoring tasks, the functions and parameters are more rich and diverse. Accordingly, input sentences are also complex and may conform to a large number of different syntactic rules, making it difficult to maintain a set of patterns and rules.
%Therefore, to establish rules and analyze the syntax structure of the sentence is either complicated or low scalable. 
%Because the accuracy of these systems largely depends on the formulation of rules, the difficulty of maintaining a set of NL patterns and rules also substantially increased.
%If the input sentence is in a different form, we may have to add new rules to explain it. In addition, when the input is incomplete and ambiguous, it becomes harder to identify a set of NL patterns cover the input by rules. 

Recently, deep learning-based models have been employed in natural language understanding tasks\cite{xu2013convolutional,guo2014joint,zhang2016joint,liu2016attention}. Compared with rule-based methods, deep learning-based models show better performance in terms of simplicity, scalability, and accuracy. Taking NL sentences as input and extracting intents and word labels through neural network, the systems can get rid of complicated rules. Generally, most of the models consist of two parts, intention recognition and slot filling, to detect user intents and word labels, respectively. %, i.e., operation parameters. %Compared with the methods that feed human query as input and directly generate codes, dividing the entire task into two parts and explicitly recognize the intent, operation objects and parameters usually achieves stronger interpretability and higher accuracy.
%We review some of the NN based methods in natural language understanding task.
Dividing the task into two parts usually achieves stronger interpretability and higher accuracy. For example, Xu \etal  \cite{xu2013convolutional} propose a joint model for intent determination and slot filling leveraging convolutional neural network-based triangular CRF. Guo \etal \cite{guo2014joint} employ path features constructed by semantic analysis tree in classification process. Zhang \etal \cite{zhang2016joint} combine Bi-GRU and CRF as the joint model for spoken language understanding. Liu \etal \cite{liu2016attention} emphasize the effectiveness of attention mechanism in intent detection and slot filling. In our work, we build the NL interpreter based on a deep-learning model to extract user intents from natural language utterances. We establish a joint model and leverage CRF and attention mechanism to improve the performance.


==> sections/VIS_vistalk.tex <==

\section{VisTalk}
To assess the design of our natural language framework, we build a proof-of-concept NL-based visualization authoring system in the form of VisTalk. %Here we discuss VisTalk design considerations and implementation, highlighting the usages of the natural language framework.
As shown in Figure \ref{fig:interface}, VisTalk provides a natural language interface for visualization creating and editing. The major parts of VisTalk are simply a text input box and the target visualization design. VisTalk takes users' natural language input and renders visualizations to show changes accordingly. After a user upload a tabular dataset, the data table will shown on the left. The user can specify multiple charts for the dataset. In the textbox (Figure \ref{fig:interface}b), users can type in their authoring utterances. While typing utterances, VisTalk auto-completes users utterances with a list of popular phrases (Figure \ref{fig:interface}g). Users can also modify existing utterances and the visualization updates automatically.
Currently, VisTalk supports bar charts, column charts, line charts, and pictographs. 
VisTalk parses the utterances sentence by sentence and render visualization changes to the users (Figure \ref{fig:interface}c). At the same time, visTalk highlight semantic types for the words and phrases and the table columns and values involved in the chart being edited. Users can fine-tune their statements by clicking the keywords for icons, colors, chart types, and values. The system pops out interactive widgets (Figure \ref{fig:interface}f) that helps users further specify or modify the parameters. %错的话


% \subsection{User Interface and Interaction}
% VisTalk provides a set of design views to support users' design. 
% For example, a user can input statements in the input box. Users input a list of sentences and VisTalk parses the input statements one by one. VisTalk 

% Finally, users can save the fine-tuned natural language for future replication. Users can ask VisTalk to ``export the authoring commands'' as a script. The system packs up the natural language utterances with the fine-tune values generated by system. The natural language-like script can be easily understood and modified for similar authoring tasks.

VisTalk is implemented based on our natural language framework. Through VisTalk, users first upload datasets to the backend database. Then, they can author visualizations against an underlying dataset with NL utterances. The utterances are sent to the NL interpreter. After processing, the NL interpreter send back corresponding  authoring actions. To execute an authoring action, VisTalk needs to resolve object selectors, execute data queries, and convert vague parameters into accurate default values. 


%Users then input natural language and the systems bind the data entities to the sentences, and output abstract utterances. For example, \todo{example}. After that, the abstract utterances are digested by the deep learning-based natural language interpreter, which extracts a list of intents, entities, and parameters. VisTalk then interprets the output intentions based on its' own visualization model and renders the visualizations through the visualization generator.


% The major parts of VisTalk are simply a text input box and the target visualization design. Users can upload the dataset in csv format and then start to type their commands. When one sentence is completed and the user presses ``enter'', the system parses the input and shows the change on the visualization directly. If there are vague descriptions, users can directly click on the text to make the command more accurate.

% \subsection{Design Considerations}
% We considered several factors of design considerations for developing a natural language-based visualization system. Different from traditional visualization authoring tools, natural language-based systems rely largely on users' text or speech input. The design of the systems should leverage the advantages of natural language and WIMP interactions.

% \begin{compactitem}
%     \item \textbf{Instant feedback of chart creations} The system should provide a prompt feedback to users' input. The  
%     \item \textbf{Easy to correct misunderstandings} The tool should support easy correction of misunderstanding between system and users. 
%     \item \textbf{Flexible switches between authoring paradigms} The misunderstandings come from the inadequate understanding 
%     \item \textbf{Smart reference and selection} Natural language contains ambiguity in referring objects. The system should support smart selection of visualizations.   \textbf{Name of the charts}
%     \item \textbf{Accurate or fuzzy parameter specifications.} A natural language-based system should support both accurate and fuzzy specifications. Usually, users may input a fuzzy description of the intention because they are not certain about the extent of their parameter specifications. The system should take advantage of the accuracy of direct specification with WIMP interface and fuzziness of natural language input.
% \end{compactitem}



% \subsection{VisTalk Implementation}
% We implemented VisTalk as a Web Application, and used a client-server architecture to distribute the NL interpreter and database operations on remote servers. VisTalk consists of three main components (1) NL interpreter (2) a program synthesis module (3) a visualization renderer...

% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth,height=150px]{pictures/architecture.pdf}
%     \caption{vistalk architecture}
%     \label{fig:interface}
%     %\vspace{-10px}
% \end{figure}







% \subsection{VisTalk Functions}
% VisTalk supports the basic functions provided by the natural language interpreter to configure the data binding, style, and higher level operations that supports nested layouts, pictographs, and multiple facets.
% By implementing these visualization authoring operations, we support the building blocks of visualization authoring in a flexible way. 

% Implementation detail for natural language understanding

% Natural Language Operations + objects.
% All the basic operations.
% Smart operations: 



\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1\linewidth]{pictures/examples.pdf}
    \caption{Example visualizations authored in VisTalk with natural language utterances. (a) is based on a stock datatset, (b) and (e) are based on a car sales dataset, (c) is based on a shark attacks dataset, and (d) is based on a product sales data. The terms displayed in bold are column names in data, and the terms displayed in italic are values in data.}
    \label{fig:examples}
    \vspace{-2px}
\end{figure*}

\textbf{Executing Operations}
VisTalk implements an execution engine that processes the interpreted authoring actions and executes the operations. If the operations and target objects are clearly specified, the execution engine blends the objects and calls the related functions. 
If the operation is not supported by VisTalk, the execution engine returns an error message to notice the users. If the operation is not supported but related operations are supported, VisTalk further show simple examples to help users understand the functions of the system.
If the authoring action are not fully specified, VisTalk predefine a set of rules to recommend proper actions for under specified utterances, following the research of chart recommendations \cite{setlur2019inferencing, mackinlay2007show}. For example, one common requests is ``Sales by year''. This can be parsed into \texttt{\{BindX, x axis, data field="Year"\}} and \texttt{\{BindY, y axis, data field="Sales"\}}.  VisTalk automatically recommends a bar chart based on the data types. 




\textbf{Selecting Objects}
VisTalk manages users' web session and maintains a list of objects on canvas with corresponding attributes. If the objects are clearly referred, VisTalk simply looks for the objects and applies the operations to the target objects.
For objects with selectors, VisTalk traverses through the object list and finds out all the objects with specific parameters. If the object is targeted by a pronoun, we simply take the most recent operated object. If the objects cannot be resolved, VisTalk shows an error message to notify users.



\textbf{Resolving Vague Parameters}
% three types of vague parameters: 
% VisTalk implement a wide range of dynamic widgets to deal with 
% Dynamic Widgets 
% change value (text box, +/- buttons)
% change category (select box)
% change color (color panel)
% choose color theme (select box)
% position (select box; +/- buttons)
% modify content
%Next, we identify the parameters from the output. The intents produced by the NL interpreter contain four types of paramters, namely, exact parameters, under specified parameters, vague parameters, and relational parameters. 
There are three types of parameters, exact parameters, vague parameters, and relational parameters.
For exact parameters, we directly map the extracted parameters to the data value. We just check whether the value can be legally assigned. For example, `10px' for height can be simply assigned to the objects. 
%For under specified parameters, VisTalk implements a wide range of dynamic widgets. For example, if a user inputs a statement, ``change the bar color'', the system highlights the keyword ``color'' and popups a color selector. 
For vague parameters, VisTalk maintains a list of explanations to the vague parameters supported by the NL interpreter. Whenever users input a vague parameter, VisTalk lookups the descriptive parameters and finds the corresponding accurate value. For example, the parameter ``red'' yields the color code RGB(255, 0, 0). For ``high'' values, VisTalk infers it to the range (average, max).
For relational parameters, VisTalk also empirically maintains a set of predefined rules to adjust the value. For examples, ``on the top'' for ``put it on the top of the china bar'', means putting the item 10px away from the rectangle; ``make it bigger'', means increasing the size by 20\%. For relational parameters, VisTalk also highlights the parameters in the original utterances to enable users to do modifications through interactive widgets.



% \subsection{Reusable Chart Templates}
% export the charts as templates.
% Power BI


